Relaxed Earth Mover's Distances for Chain- and Tree-connected Spaces and their use as a Loss Function in Deep Learning

The Earth Mover's Distance (EMD) computes the optimal cost of transforming one distribution into another, given a known transport metric between them. In deep learning, the EMD loss allows us to embed information during training about the output space structure like hierarchical or semantic relations. This helps in achieving better output smoothness and generalization. However EMD is computationally expensive.Moreover, solving EMD optimization problems usually require complex techniques like lasso. These properties limit the applicability of EMD-based approaches in large scale machine learning. We address in this work the difficulties facing incorporation of EMD-based loss in deep learning frameworks. Additionally, we provide insight and novel solutions on how to integrate such loss function in training deep neural networks. Specifically, we make three main contributions: (i) we provide an in-depth analysis of the fastest state-of-the-art EMD algorithm (Sinkhorn Distance) and discuss its limitations in deep learning scenarios. (ii) we derive fast and numerically stable closed-form solutions for the EMD gradient in output spaces with chain- and tree- connectivity; and (iii) we propose a relaxed form of the EMD gradient with equivalent computational complexity but faster convergence rate. We support our claims with experiments on real datasets. In a restricted data setting on the ImageNet dataset, we train a model to classify 1000 categories using 50K images, and demonstrate that our relaxed EMD loss achieves better Top-1 accuracy than the cross entropy loss. Overall, we show that our relaxed EMD loss criterion is a powerful asset for deep learning in the small data regime.

==> nips/crap.tex <==





The Earth Mover's Distance is a natural measure for probability distributions based on the optimal transport problem.
%It is also known as the Earth Mover's Distance, because it can be informally defined as the minimum effort required to move \emph{"dirt"} to make two distributions equal.
%However, it has seen limited use as a learning loss in deep learning frameworks because its computation in generally expensive,
%and the Kullback-Leibler (KL) divergence which can be calculated efficiently is used instead as a proxy.
Its use in deep learning frameworks has been hindered by its high computational cost,
but approximated versions have shown promising results.
We start by analyzing the Wasserstein distance for one dimensional distributions, as it can be computed efficiently in this particular case.
We derive a closed-form solution for its gradient that allows efficient calculation, but reveals convergence issues.
We solve this issues by enforcing the gradient to preserve the $\ell_1$ norm of the original distribution and minimizing the squared Wasserstein Loss.
We proceed to argue that both solutions for the one dimensional case are also valid for the general case.
Finally, we discuss the advantages of Wasserstein loss against the commonly used Kullback-Leibler divergence in predicting probability distributions.
We show how Wasserstein loss achieves better generalization and convergence rate with limited training data.

%Most criterions used for regression in deep learning evaluate each bin independently,
%which is fast, but is suboptimal for continuous distributions as more suited metrics are available for them.
%Particularly, the Earth Mover's Distance offers an hollistic metric for 
%We show how EMD gradient does not converge by showing a simple example:

the recent development of the Sinkhorn Distances (SD).
The SDs 


a recent breakthrough in its calculation.
 named Sinkhorn Distance.
The named Sinkhorn Distance is a regularized version of the EMD which can be calculated fast and approximates 


0.2 0.3 0 0.1 0.4

0.25 0.25 0.25 0.25 0.25

%It is also known as the Earth Mover's Distance, because it can be informally defined as the minimum effort required to move \emph{"dirt"} to make two distributions equal.
%However, it has seen limited use as a learning loss in deep learning frameworks because its computation in generally expensive,
%and the Kullback-Leibler (KL) divergence which can be calculated efficiently is used instead as a proxy.
Its use in deep learning frameworks has been hindered by its high computational cost,
but approximated versions have been used with promising results.
Nevertheless, the Wasserstein distance can be computed efficiently for one dimensional distributions, and we derive a closed-form solution for its gradient that allows efficient calculation, but reveals convergence issues.
We solve this issues by enforcing the gradient to preserve the $\ell_1$ norm of the original distribution and minimizing the squared Wasserstein Loss.
We proceed to argue that both solutions for the one dimensional case are also valid for the general case.
Finally, we discuss the advantages of Wasserstein loss against the commonly used Kullback-Leibler divergence in predicting probability distributions.
We show how Wasserstein loss achieves better generalization and convergence rate with limited training data.


\section{Introduction}
The Wasserstein metric is a natural measure for probability distributions based on the optimal transport problem.




The Wasserstein distance is a

Spectral analysis is performed in several domains of physiological monitoring (\eg~respiratory analysis~\cite{martinezbreath}, EEG~\cite{Sano2014}, ECG~\cite{clifford2006advanced}).
%However, despite the recent developments in deep learning, there are no good techniques to train regression networks in the spectral domain.
%The common approach is to treat the Power Spectral Density (PSD) as a probability distribution and train against the Kullback-Leibler (KL) divergence,
Regression models in the spectral domain enable several applications, often through the use of Power Spectral Density (PSD).
Within machine learning frameworks, PSD is commonly treated as a probability distribution and learned using the Küllback-Leibler (KL) divergence.
However, KL compares each bin independently. % and in fact is not a metric.
%We suggest using the Earth Mover's Distance (EMD) as the loss metric for spectral physiological data.
%The EMD distance has been seldomly used as it is obtained from dynamic programming techniques, and it was though not to be differentiable.
The Earth Mover's Distance (EMD) is a natural metric to compare distributions, but has seen limited use due to its computational cost.
% This is not the case for the 1D case, as we derived the closed-form solution for the 1 dimensional EMD gradient.
Nevertheless, for one dimensional distributions (\eg~PSD) the EMD can be computed efficiently, and we derive a closed-form solution for its gradient.
We enforce the gradient to preserve the $\ell_1$ norm of the original distribution.
% The formula reveals why pure EMD perform poorly as a loss function, so we show a modified $\ell_1$ preserving variation that performs efficiently.
% Our EMD GPU implementation is slower than Mean Squared Error (MSE) but faster than KL.
We evaluate on a data set of 81 sleep laboratory patients, predict breathing rate, and compare EMD as a loss against KL divergence and Mean Squared Error.

\section{Related Work}
Recently there have been efforts to integrate EMD as a loss criterion for deep learning~\cite{solomon2014wasserstein,frogner2015learning}.
However, as compared to other criteria such as Mean Squared Error (MSE) or KL divergence, the perceived inefficiency in EMD computation has hindered progress.



In the general case, calculating the EMD requires to solve the optimal transport problem that turns the source distribution to the target one.
As this calculation is expensive, much effort has been invested in relaxed definitions of the EMD that allow more efficient computation~\cite{cuturi2015smoothed,shirdhonkar2008approximate,pele2009fast,cuturi2013sinkhorn,cuturi2013fast}.

% Recently, Frogner~\etal~\cite{frogner2015learning} suggest a deep learning framework using the latest lightspeed~\cite{cuturi2013sinkhorn} EMD calculation that transforms the problem into a matrix balancing problem which is efficiently solved using the Sinkhorn-Knopp algorithm.
Recently, Frogner~\etal~\cite{frogner2015learning} suggest a method to incorporate EMD in a deep learning framework using the entropic regularization proposed by Cuturi~\cite{cuturi2013sinkhorn}.
We consider that this approach to compute EMD is unnecessarily complex for the common case of one dimensional distributions for which there exists a closed-form solution.



\section{Convergence behavior of the Earth Mover's Distance}

Within gradient descent methods, the Earth Mover's Distance has a distinct behavior that needs to be well understood in order to use it correctly.

\noindent\textbf{Strong initial gradient magnitude.}
Compared to common non-space aware losses, the EMD shows huge variations in gradient magnitude which depends on the dimensionality of the space (\ie moving dirt from the first dimension of the descriptor to the last one).
This usually implies that EMD provides fast convergence rate at the beginning of the optimization process, and more care than usual must be taken in choosing the right learning rate in order to avoid divergence.

\noindent\textbf{Weak late gradient magnitude.}
Conversely, once the "dirt" is close to its final destination, convergence turns into a crawl, as moving "dirt" becomes cheap, and thus the gradient flattens.
We suggest to combine always EMD with other losses, specially Mean Squared Error, in order to obtain a more steady learning rate.

\section{Synergy with Mean Squared Error loss}

As we discussed on the previous section, we suggest to use EMD together with some other loss in order to obtain a smoother behavior during training.

Frogner~\etal~\cite{frogner2015learning} suggested to combine the relaxed EMD~\equref{relaxedEMD} with the Küllback-Leibler (KL) divergence as a way to extend their domain to non normalized distributions.
Conversely we also suggest to combine EMD with a second metric \textbf{always}, we do it from the opposite point of view:
choose a main metric that has good convergence properties, and combine it with the EMD that will act as a smoothness guard (\ie not interfering with the training unless non-smoothness is detected).
Our goal is to achieve fast training at the beginning when the output is not smooth, thanks to EMD, and good finesse thanks to the main metric.

We have several options when choosing the best metric to use with EMD.
The KL divergence is clearly the best match for the relaxed EMD as its gradient has an entropic regularization term in the logarithmic space.
Therefore, the Mean Squared Error (MSE) is the best metric for our $\oEMD^2_L1$ as our transport relaxation has the same structure.
Furthermore, $\emph{gMSE}(\mathbf{p}, \mathbf{q})$ is $2(\mathbf{p}-\mathbf{q})$, as the $\ell_1$ norms of $\mathbf{p}$ and $\mathbf{q}$ are the same, 
$\Sigma^N\emph{gMSE}(\mathbf{p}, \mathbf{q})=0$ and thus is $\ell_1$ preserving.
This means that, unlike~\cite{frogner2015learning}, we can use $\oEMD^2_L1$ + MSE both in normalized and unnormalized scenarios without altering the criterions.

\section{Using EMD for non $\ell_1$-norm = 1 distributions}

The original EMD is not defined for $\norm{\mathbf{p}}_1 \ne \norm{\mathbf{q}}_1$.
Although there are several ways to modify the EMD for unnormalized distributions~\cite{pele2009fast,chizat2015unbalanced,frogner2015learning} we consider that this goes against the spirit of the metric.
We think that 
%Therefore, prior to computing the EMD, we $\ell_1$-normalize the input distributions (see Eq.~\eqref{eq:emd}).
%Such a normalization can lead to a mismatch between the absolute magnitudes, which may result in numerical instability during optimization.
%We address this by defining our loss as the weighted combination of EMD and MSE criterion ($w_{\text{EMD}} = 0.9, w_{\text{MSE}} = 0.1$).




However, in 20

%\section{Minimize the squared EMD}


%This makes performing gradient descent difficult, as the learning parameter $\lambda$ becomes the step size taken at each iteration,
%thus the precision of the estimation does not increase over time, and the algorithm tends to oscillate or converge too slowly.

%Frogner\etal~\cite{frogner2015learning} were aware of the problem as they claim their algorithm is not proven to converge but could not argue why,
%however their relaxed regularization they added to make EMD tractable in their framework had the side effect to add a small convex part to the optimization problem.
%This convex part of the equation is dominant where EMD has zero gradient, and thus their algorithm converges.

%We suggest a classical, stronger approach by minimizing the squared EMD thus using the following gradient:

%\begin{equation}
%\nabla \emph{EMD}^2(\mathbf{a},\mathbf{b}) = 2 \emph{EMD}(\mathbf{a},\mathbf{b}) \nabla \emph{EMD}(\mathbf{a},\mathbf{b})
%\end{equation}

\subsection{Implementation details}
% Our Torch~\cite{collobert2011torch7} implementation of the EMD criterion is slower than MSE,
% but faster than the KL divergence (tested for $N=30$ on a GPU).

%Equations \eqref{eq:grad} and \eqref{eq:gradZeroSum} show how EMD behaves similarly to $\ell_1$ distance.

\vspace{1mm}
\noindent\textbf{Absolute magnitude.}
The original EMD is not defined for $\norm{\mathbf{a}}_1 \ne \norm{\mathbf{b}}_1$.
Although there are several ways to modify the EMD for unnormalized distributions~\cite{pele2009fast,chizat2015unbalanced} we consider that this goes against the spirit of the metric.
Therefore, prior to computing the EMD, we $\ell_1$-normalize the input distributions (see Eq.~\eqref{eq:emd}).
Such a normalization can lead to a mismatch between the absolute magnitudes, which may result in numerical instability during optimization.
We address this by defining our loss as the weighted combination of EMD and MSE criterion ($w_{\text{EMD}} = 0.9, w_{\text{MSE}} = 0.1$).
% To address the normalization problem, we suggest to combine the EMD loss together with a traditional loss sensible to the norm.
% In our examples we apply EMD and MSE criteria with respective weights of 0.9 and 0.1.
% Not only this forces the network to learn the absolute magnitude of a signal (albeit slower than its distribution shape), 
% it also allows the network to keep converging where $\nabla$EMD equals zero.

\vspace{1mm}
\noindent\textbf{Non-negative distributions.}
We square the output of the last layer of our model to ensure non-negative values for the distribution.
% Finally, we square the output layer to force all vectors to be positive.




We train a two layer Multilayer Perceptron regressor to predict the breathing signal PSD from the chest excursion of 81 sleep laboratory patients with different degrees of apnoea, and use the PSD from a nose thermistor as reference.
%we capture 30 second windows at 20Hz and train against the PSD obtained from a nose thermistor. 
As we see in~\figref{results}, the PSD obtained using $g\EMD_{\text{L1}}$ loss converges faster and provides a better estimation of the breathing rate (the largest peak of the PSD).
We also see that the gradient sums to 0 for $g\EMD_{\text{L1}}$.



==> nips/earthdistance.tex <==
%!TEX root = nips2016.tex
\section{The Earth Mover's distance}
As discussed earlier, the EMD is generally defined in the discrete domain.
Here, the probability mass, or \emph{dirt} is distributed in discrete piles or bins, and the effort of moving a mound of \emph{dirt} between two bins is a non-negative cost linearly proportional to the amount of \emph{dirt}.

Within this discrete domain, the general form of the $\EMD$ distance between two distributions $\mathbf{p}, \mathbf{q}\in \mathbb R^N_{+}$ with $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1$ is

\begin{equation}
\label{eq:emd_general}
\EMD(\mathbf{p}, \mathbf{q}) = \inf_{T \in U(\mathbf{p}, \mathbf{q})} \langle M, T \rangle \, ,
\end{equation}

where $\langle \cdot, \cdot \rangle$ is the Frobenius inner product and $M \in \mathbb R^{N \times N}_{+}$ defines the generalized distance between bins.
$U(\mathbf{p}, \mathbf{q})$ is the set of valid transport plans between $\mathbf{p}$ and $\mathbf{q}$, and is defined as

\begin{equation}
\label{eq:transport_domain}
U(\mathbf{p}, \mathbf{q}) = \{ T \in \mathbb R^{N \times N}_{+} : T \mathbf{1}_N = \mathbf{p},\, T^\top \mathbf{1}_N = \mathbf{q} \} \, .
\end{equation}

$\mathbf{1}_N$ is a $N$ dimensional vector of all $1$, and $T$ is constrained such that its row sum corresponds to the distribution $\mathbf{p}$ and column sum to $\mathbf{q}$.



\subsection{Sinkhorn distance}

The general formulation of the $\EMD$ (Eq.~\ref{eq:emd_general}) is solved using linear programming that is computationally expensive.
However, this problem was greatly alleviated by Cuturi~\cite{cuturi2013sinkhorn} who suggested a smoothing term for the $\EMD$ in the form of

\begin{equation}
\label{eq:sd}
\SD_\gamma(\mathbf{p}, \mathbf{q}) = \inf_{T \in U(\mathbf{p}, \mathbf{q})} \langle M, T \rangle - \gamma\langle T, log T \rangle \, ,
\end{equation}

which allows to use the Sinkhorn-Knopp algorithm~\cite{sinkhorn1967diagonal} to obtain an iterative and efficient solution.




\subsection{Earth Mover's Distance for one dimensional distributions}

We analyze a version of the problem where the distribution bins are placed in a one dimensional space in such a way that
traveling between two bins requires an ordered visit to every bin between the source and the target (see \figref{onedim} (right)).

In this case the distance between bins $M$ is defined recursively as
\begin{equation}
M_{i,j} =
\begin{cases}
0 &\text{if } i = j \, ,\\
M_{i-1,j} + d(i-1,i) &\text{if } i > j \, ,\\
M_{j,i} &\text{if } i < j \, .
\end{cases}
\end{equation}
Here, $d(i-1, i)$ is the distance between two consecutive bins (typically $1$), and the recursive definition ensures that only consecutive bin distances are considered.

The above bin distances facilitate a simple solution to the $\EMD$ computation using a recursion.
% There is a simple solution for this problem that uses the following recursion:
Each bin either receives all the excess \emph{dirt} that results from leveling previous bins, or in case of a deficit, tries to provide for it.
Note that the cost of going left-to-right $M_{ij}$ or right-to-left $M_{ji}$ is symmetric, and the magnitude of the excess or deficit helps compute the distance:
% In both cases, the cost to pay is the same as $M'_{ij}=M'_{ji}$,
% therefore the absolute value fulfills both cases in the following expression:

\begin{equation}
\label{eq:emd}
\oEMD(\mathbf{p}, \mathbf{q}) = \sum_{i=1}^{N-1} M_{i,i+1} \cdot | \varphi_i |,
\text{ where }
\varphi_i =
    \sum_{j=1}^i \left(
		  \frac{p_j}{\norm{\mathbf{p}}_1} -  \frac{q_j}{\norm{\mathbf{q}}_1}
    \right) \, .
\end{equation}

For notational brevity, we will refer to $M_{i,i+1}$ as $\hat{M}_i$.
The above formulation is rewritten with the sign function as
\begin{equation}
\oEMD(\mathbf{p}, \mathbf{q}) =  \sum_{i=1}^{N-1} \hat{M}_i  \cdot \sgn(\varphi_i) \cdot \varphi_i \, .
\end{equation}

Note that as both distributions have the same amount of total mass, and we progressively level out the \emph{dirt} over all bins, $\varphi_N = 0$, allowing us to compute the outer sum only up to $N-1$.
%, and therefore dimensionality gets reduced by one.





\subsection{Gradient of the Earth Mover's Distance}

In a learning framework, model parameter updates are often performed using the gradient or Hessian.
To integrate $\EMD$ as a loss, we now compute the analytical form of the gradient.

%\begin{equation}
%\emph{EMD}(\mathbf{a},\mathbf{b}) = { \sum_{i=1}^{N-1}\abs{\sum_{j=1}^i \left(a_j-b_j\right)} \over \sum_{i=1}^{N-1} a_i }
%\end{equation}
%If we and $\norm{\mathbf{a}}_1 = \norm{\mathbf{b}}_1 = 1$ is:
%From now on, we asume without lack of generality $\Sigma_i a_i = \Sigma_i b_i = 1$:
%\begin{equation}
%\emph{EMD}(\mathbf{a},\mathbf{b}) = \sum_{i=1}^{N-1}\abs{\sum_{j=1}^i \left(a_j-b_j\right)}
%\end{equation}

Let $\mathbf{e}_k$ be a unit vector of length $N$ whose value at dimension $k$ is 1, and 0 elsewhere.
% To work on the derivative we define the helper unit vector  such as:
%
% \begin{equation}
% \mathbf{\hat{e}_{k}} =
% \begin{cases}
% 0 &\text{if} i \ne k,\\
% 1 &\text{if} i =  k.
% \end{cases}
% \end{equation}
%
%therefore
%
%\begin{equation}
%\begin{split}
%\emph{EMD}\left( \mathbf{a}+h\mathbf{\hat{e}_{k}},\mathbf{b}\right) = \\
%\sum_{i=1}^{N-1}\abs{
%    \sum_{j=1}^i \left(
%        {a_j \over \norm{\mathbf{a}}_1+h} -
%        {b_j \over \norm{\mathbf{b}}_1 }\right) +
%  h \sum_{j=1}^i {\delta_{jk} \over \norm{\mathbf{a}}_1 + h} }
%\end{split}
%\end{equation}
%
For a small perturbation $h$, we compute the distance between the modified distribution $\mathbf{p} + h\mathbf{e}_k$ and $\mathbf{q}$ as:
% We can write $\EMD(\mathbf{a} + h\mathbf{e}_{k}, \mathbf{b})$ as:
% For a small $h$, small enough not to impact the output of the sign function,
% we can write
\begin{equation}
\oEMD(\mathbf{p} + h\mathbf{e}_k, \mathbf{q}) \simeq
    \sum_{i=1}^{N-1} \hat{M}_i  \cdot \sgn(\varphi_i)
    \sum_{j=1}^i \left( \frac{p_j + h \delta_{jk}}{\norm{\mathbf{p}}_1 + h} -  \frac{q_j}{\norm{\mathbf{q}}_1} \right) \, ,
\end{equation}
where $\delta_{jk} = 1$ when $j = k$.
Note that by choosing $h$ small enough, $\sgn(\varphi_i)$ can be assumed to remain unchanged.

We now compute the partial derivative for $\EMD$.
As we define $\EMD$ on distributions with equal total mass (Eq.~\ref{eq:emd}), without the loss of generality,
we assume $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1 = 1$, and operate on unit $\ell_1$ norm vectors $\hat{\mathbf{p}}$ and $\hat{\mathbf{q}}$.
\begin{eqnarray}
\label{eq:grad_emd}
g\oEMD
& = & \frac{\partial \oEMD( \hat{\mathbf{p}}, \hat{\mathbf{q}} )} {\partial p_k}
=
\lim_{h \rightarrow 0} \,\, \frac{1}{h}
\left( \EMD(\hat{\mathbf{p}} + h \mathbf{e}_k, \hat{\mathbf{q}}) - \EMD(\hat{\mathbf{p}},\hat{\mathbf{q}}) \right) \\
& \simeq &
\lim_{h \rightarrow 0} \,\,\frac{1}{h}
  \sum_{i=1}^{N-1} \hat{M}_i  \cdot \sgn (\varphi_i)
  \left(
    \sum_{j=1}^i \left( \frac{\hat{p}_j + h \delta_{jk}}{1 + h} - {\hat{q}_j} \right) -
    \sum_{j=1}^i \left( \hat{p}_j - \hat{q}_j \right)
  \right) \nonumber \\
& = &
\lim_{h \rightarrow 0} \,\,\frac{1}{h}
  \sum_{i=1}^{N-1} \hat{M}_i  \cdot \sgn (\varphi_i)
  \sum_{j=1}^i \frac{h \delta_{jk} - h \hat{p}_j}{1 + h} \nonumber \\
& = &
\label{eq:gemd}
  \sum_{i=1}^{N-1} \hat{M}_i  \cdot \sgn (\varphi_i) \sum_{j=1}^i \left( {\delta_{jk} - \hat{p}_j} \right) \, .
\end{eqnarray}




\subsection{$\ell_1$ preserving gradient}

The above gradient disobeys the law of \emph{dirt} conservation and creates new or destroys existing \emph{dirt}, changing the total mass of the distributions.
As the gradient sum is not 0, it makes the gradient unsuitable for applications%
\footnote{Symbolic differentiation performed by Theano or TensorFlow produces non-$\ell_1$ preserving gradients that are unsuitable for optimization.}.

To solve this problem, and in contrast to $\mathbf{e}_k$, we redefine our unit vector such that its sum is 0.
We propose a set of vectors $\tilde{\mathbf{e}} \in \{-1, N-1\}^N$, where $\tilde{\mathbf{e}}_k$ takes the value $N-1$ at dimension $k$, and $-1$ elsewhere.

The partial derivatives for such a setting are
\begin{eqnarray}
\label{eq:gradZeroSum_emd}
g\oEMD_{L1}
& = & \frac{\partial \oEMD_{L1}( \hat{\mathbf{p}}, \hat{\mathbf{q}} )} {\partial p_k}
=
\lim_{h \rightarrow 0} \,\, \frac{1}{h}
\left( \EMD(\hat{\mathbf{p}} + h \tilde{\mathbf{e}}_k, \hat{\mathbf{q}}) - \EMD(\hat{\mathbf{p}}, \hat{\mathbf{q}}) \right) \\
& \simeq &
\lim_{h \rightarrow 0} \,\, \frac{1}{h}
  \sum_{i=1}^{N-1} \hat{M}_i \cdot \sgn (\varphi_i)
  \left(
    \sum_{j=1}^i \left( \hat{p}_j +  h (N \delta_{jk} - 1) - \hat{q}_j \right) -
    \sum_{j=1}^i \left( \hat{p}_j - \hat{q}_j \right)
  \right) \nonumber \\
& = &
\lim_{h \rightarrow 0} \,\, \frac{1}{h}
  \sum_{i=1}^{N-1} \hat{M}_i \cdot \sgn (\varphi_i)
  \sum_{j=1}^i h \left(N \delta_{jk} - 1 \right) \nonumber \\
& = &
\label{eq:gemd_l1}
  \sum_{i=1}^{N-1} \hat{M}_i \cdot \sgn (\varphi_i) \cdot (N \cdot H(i-k) - i) \, ,
\end{eqnarray}
where $H: \mathbb{R} \rightarrow \{0, 1\}$ is the Heaviside step function defined as $H(n) = \{1 \text{ if } n \geq 0, 0 \text{ elsewhere}\}.$





\subsection{Relaxed Earth Mover's Distance}

As compared to the original $\EMD$ gradient (Eq.~\ref{eq:gemd}), the $\ell_1$ preserving gradient (Eq.~\ref{eq:gemd_l1}) is numerically stable and avoids erosion or addition of new dirt.
This is an important step forward to use $\EMD$ in learning frameworks.
However, as the distance uses absolute values ($|\varphi_i|$) we observe similar properties to $\ell_1$ optimization.

In particular, when $\hat{M}_i \in \mathbb{N}$, it is easy to see that the terms of $g\oEMD_{L1}$ are integer values.
Furthermore, as small changes to the distribution does not change the gradient, the Hessian is zero except at a few discrete set of points making optimization a hard process.

% \begin{enumerate}
% \item For $\hat{M} \in \mathbb{N}^N$ the gradient is made up of integer values.
% \item Its Hessian matrix is zero except over a discrete set of points.
% \end{enumerate}

To solve these issues, we suggest a relaxed form of the $\EMD$ where the cost is calculated proportional to a certain power of the excess/deficit of \emph{dirt}.

\begin{equation}
\label{eq:emd_rho}
\oEMD^\rho(\mathbf{p}, \mathbf{q}) = \sum_{i=1}^{N-1} \hat{M}_i \cdot | \varphi_i |^\rho \, .
\end{equation}

In particular, we explore the case with $\rho=2$ that bears similarity with the popular Mean Squared Error loss.
The standard and $\ell_1$ preserving gradients for $\oEMD^2$ are:

\begin{eqnarray}
\label{eq:g_emd2}
g\oEMD^2
= \frac{\partial \oEMD^2( \hat{\mathbf{p}}, \hat{\mathbf{q}} )} {\partial p_k}
& = & 2 \sum_{i=1}^{N-1} \hat{M}_i \cdot \varphi_i
  \sum_{j=1}^i \left( {\delta_{jk} - \hat{p}_j} \right) \, , \\
\label{eq:g_emd2_l1}
g\oEMD^2_{L1}
= \frac{\partial \oEMD^2_{L1}( \hat{\mathbf{p}}, \hat{\mathbf{q}} )} {\partial p_k}
& = & 2 \sum_{i=1}^{N-1} \hat{M}_i \cdot \varphi_i
%  \sum_{j=1}^i ( N \delta_{jk} - 1 ) \, ,
  \cdot (N \cdot H(i-k) - i) \, .
\end{eqnarray}

We see that $g\oEMD^2_{L1}$ preserves the nice properties of conserving dirt, while having real valued gradients.
In addition, we see that $\EMD^2$ also exhibits non-zero Hessians.

\begin{eqnarray}
% \label{eq:hessian_emd2}
% \frac{\partial^2 \oEMD^2( \hat{\mathbf{p}}, \hat{\mathbf{q}} )} {\partial p_k \partial p_l}
% & = & 2 \sum_{i=1}^{N-1} \hat{M}_i \cdot  \sum_{j=1}^i \left( {\delta_{jl} - \hat{p}_j} \right) \cdot  \sum_{j=1}^i \left( {\delta_{jk} - \hat{p}_j} \right) \, , \,  \text{and} \\
\label{eq:hessian_emd2_l1}
\frac{\partial^2 \oEMD^2_{L1}( \hat{\mathbf{p}}, \hat{\mathbf{q}} )} {\partial p_k \partial p_l}
& = & 2 \sum_{i=1}^{N-1} \hat{M}_i \cdot (N \cdot H(i-l) - i) \cdot (N \cdot H(i-k) - i) \, .
\end{eqnarray}

% Both Hessians are positive semi-definite for any $\mathbf{p}, \mathbf{q}\in \mathbb R^N_{+}$ with $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1 = 1$.%\footnote{See proof in appendix A}


==> nips/experiments.tex <==
%!TEX root = nips2016.tex
\section{Experimental analysis}

\noindent\textbf{Setup.}
We implement our regression model with the $\EMD$ criterion using Torch~\cite{collobert2011torch7}\footnote{Code will be made publicly available}.
Note that $\varphi_i$ can be computed very fast through the use of a cumulative sum operator (\texttt{cumsum}).


\subsection{Convergence by Gradient Descent}

We analyze the convergence behavior of the four different versions of the gradients.
We propose a toy experiment where a random source distribution $\mathbf{p}$ is converted into a random target distribution $\mathbf{q}$ using gradient descent as follows:
\begin{eqnarray}
\hat{\mathbf{p}}_0     & = & \mathbf{p} \nonumber \\
\hat{\mathbf{p}}_{t+1} & = & \hat{\mathbf{p}}_t - \lambda_t \nabla_{\hat{\mathbf{p}}_t} \oEMD^\rho(\hat{\mathbf{p}}_t,\mathbf{q}) \, .
\end{eqnarray}

The experiment details are: $\mathbf{p}, \mathbf{q} \in \mathbb R^N_{+}$, $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1 = 1$, $N=64$, $\hat{M}_i = 1$ and $\lambda_0 = 2^{20}$.

Finding an optimal fixed learning rate for different versions of the gradients is a significant problem in itself.
We alleviate this by performing backtracking line search at each iteration adjusting $\lambda$ using a scaling factor of $\sqrt{2}$ so as to make $\hat{\mathbf{p}}_{t+1}$ similar to $\mathbf{q}$.

We evaluate two experimental settings for the $\EMD$ metric.
(i) \textbf{Easy}: $\mathbf{p}$ and $\mathbf{q}$ are vectors with random samples drawn from a uniform distribution in all the $N$ bins.
We expect that the amount of \emph{dirt} transported to make $\mathbf{p}$ equal to $\mathbf{q}$ is small.
(ii) \textbf{Hard}: we zero-out the right half of $\mathbf{p}$ and the left half of $\mathbf{q}$ while maintaining $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1 = 1$.
Here, all the \emph{dirt} from $\mathbf{p}$ needs to be displaced, which is a harder transport problem.
We report averaged results over 64 runs in~\figref{resultsA} (left Easy, right Hard).

% On the left column of~\figref{resultsA} we evaluate the behavior of $\EMD$ when $\mathbf{p}$ and $\mathbf{q}$ are randomly sampled from a uniform distribution along all $N$ dimensions.
% In this case, the distance required to transport \emph{dirt} is minimal.
% Conversely, the right column shows a case where the right half of $\mathbf{p}$ is zeroed, and the left half of $\mathbf{p}$ is also zeroed, while maintaining $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1 = 64$.
% This implies that \emph{all} the "dirt" from $\mathbf{p}$ needs to be displaced, thus implying much higher magnitudes.
% We report the average of 64 runs.
% Evaluation is performed under the $\EMD$ metric, as we normalize both vectors before evaluating the distance (see Eq.~\ref{eq:emd}) the actual norm of $\mathbf{p}$ or $\mathbf{q}$ is irrelevant.

\textbf{Optimal} $\EMD$ \textbf{does not converge.}
We see in the top row of \figref{resultsA} that the optimal $\EMD$ does not converge.
A reason for this is the zero Hessian that implies that the gradient brings no information about step size.
% Our simple line search is unable to find the edges of the simplex, and is easily lost.
In contrast, the relaxed $\EMD$ (Eq.~\ref{eq:emd_rho}) presents a steady decline for both settings.

\textbf{$\ell_1$ preserving gradients.}
A second observation is the bottom row of \figref{resultsA}.
Here, we see that the $\ell_1$ preserving gradients ($g\oEMD_{L1}$, $g\oEMD^2_{L1}$) do not change the total mass of the distributions, while the gradients $g\oEMD$ and $g\oEMD^2$ change.
In fact, for the Hard experiment, $g\EMD^2$ starts diverging rapidly around iteration 200 and can not recover.

\textbf{Best convergence by} $g\EMD^2_{L1}$.
The $\ell_1$ preserving, relaxed $\EMD$ gradient shows good performance consistently through both experiments.
The learning rate is steady, total mass is maintained, and error reduces significantly.
 % which converges at a constant rate while having an almost constant learning rate and not altering the norm of $\mathbf{p}$.
As a side note, given the current setup, Mean Squared Error ($\MSE$) converges to zero in a single step as it can pick the best $\lambda$.

\begin{figure}[t]
\centering
\subfloat{
\begin{tikzpicture}
    \begin{axis}[%
    hide axis,
    xmin=10,
    xmax=50,
    ymin=0,
    ymax=0.4,
	legend columns=4,
    legend style={}
    ]
    \addlegendimage{line width=1.5pt, purple}
    \addlegendentry{$g\emph{EMD} \quad$};
    \addlegendimage{line width=1.5pt, blue}
    \addlegendentry{$g\emph{EMD}_{L1} \quad$};
    \addlegendimage{line width=1.5pt, teal}
    \addlegendentry{$g\emph{EMD}^2 \quad$};
    \addlegendimage{line width=1.5pt, olive}
    \addlegendentry{$g\emph{EMD}^2_{L1} \quad$};
    \end{axis}
\end{tikzpicture}}
\\
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=2.8cm,  width=5.3cm,  ymode = log,
scale only axis, ymin=1e-4,ymax=1e+4,xmin=0,xmax=2000 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=Error (EMD),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=north east,font=\scriptsize}]
\input{artificialNearScore}
\end{axis}
\end{tikzpicture}}
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=2.8cm,  width=5.3cm,  ymode = log,
scale only axis, ymin=1e-4,ymax=1e+4,xmin=0,xmax=2000 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=Error (EMD),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=north east,font=\scriptsize}]
\input{artificialFarScore}
\end{axis}
\end{tikzpicture}}
\\
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=2.8cm,  width=5.3cm,  ymode = log,
scale only axis, ymin=1e-20,ymax=1e+20,xmin=0,xmax=2000 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=Learning rate ($\lambda$),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=north east,font=\scriptsize}]
\input{artificialNearLearn}
\end{axis}
\end{tikzpicture}}
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=2.8cm,  width=5.3cm,  ymode = log,
%log ticks with fixed point,
scale only axis, ymin=1e-20,ymax=1e+20,xmin=0,xmax=2000 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=Learning rate ($\lambda$),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=north east,font=\scriptsize}]
\input{artificialFarLearn}
\end{axis}
\end{tikzpicture}}
\\
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=2.8cm,  width=5.3cm,
y filter/.code={\pgfmathparse{#1/64}\pgfmathresult},
%log ticks with fixed point,
scale only axis, ymin=0.9,ymax=1.1,xmin=0,xmax=2000 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=$\Sigma \hat{\mathbf{p}}$,  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=north east,font=\scriptsize}]
\input{artificialNearSum}
\end{axis}
\end{tikzpicture}}
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=2.8cm,  width=5.3cm,  ymode = log,
%log ticks with fixed point,
scale only axis, ymin=1e1,ymax=1e30,xmin=0,xmax=2000 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=$\Sigma \hat{\mathbf{p}}$,  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=north east,font=\scriptsize}]
\input{artificialFarSum}
\end{axis}
\end{tikzpicture}}
\caption{
We compare the convergence behavior of the $\EMD$ in two different settings.
\emph{Left}: in the \textbf{Easy} setting, two uniformly sampled distributions are compared.
\emph{Right}: in the \textbf{Hard} setting, the distributions are sampled in a non-overlapping manner which requires all the \emph{dirt} to be displaced.
We see that the optimal $\EMD$ fails to converge as its Hessian is zero, and the gradient carries no information about the step size required to converge (top row).
The $g\EMD^2_{\text{L1}}$ shows good performance across the 4 alternatives, converging in all cases while using a stable learning rate, and maintaining the total mass of the distribution (keeping $\ell_1$ norm constant).
}
\vspace{-2mm}
\label{fig:resultsA}
\end{figure}





\subsection{Analyis of the shape of the gradient}
Plotting the gradients provide a good impression of the actual behavior of the $\EMD$ and the reason it serves as a holistic optimization over the full distribution.
In \figref{resultsB} (left), we compare a uniform distribution with one that has a single peak.
The $\EMD$ gradients affect every bin as the mass propagates to flatten the distribution.
In particular, at the bins surrounding the peak, the gradient for $\EMD$ has the opposite sign as that for $\MSE$.

In \figref{resultsB} (right), we compare two mirrored distributions with one peak each.
Here, we notice that the $\ell_1$ preserving gradients show 0 gradient at the center bin, demonstrating the symmetric nature.

\begin{figure}[ht!]
	\centering
	\subfloat{\includegraphics[width=6.8cm]{figures/gradA.png}}\quad
	\subfloat{\includegraphics[width=6.8cm]{figures/gradB.png}}
	\caption{Gradient flow to convert a source distribution $\mathbf{p}$ to a target $\mathbf{q}$.
    Different versions of the gradients are analyzed and plotted on top of each other.}
	\label{fig:resultsB}
\end{figure}







\subsection{Power Spectral Density prediction of synthetic signals with noise}

In this experiment we estimate the Power Spectral Density (PSD) of a synthetic signal using a neural network and evaluate it using the Earth Mover's Distance.
Our dataset consists of vectors of size $N=64$ each containing a single sine wave of unit amplitude and frequency $F = \{ f \in \mathbb{N} : 5~\le~f~\le~15\}$.
The signals are corrupted with additive white Gaussian noise (AWGN) of $\sigma^2=0.2$.
We generate 2,000 vectors for each frequency to obtain a total of 22,000 data samples.
We use 1000 vectors for each frequency to train the model, and the remainder for test.

Our network consists of two layers that are sufficient for the complexity of this problem.
The first layer consists of $16$ \emph{temporal convolution} filters with a receptive field of $11$.
We apply the \emph{tanh} nonlinearity, and stack a fully connected layer on top of this.
This output layer non-linearity is a \emph{square} function that ensures positive outputs.

As discussed before, using SGD with the optimal $\EMD$ is tricky as the learning rate needs to be constantly adjusted to ensure convergence.
We thus use the \emph{Adam} optimizer~\cite{ba2015adam}.

The test error for predicting PSD is plotted in \figref{resultsC}.
Firstly, note how using \emph{Adam} helps to achieve convergence for all variants of the $\EMD$ gradient.
Nevertheless, while all gradients are able to train the model, $g\oEMD^2_{L1}$ converges faster than the others.

\begin{figure}[t]
\centering
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=3cm,  width=7.4cm,
x filter/.code={\pgfmathparse{#1/10}\pgfmathresult},
scale only axis, ymin=0,ymax=3,xmin=0,xmax=15 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=Test Error (EMD),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=outer north east,font=\scriptsize}]
\input{experimentSinus}
\legend{$g\emph{MSE}$,$g\emph{EMD}$,$g\emph{EMD}_{L1}$,$g\emph{EMD}^2$,$g\emph{EMD}^2_{L1}$}
\end{axis}
\end{tikzpicture}}
\vspace{-0.2cm}
\caption{We train a 2 layer neural network regressor to estimate the PSD of an artificial sinusoid contaminated by noise.
As the PSD is a holistic operation, $\EMD$ performs well on this task.
With enough data, and smarter optimization schemes like Adam, all versions of the gradient are capable of achieving the similar errors.
However, $g\emph{EMD}^2_{L1}$ demonstrates faster convergence.}
\label{fig:resultsC}
\vspace{-0.3cm}
\end{figure}






\subsection{Power Spectral Density prediction of Real Signals}
In our final experiment we evaluate the use of $\EMD$ on real-world data.
Our task is to predict the PSD of breathing rate of a patient using chest excursion signals (a nose thermistor acts as reference).
Our data is recorded from 75 patients at a sleep laboratory, where 200 clips of 1 minute each are extracted for each patient, giving us a corpus of 15000 samples.
We use 60 patients to train our models, and the remainder 15 as test.
 % using a mini-batch size of 100 (randomly sampled), and 15 were used for the testing set.
We use a similar network to the previous experiment, but scale the input and output layers to match input (600) and output (30) dimensions.

In this experiment, noise is negligible if the patient is relaxed.
On the other hand, if the patient moves, sits, or talks during the clip, the correlation between chest movement and respiration drops.
In \figref{resultsD}, we see that \emph{Adam} manages to converge the model significantly faster and better using the $\EMD$ gradients, compared to the $\MSE$.
In fact, the holistic optimization is capable of extracting more information from the source data, as the model when using $\EMD$ gradients converges within the a fraction of the first epoch.
This highlight the benefits of using $\EMD$ distances in cases where capturing data is expensive.


\begin{figure}[t]
\centering
\subfloat{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=3cm,  width=7.3cm,
x filter/.code={\pgfmathparse{#1/120}\pgfmathresult},
scale only axis, ymin=0,ymax=10,xmin=0,xmax=10 ,enlargelimits=false, y label style={at={(axis description cs:-0.1,.5)},anchor=south},  ylabel=Test Error (EMD),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend style={legend pos=outer north east,font=\scriptsize}]
\input{experimentPSD}
\legend{$g\emph{MSE}$,$g\emph{EMD}$,$g\emph{EMD}_{L1}$,$g\emph{EMD}^2$,$g\emph{EMD}^2_{L1}$}
\end{axis}
\end{tikzpicture}}
\caption{We train a regressor to estimate the PSD of real breathing signals, using the chest excursion as our source signal.
%Data was obtained from a sleep laboratory, where 75 patients were recorded and 200 1 minute long sequences were extracted.
In this case, we observe all models using variations of $\EMD$ gradients are capable of learning the transformation significantly faster than the $\MSE$ (fraction of the first epoch).
}
\label{fig:resultsD}
\end{figure}


==> proof.tex <==
%!TEX root = cvpr2017A.tex

\newtheorem{theorem}{Proposition}
%{\color{red}You mean proposition right? Also, https://en.wikipedia.org/wiki/Theorem\#Terminology}

%{\color{red}what values?} 
However, a tree structured graph, with undefined root, does not define a unique parent-child relationship.
Therefore, there is no unique way in which the $\tEMD$ distance can be defined for a given tree.
However, we show that $\tEMD^\rho$ and its gradient are uniquely defined for a given tree.

%{\color{red}what happens if the leaf is chosen as the root? or can't that be done? doesn't that change which nodes are measured as bins and twist the whole concept around?}
\begin{theorem}
Let $T'$ and $T$ be two identical trees with different nodes selected as root.
Then, the $\tEMD^\rho$ between any two distributions is identical:
\[\tEMD^\rho_{T'}(\mathbf{p},\mathbf{q})=\tEMD^\rho_T(\mathbf{p},\mathbf{q}).\]
\end{theorem}
%{\color{red}regularized? or relaxed?}

\begin{proof}
Let $T$ and $T'$ be two trees with nodes~$G$ and transportation cost function~$\tilde{M}:G \rightarrow \mathbb{R}^+$.
As the $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1$, the excess of dirt arriving at the root nodes~$\tilde{\varphi}_{r_0} = \tilde{\varphi}_{r_1} = 0$.
We prove that our proposition holds for the case where, in $T$, $r_0$ is the parent of $r_1$, as a consequence, this proves by induction that our proposition is correct for every two root nodes.
%{\color{red}hm.. the grammar on the above sentence. What does directly connected mean? }
% Inductively, we can extend our proof it to any tree.

%Since $r_0$ is the parent of $r_1$, then $r_1$ is the immediate child of the root: $r_1 \in p(r_0)$ in $T'$.


\begin{figure}[t]
  \centering
  \subfloat[$T$]{\includegraphics[width=3cm]{figures/trie1-crop}}\hspace{1cm}
  \subfloat[$T'$]{\includegraphics[width=3cm]{figures/trie2-crop.pdf}}
  \caption{Example trees with different roots.}
  \label{fig:proof_trees}
\end{figure}




% First, we prove that our assumption is true in the case that in $T'$ the node $r_1$ is the immediate child of the root:~$r_1 \in p(r_0)$~(see Figure~\ref{fig:proof_trees}).
Without any loss of generality, we group all other children nodes of $r_0$ in $T'$ in the subtree $S_0$, while the nodes that span from~$r_1$ we define as~$S_1$~(see \figref{proof_trees}).
We define $c:G \rightarrow \mathbb{R}^+$ the cost of node $i$: $c(i)=M_{i, p(i)}...$.
%In the case of $T$ we obtain $S_0$ and $S_1$ as shown by \figref{proof_trees}.
% The subtrees $S_0$ and $S_1$ are identical in both trees in the sense that the excess dirt and transportation cost are equal.
The cost~$c'$ of the first tree $T'$ and the cost $c$ of the second tree $T$ are equal for all nodes in the subtrees~$S_0$ and $S_1$: \[c'(i)=c(i), \forall i \in S_0\cup S_1.\]
Thus, we are only left to prove that the sum of the costs of the nodes~$r_0$ and~$r_1$ in~$T$ and~$T'$ are identical.
The excess dirt of~$r_0$ in~$T$ is equal to:
\[\tilde{\varphi}(r_0) = \tilde{\varphi}'(r_0) - \tilde{\varphi}'(r_1). \]
In the same way we are able to compute the excess in $r_1$ of $T_1$:
{\color{red}what's $T_1$?}
\[\tilde{\varphi}(r_1) = \tilde{\varphi}(r_0) + \tilde{\varphi}'(r_1). \]
Since $\phi'(r_0)=0$ and $\phi(r_1)=0$, we are able to simplify both equations to:
{\color{red}Ehm.. don't you mean $\tilde{\varphi}_{r_0} = 0$ and $\tilde{\varphi}_{r_1} = 0$?}
\[\tilde{\varphi}(r_0) = - \tilde{\varphi}'(r_1), \]
and obtain
\[ |\tilde{\varphi}(r_0)| = |\tilde{\varphi}'(r_1)|. \]

As we have an undirected graph: $M_{i, j} = M_{j, i}, \forall i,j\in G$, we obtain $c(i)+c(j) = c'(j)+c'(i)$.
Since the distance function is the sum of all costs, we obtain $\tEMD'=\tEMD$.
Finally, this shows that the distance function does not depend on the ordering of the nodes in the tree.
\end{proof}

{\color{red}This proof is rife with inaccuracies for math. Too many notational confusions too between $T$ and $T'$ and so on. I think it would be best to skip it and include in supplementary material. Otherwise, this needs much work tomorrow.}
{\color{blue}Z: +1}
% More precisely, we prove that choosing different roots does not change the outcome of our distance function~$SMD$.
% Since the order depends on the root choice, we prove that the distance function between any distributions $p$ and $g$ is not dependent on the root choice.


==> proof2.tex <==
%!TEX root = cvpr2017A_supplement.tex

\section{$\tEMD^\rho$ does not depend on selecting a particular node as a root}

\newtheorem{theorem}{Proposition}
A tree structured graph does not generally define the parent-child relationship between nodes.
As the $\tEMD^\rho$ definition is based on the parent-child relationship, there are multiple ways in which the $\tEMD^\rho$ can be calculated for a given tree.
However, we prove that $\tEMD^\rho$ and by extension, its gradient, is uniquely defined for a given tree.

\begin{theorem}
Let $A$ and $B$ be two identical undirected trees with different nodes selected as root.
Then, the $\tEMD^\rho$ between two distributions $\mathbf{p}$ and $\mathbf{q}$, is identical:
\[\tEMD^\rho_{A}(\mathbf{p},\mathbf{q})=\tEMD^\rho_{B}(\mathbf{p},\mathbf{q}).\]
\end{theorem}
%{\color{red}regularized? or relaxed?}

\begin{proof}
%{\color{red}define p, q}
Let $\mathbf{p}$ and $\mathbf{q}$ be two distributions with $\norm{\mathbf{p}}_1 = \norm{\mathbf{q}}_1 = 1$.
Let $A$ and $B$ be two undirected trees with nodes~$G$ and transportation cost function~$M:G \rightarrow \mathbb{R}^+$.
Let $n_0$ be the root node of $A$ and $n_1$ be the root node of $B$.
We prove that our proposition holds for the case where $n_0$ is adjacent to $n_1$.
As a consequence, this proves by induction that our proposition is correct for every two root nodes.

\begin{figure}[h]
  \centering
  \subfloat[$A$]{\includegraphics[width=3cm]{figures/t0-n0-crop.pdf}}\hspace{1cm}
  \subfloat[$B$]{\includegraphics[width=3cm]{figures/t1-n1-crop.pdf}}
  \caption{Identical trees $A$ and $B$ with different root nodes.
  $S_0$ and $S_1$ represent a bunch of nodes and corresponding subtrees connected to $n_0$ and $n_1$ respectively.}
  \label{fig:proof_trees}
\end{figure}

We first simplify the tree structure~(see \figref{proof_trees}).
Without any loss of generality, we group all adjacent nodes of $n_0$ except $n_1$ as a virtual subtree $S_0$ with $M_{S_0,n_0}$ as the virtual transportation cost function from $S_0$ to $n_0$.
Similarly, we group the adjacent nodes of $n_1$ except $n_0$ as $S_1$.

In this setting we have:
\begin{eqnarray}
\tEMD_{A}^\rho(\mathbf{p}, \mathbf{q}) &=& M_{S_0,n_0} | \tilde{\varphi}^{A}_{S_0} |^\rho + M_{S_1,n_1} | \tilde{\varphi}^{A}_{S_1} |^\rho + M_{n_1,n_0} | \tilde{\varphi}^{A}_{n_1} |^\rho \, , \text{and} \\
\tEMD_{B}^\rho(\mathbf{p}, \mathbf{q}) &=& M_{S_0,n_0} | \tilde{\varphi}^{B}_{S_0} |^\rho + M_{S_1,n_1} | \tilde{\varphi}^{B}_{S_1} |^\rho + M_{n_0,n_1} | \tilde{\varphi}^{B}_{n_0} |^\rho \, .
\end{eqnarray}

%{\color{red}rephrase .. :)}
As $S_0$ and $S_1$ are identical in both trees, $\tilde{\varphi}^{A}_{S_0}=\tilde{\varphi}^{B}_{S_0}$ and $\tilde{\varphi}^{A}_{S_1}=\tilde{\varphi}^{B}_{S_1}$.
Therefore, the difference of $\tEMD^\rho$ between $A$ and $B$ is:
\begin{equation}
\tEMD_{A}^\rho(\mathbf{p}, \mathbf{q}) - \tEMD_{B}^\rho(\mathbf{p}, \mathbf{q}) =
M_{n_1,n_0} | \tilde{\varphi}^{A}_{n_1} |^\rho -
M_{n_0,n_1} | \tilde{\varphi}^{B}_{n_0} |^\rho
 \, .
\end{equation}

Furthermore, $M_{n_1,n_0}$ and $M_{n_0,n_1}$ refer to the same edge, and as the graph is undirected, they are equal.
Thus, to prove $\tEMD_{A}^\rho(\mathbf{p}, \mathbf{q}) = \tEMD_{B}^\rho(\mathbf{p}, \mathbf{q})$ we only need to show that $| \tilde{\varphi}^{A}_{n_1} |^\rho = | \tilde{\varphi}^{B}_{n_0} |^\rho$.

%{\color{red}please explain? :)}


%$\tilde{\varphi}$ is the sum of all


If $n_0$ is a leaf node of the tree, then $\tilde{\varphi}^{B}_{n_0} = p_0 - q_0$ and $S_0$ is empty.
On the other hand, if $n_0$ is an intermediate node, then $\tilde{\varphi}^{B}_{n_0} = \tilde{\varphi}^{B}_{S_0}$ as $\mathbf{p}$ and $\mathbf{q}$ are not defined on non-leaf nodes.
To cope with both cases, we define $\tilde{\varphi}^{B}_{n_0}$ as follows:
\begin{eqnarray}
%\tilde{\varphi}^{A}_{n_1}  &=& p_1 - q_1 + \tilde{\varphi}^{A}_{S_1} \, , \\
\tilde{\varphi}^{B}_{n_0}  &=& p_0 - q_0 + \tilde{\varphi}^{B}_{S_0} \, ,
\end{eqnarray}
and equivalently
\begin{eqnarray}
\tilde{\varphi}^{A}_{n_0}  &=& p_0 - q_0 + \tilde{\varphi}^{A}_{S_0} + \tilde{\varphi}^{A}_{n_1} \, .
\end{eqnarray}

As before, since the trees identical, $\tilde{\varphi}^{A}_{S_0} = \tilde{\varphi}^{B}_{S_0}$.
This gives
\begin{eqnarray}
\tilde{\varphi}^{A}_{n_0}  &=& \tilde{\varphi}^{B}_{n_0} + \tilde{\varphi}^{A}_{n_1} \, , 
\label{eq:good}
\end{eqnarray}

Finally, as $\mathbf{p}, \mathbf{q} \in \mathbb{R}^+$ and have the same $\ell_1$ norm, we know that $\tilde{\varphi}$ is zero for any root node (as $\tilde{\varphi}$ is the sum of differences of all children, and the total amount of \emph{dirt} is the same).
In this case, since $n_0$ is the root of $A$, $\tilde{\varphi}^{A}_{n_0} = 0$.
Applied to \equref{good}, we show that $\tilde{\varphi}^{A}_{n_1}  = -\tilde{\varphi}^{B}_{n_0}$, and $| \tilde{\varphi}^{A}_{n_1} |^\rho = | \tilde{\varphi}^{B}_{n_0} |^\rho$ follows.
Thus, $\tEMD^\rho_{A}(\mathbf{p},\mathbf{q})=\tEMD^\rho_{B}(\mathbf{p},\mathbf{q})$.

\end{proof}






%%\begin{equation}
%%\tEMD_{T'}^\rho(\mathbf{p}, \mathbf{q}) = $\tilde{M}_{S_0} | \tilde{\varphi}_{S_0} |^\rho + $\tilde{M}_{S_1} | \tilde{\varphi}_{S_1} |^\rho + $\tilde{M}_{n_0} | \tilde{\varphi}_{n_0} |^\rho \, .
%%\end{equation}



%Then, $S_0$ and $S_1$ are equal in both trees, so 





%We define $c:G \rightarrow \mathbb{R}^+$ the cost of node $i$: $c(i)=M_{i, p(i)}...$.
%%In the case of $A$ we obtain $S_0$ and $S_1$ as shown by \figref{proof_trees}.
%% The subtrees $S_0$ and $S_1$ are identical in both trees in the sense that the excess dirt and transportation cost are equal.
%The cost~$c'$ of the first tree $T'$ and the cost $c$ of the second tree $A$ are equal for all nodes in the subtrees~$S_0$ and $S_1$: \[c'(i)=c(i), \forall i \in S_0\cup S_1.\]
%Thus, we are only left to prove that the sum of the costs of the nodes~$r_0$ and~$r_1$ in~$T$ and~$T'$ are identical.
%The excess dirt of~$r_0$ in~$T$ is equal to:
%\[\tilde{\varphi}(r_0) = \tilde{\varphi}'(r_0) - \tilde{\varphi}'(r_1). \]
%In the same way we are able to compute the excess in $r_1$ of $T_1$:
%{\color{red}what's $T_1$?}
%\[\tilde{\varphi}(r_1) = \tilde{\varphi}(r_0) + \tilde{\varphi}'(r_1). \]
%Since $\phi'(r_0)=0$ and $\phi(r_1)=0$, we are able to simplify both equations to:
%{\color{red}Ehm.. don't you mean $\tilde{\varphi}_{r_0} = 0$ and $\tilde{\varphi}_{r_1} = 0$?}
%\[\tilde{\varphi}(r_0) = - \tilde{\varphi}'(r_1), \]
%and obtain
%\[ |\tilde{\varphi}(r_0)| = |\tilde{\varphi}'(r_1)|. \]

%As we have an undirected graph: $M_{i, j} = M_{j, i}, \forall i,j\in G$, we obtain $c(i)+c(j) = c'(j)+c'(i)$.
%Since the distance function is the sum of all costs, we obtain $\tEMD'=\tEMD$.
%Finally, this shows that the distance function does not depend on the ordering of the nodes in the tree.

%{\color{red}This proof is rife with inaccuracies for math. Too many notational confusions too between $A$ and $T'$ and so on. I think it would be best to skip it and include in supplementary material. Otherwise, this needs much work tomorrow.}

%% More precisely, we prove that choosing different roots does not change the outcome of our distance function~$SMD$.
%% Since the order depends on the root choice, we prove that the distance function between any distributions $p$ and $g$ is not dependent on the root choice.


==> results/experimentPSD_train.tex <==
\addplot+[line width=2pt, mark=none] coordinates { (1,6.963051975538) (2,8.8785478301405) (3,6.6729162360428) (4,8.0767096902172) (5,6.9503177972023) (6,7.7621147048712) (7,7.411031165489) (8,8.3353900312781) (9,7.3650100170943) (10,6.3659292551694) (11,8.4896779121224) (12,7.9231143576761) (13,7.6013609851237) (14,6.4211802914021) (15,6.803304433179) (16,8.5454430484977) (17,4.9835375135765) (18,7.0895160617286) (19,6.9299974272436) (20,8.0188992739849) (21,6.8548905917396) (22,8.7027575978393) (23,6.9845556253891) (24,10.100267163251) (25,6.239221825013) (26,6.6774964813324) (27,7.8244096901959) (28,7.4998016879743) (29,6.4417923778547) (30,6.5541794626509) (31,7.0142827009081) (32,6.7849144721662) (33,6.5380263160762) (34,8.2171673398926) (35,6.8035274409389) (36,7.274742645969) (37,6.0989780192975) (38,8.4791450730418) (39,6.9901451937675) (40,7.6981054503784) (41,7.1069791062137) (42,5.8115124561234) (43,9.0831249695579) (44,6.0210334265414) (45,7.2480008590222) (46,6.5115682435895) (47,9.4729817538603) (48,7.2947516705048) (49,8.0442157155473) (50,5.6769240396143) (51,8.5821197896828) (52,7.2397913452476) (53,5.2425827667545) (54,6.0148660290517) (55,6.0058604155326) (56,5.228064271666) (57,7.3367009077755) (58,5.001561502412) (59,8.0141616797793) (60,6.866805551428) (61,7.2225963395425) (62,6.6113966789718) (63,6.4445727707981) (64,6.3771837916264) (65,6.8780095508176) (66,6.5508432573287) (67,7.7184632053641) (68,8.3222934718182) (69,5.2119211257221) (70,5.6282749275728) (71,6.1127333530929) (72,5.5810652832091) (73,6.7780397043712) (74,5.6801821575784) (75,7.9339359534164) (76,5.9101183429178) (77,4.1862215680565) (78,8.2745905125177) (79,4.2556351590555) (80,6.6766939483428) (81,6.8271759739874) (82,6.0012504725512) (83,4.6135977692947) (84,5.4336727991776) (85,5.2121463133009) (86,5.6292168717912) (87,6.7886057552361) (88,5.3728884926988) (89,5.8966675257966) (90,7.8214628603573) (91,5.4463455048348) (92,5.6955477063989) (93,6.4309945978794) (94,4.8951493534372) (95,6.6872435610892) (96,5.7637435908436) (97,6.9357997569936) (98,6.0141517278812) (99,6.2934332668774) (100,5.0017990767139) (101,6.6501157519354) (102,5.2717323544357) (103,6.0419480852431) (104,4.3632752817436) (105,7.96821585164) (106,5.3450498363153) (107,7.3264703155286) (108,4.4338513185998) (109,7.300613866181) (110,4.7506809623827) (111,5.226014333591) (112,5.2353751803116) (113,4.3694843534454) (114,3.4330711949394) (115,5.5817008260276) (116,7.6992565537659) (117,5.3089698340707) (118,7.4787288473063) (119,5.9007179152184) (120,7.0451993998021) (121,4.3004722354665) (122,2.6358672530357) (123,6.7406714525121) (124,4.0095204266473) (125,4.5661329719949) (126,4.2967712316714) (127,6.0804682648956) (128,5.4763725441066) (129,6.8418470017139) (130,6.081599883699) (131,3.9630571812937) (132,3.6417810007945) (133,5.3148411571162) (134,3.2951976756653) (135,5.4568713210654) (136,3.2250413333431) (137,3.8189353833649) (138,2.5626902613102) (139,4.6249318217247) (140,3.8998920608297) (141,5.0724601415861) (142,3.8646279131352) (143,3.7106689692442) (144,3.375177219507) (145,4.4289040039399) (146,4.9624328841045) (147,4.2754657971221) (148,4.8218122125905) (149,4.0133715039085) (150,3.2706928673849) (151,5.6982876137879) (152,4.6079618824722) (153,5.3586500182214) (154,3.8132710379025) (155,3.27674254185) (156,3.4038141453926) (157,3.8503730821529) (158,3.8804495514647) (159,4.8764617588544) (160,3.820970520897) (161,3.2283903361937) (162,3.7870562287832) (163,3.275586011288) (164,3.0506676297751) (165,3.7513316512713) (166,5.7187045764631) (167,3.136795595348) (168,5.9928599795614) (169,3.1454962645739) (170,4.1109094364584) (171,2.7627854363015) (172,4.1530180779723) (173,3.0976804978736) (174,5.7669261187546) (175,3.4752285531173) (176,3.7915418604319) (177,3.7160869984454) (178,3.7726973851394) (179,2.7396617726184) (180,2.9615168887321) (181,4.1779055782493) (182,4.0246814453246) (183,2.8222455503235) (184,4.7480759309625) (185,3.3271715950661) (186,6.2100545749642) (187,3.4390570521051) (188,3.2849629959871) (189,3.9148685620548) (190,3.8941277037655) (191,4.3113563515371) (192,3.0125627973537) (193,4.0305987652172) (194,3.8444294552355) (195,3.3581954724417) (196,3.2291222315032) (197,3.3430995708756) (198,3.6654299873507) (199,3.457370183903) (200,2.8403356731356) (201,3.012929851677) (202,2.4642872915382) (203,1.9866153681055) (204,4.9171072304522) (205,3.0437127901202) (206,3.2891263298792) (207,3.8806295941239) (208,3.0228668181534) (209,2.852135281037) (210,3.8444853605711) (211,2.5537648483617) (212,2.6132122476025) (213,3.2640790983993) (214,2.6532447636243) (215,2.3000734743269) (216,2.6192095332638) (217,3.0120479996946) (218,3.1721801881038) (219,2.9720200943048) (220,3.1152944347188) (221,2.8411463581469) (222,2.5994511925413) (223,3.656768775414) (224,2.0805527737707) (225,2.4420249975825) (226,2.2627631859675) (227,3.1714688584664) (228,2.9234990288363) (229,2.7266136727979) (230,3.7595204727383) (231,2.4839758749108) (232,2.2213485392914) (233,2.8967239795011) (234,3.6528680234197) (235,2.7133365186529) (236,2.9791377689535) (237,2.3032058495103) (238,2.7268436881212) (239,2.4469638371566) (240,2.1386264004726) (241,3.2582813342922) (242,2.5060275886313) (243,3.5007314164705) (244,2.5430187167967) (245,3.2868500220679) (246,3.0571060244565) (247,2.6599170336843) (248,3.0956858842551) (249,2.1577299533781) (250,3.0763141264383) (251,2.4069730353317) (252,2.9974646831079) (253,3.2974824813066) (254,2.602404669684) (255,2.9731277009497) (256,2.1649805694949) (257,2.2139919013885) (258,2.7149892607266) (259,3.1810055064925) (260,3.0298290575695) (261,2.8470149939539) (262,3.3030352435587) (263,2.8091527532302) (264,3.3997900562702) (265,4.5146511007197) (266,2.6781361183786) (267,3.4628555285012) (268,2.5593134799029) (269,3.0296583074964) (270,2.5081302806269) (271,2.1725862144575) (272,2.6511009950646) (273,2.7279181617151) (274,2.6453394837011) (275,4.0123235211386) (276,3.8307346950825) (277,2.6371639575672) (278,3.173410315301) (279,3.0629017233245) (280,3.2587590974747) (281,3.7041260496508) (282,2.8957405258064) (283,2.5520906781436) (284,2.7716405309514) (285,2.7047071083234) (286,2.1987140060896) (287,3.3113476599573) (288,2.5073145529896) (289,2.8232875771936) (290,2.8478992919127) (291,2.4085127611856) (292,2.3414364315133) (293,2.8985611754462) (294,1.9233184159027) (295,3.4062850417166) (296,2.0878672592239) (297,2.3530083534507) (298,2.6486812011323) (299,2.1219934920416) (300,2.9973312555931) (301,2.4112198793792) (302,2.6017764262274) (303,1.9657789703663) (304,2.9343243158782) (305,2.23697501707) (306,2.4747168366311) (307,2.5280005963141) (308,2.4014751219778) (309,2.4036972340896) (310,3.1912812318227) (311,2.9975083622898) (312,2.5946545292634) (313,2.6752583336319) (314,2.4815812224394) (315,2.4327749713078) (316,2.6229475434857) (317,2.6006097138272) (318,1.9324496839951) (319,2.5410441182944) (320,2.768114342648) (321,2.3048528929529) (322,2.3626531632198) (323,2.0055616891302) (324,2.274062254851) (325,2.2445510289411) (326,2.2236668155412) (327,2.6760627859639) (328,2.5636595135435) (329,2.688094465533) (330,2.2736172771865) (331,2.4192515899947) (332,2.4293231525626) (333,2.7016037226992) (334,2.8227745068996) (335,2.0997919942309) (336,2.5606275361024) (337,2.4821695067974) (338,2.5762247105415) (339,2.4856015508024) (340,3.1082160186217) (341,2.0364091288937) (342,2.0685732835561) (343,2.6048232776744) (344,1.7196630292696) (345,2.2404902199373) (346,2.3180505308456) (347,2.1913029323649) (348,2.3428955261007) (349,2.2369283803261) (350,1.8971972000569) (351,3.1965106328594) (352,2.3226751396994) (353,2.0102223720766) (354,2.3706886766625) (355,1.9335608219655) (356,2.3111919620308) (357,2.6289656410518) (358,1.8624424538524) (359,1.7155486490664) (360,1.9082356703131) (361,2.4651289654572) (362,2.4663934348481) (363,2.2548197309215) (364,2.1162682904016) (365,2.5265182275111) (366,2.3773805550881) (367,2.6777722808047) (368,2.46305773137) (369,2.1358883370155) (370,2.006480171606) (371,2.2831100789438) (372,2.0690088437448) (373,1.7456158559776) (374,2.1986446599038) (375,2.5355125090992) (376,2.3746997323727) (377,2.0869423561619) (378,1.7475217921764) (379,2.4606644616478) (380,2.0976792788335) (381,2.0495042434337) (382,2.5673754877405) (383,2.4278985380756) (384,2.1863488674342) (385,1.9914475723049) (386,2.1549435658368) (387,2.1063385601696) (388,2.0257588330094) (389,2.1721604032062) (390,2.2674181572566) (391,2.1720454735564) (392,2.0901525897752) (393,1.9044787534372) (394,2.3203937757799) (395,1.7600840495998) (396,2.5036219001561) (397,2.3262181498454) (398,2.3618220430398) (399,2.5031474429008) (400,2.0536660212954) (401,2.0331028127779) (402,2.0888030414543) (403,2.0909427996732) (404,2.2822463717209) (405,1.9445765706336) (406,2.058685952086) (407,1.8523046310299) (408,2.3201490002515) (409,1.9999550813261) (410,2.0466152378023) (411,2.2732521090925) (412,1.9104132779705) (413,1.7897811818915) (414,2.6520750279707) (415,2.1071156870382) (416,1.9899663489366) (417,2.1599634525752) (418,1.9482039080256) (419,2.1864361812174) (420,1.758203503725) (421,2.0004805952075) (422,1.6795839195998) (423,1.9719314589714) (424,2.1795441080363) (425,2.0665491798318) (426,2.0282521088274) (427,2.222986797775) (428,2.1170996597499) (429,2.0215650427902) (430,2.3782943845801) (431,2.2625117335163) (432,2.1383444494227) (433,2.0368527354327) (434,1.9649073472288) (435,2.3346945358024) (436,1.8106059946063) (437,2.1291167407625) (438,2.1192800900619) (439,2.0738226841289) (440,2.156700624046) (441,2.0307794833989) (442,2.1525448584166) (443,1.9871636334815) (444,2.3798724312733) (445,1.6079271482109) (446,1.9080001579796) (447,2.2855935421441) (448,2.0025130334781) (449,2.5723464816885) (450,2.1888813849117) (451,1.9687754045256) (452,2.2055386403447) (453,2.1650066309109) (454,2.0943097003029) (455,1.845326144652) (456,2.2741264463573) (457,1.9441323990766) (458,1.6106531982366) (459,2.5966148349222) (460,2.8192793880681) (461,2.3156361244615) (462,2.2081238376529) (463,2.5926199509626) (464,2.2094692186331) (465,2.0596400148203) (466,2.1083609609657) (467,1.9439884634088) (468,1.9979702370951) (469,2.2312464067587) (470,2.1946575103745) (471,2.0759456555203) (472,2.4148882872644) (473,2.1214887505846) (474,1.8465872314052) (475,1.8977028466493) (476,1.7083211677818) (477,2.0630817333315) (478,2.3201727829281) (479,1.8407181984481) (480,2.2386482027074) (481,1.9262312849059) (482,2.6961123232082) (483,1.7137288771147) (484,1.8901833668701) (485,1.7936141754947) (486,1.9459375132865) (487,1.9309875062174) (488,1.8591109081078) (489,1.9068600140912) (490,2.3172574014468) (491,2.3718402218381) (492,2.1377753590873) (493,2.0742083746755) (494,2.3968185226527) (495,2.106475397132) (496,2.1194702269016) (497,2.1378389360874) (498,2.1115443471853) (499,1.7088935908113) (500,2.0714809173522) (501,1.7168211305198) (502,2.0469641786681) (503,1.9359250598169) (504,2.0267625763565) (505,2.1845143428812) (506,1.8634659352256) (507,2.0371538468642) (508,1.903190864577) (509,2.3096854115734) (510,2.3979991812795) (511,1.9249707934186) (512,2.122827238217) (513,2.206225191375) (514,1.9713546592083) (515,2.3374583476444) (516,2.1488303751922) (517,2.632544413982) (518,2.2720808437286) (519,2.0354135315124) (520,2.4863855852567) (521,2.1665243649039) (522,2.3607694939108) (523,1.7372598679871) (524,2.5012764064155) (525,1.9329180926571) (526,2.3095155890314) (527,2.1325528528727) (528,1.9886359385285) (529,2.0104075869091) (530,2.7103077837357) (531,2.3440710511398) (532,1.9726605545847) (533,1.6779595087125) (534,1.9699856124277) (535,2.1072321826456) (536,2.2853117820959) (537,2.4532422251749) (538,2.3140709837725) (539,2.2935297487519) (540,2.0364175474754) (541,1.9847080527335) (542,2.0443042896724) (543,1.8540832470342) (544,2.2634834574513) (545,2.2432575552479) (546,2.0489269339545) (547,2.586444331211) (548,2.1807904131996) (549,2.033179551495) (550,1.7194281335194) (551,2.0498607374474) (552,2.1587927040237) (553,2.0990297447775) (554,2.3112325741481) (555,1.9181199755124) (556,1.9155456262251) (557,1.7613147393128) (558,1.9736535375225) (559,2.2275145852978) (560,2.18292753979) (561,2.285138897494) (562,2.7100114410578) (563,2.236830916921) (564,2.3180212200535) (565,1.8234968873952) (566,2.2807124449037) (567,2.256479055032) (568,2.3512862220817) (569,1.7926936712391) (570,2.2403255063439) (571,2.4739066031779) (572,2.0733436217278) (573,1.7959918217055) (574,2.4226964832964) (575,2.2619262233122) (576,2.1641477363793) (577,1.5931099400827) (578,1.8815176839892) (579,1.604348521159) (580,2.2297972515795) (581,1.7839461779592) (582,2.0862740269769) (583,2.1459907567015) (584,2.3798081419817) (585,2.2949941156754) (586,2.3294570101996) (587,2.5003455476425) (588,2.6552456733845) (589,1.9660280254155) (590,2.0509685640675) (591,1.7973937598135) (592,2.2104247049548) (593,1.9088918292876) (594,1.9885913168477) (595,2.0970351349506) (596,2.2761830084081) (597,1.8985330667597) (598,2.055916190269) (599,2.2084683789215) (600,2.2218069943807) (601,2.5080669628262) (602,1.7382180325094) (603,2.3385955327912) (604,1.5466276194861) (605,2.0833568314639) (606,1.7882488588247) (607,2.2921871265742) (608,2.6276406820541) (609,2.070043462366) (610,1.8175979263671) (611,2.1331638292729) (612,1.6241154478737) (613,2.1447071738462) (614,2.0237320592134) (615,1.6865295838325) (616,2.3285689216204) (617,2.1897095749061) (618,1.872915375577) (619,2.1488235938215) (620,2.1614980744411) (621,1.8869610726256) (622,1.9231307938959) (623,2.1153677273347) (624,2.4955361603471) (625,1.7141806098875) (626,1.7940443061515) (627,2.1280497511415) (628,1.8987514724812) (629,1.9386867012677) (630,1.8254339824138) (631,2.2945932537284) (632,2.2753850317862) (633,2.4257328701548) (634,1.9247805077247) (635,2.3378534409678) (636,1.9834346778615) (637,2.2759417075514) (638,2.6232454081897) (639,2.4550214767531) (640,2.3998120064946) (641,2.5581814770036) (642,1.8313015252476) (643,2.3402656197918) (644,1.9503024460197) (645,1.9327990688293) (646,2.0231120407739) (647,2.8798957581019) (648,1.9068173374216) (649,2.0182565809209) (650,1.8559538776057) (651,2.4922291275965) (652,1.9238820492778) (653,2.2856432218253) (654,1.8721408577531) (655,2.0249495978218) (656,2.5049508285901) (657,1.8518283923819) (658,2.3553856909678) (659,1.8416961500934) (660,2.0767040721621) (661,1.9959362596802) (662,2.0664002594177) (663,1.857850306559) (664,1.7309257110154) (665,2.0206121308972) (666,1.9865452236589) (667,1.9050801261476) (668,2.4222373627667) (669,2.2873626147453) (670,1.6789679466183) (671,2.0436174403008) (672,1.7743142860691) (673,1.6961860226359) (674,1.7825141108514) (675,2.1111701413897) (676,1.9533012676117) (677,2.3367574799549) (678,2.0358721566243) (679,1.917756138525) (680,2.0413854913936) (681,1.9988780639925) (682,2.2272878472226) (683,1.8857713819414) (684,2.2945183408528) (685,1.955322743052) (686,1.6166096843948) (687,1.7565263586043) (688,2.3560392197161) (689,2.0542193336987) (690,1.8533505830769) (691,2.2460587935038) (692,2.1307305293268) (693,1.7804578849315) (694,2.0701911459474) (695,2.0368959246419) (696,2.0968218840293) (697,2.1320162762376) (698,1.8729076583367) (699,2.2919817358186) (700,2.5364047434434) (701,2.3395337623455) (702,2.0268994084263) (703,1.7653161413375) (704,1.7958933026535) (705,1.950876403975) (706,1.7603524155642) (707,2.056524113542) (708,2.082608704242) (709,1.9339206574113) (710,2.1574932815267) (711,2.0334761258251) (712,1.7646334751123) (713,1.7583829919991) (714,2.5300918577371) (715,2.3181285488967) (716,1.8942628225794) (717,1.9297393710896) (718,1.9605694235812) (719,2.0790895711644) (720,2.2715797543422) (721,1.8636356748668) (722,2.3462841200537) (723,2.2042764448092) (724,1.7997840682509) (725,2.1212819355963) (726,2.3056797259301) (727,1.9277670755635) (728,2.5968382769155) (729,1.9027422472078) (730,1.9780767158498) (731,1.9320481685643) (732,2.1015311542553) (733,2.0345030433678) (734,2.107119778052) (735,2.4020035183484) (736,1.8690915791965) (737,1.8249992005575) (738,2.3391584946258) (739,1.9447093042808) (740,2.3175252113964) (741,1.6372041423054) (742,1.8481183884585) (743,1.8239971918652) (744,2.254509503713) (745,2.8007888995896) (746,2.5147757553227) (747,2.2381499274059) (748,2.6076119848983) (749,2.240978730733) (750,2.035957773577) (751,2.1613156153309) (752,2.1102729436694) (753,2.1003069210518) (754,2.2459247692734) (755,2.3578848394905) (756,2.1996840654518) (757,2.030244601687) (758,2.4688206880186) (759,1.7451960466865) (760,1.9474927897385) (761,1.9163170810766) (762,1.9539715442097) (763,1.8644691468093) (764,2.0313106026956) (765,2.3018497963658) (766,2.5046219892505) (767,2.0645389968565) (768,2.4067330828788) (769,2.6918147379937) (770,2.1999339369489) (771,1.8605884249661) (772,1.9231863114712) (773,2.2869345257531) (774,1.9149737061935) (775,2.0116990663062) (776,1.9581070062651) (777,2.0216580056956) (778,1.8355956640184) (779,2.2305878224682) (780,2.0062702841302) (781,2.2009234044519) (782,1.9653920516018) (783,2.1823514851056) (784,1.891562124951) (785,1.5244895559507) (786,1.7733729102685) (787,1.9880001954554) (788,1.4603457876113) (789,1.9905727566649) (790,1.8557099395311) (791,2.2689062434381) (792,1.8524110840507) (793,2.2851931813013) (794,2.812570111164) (795,2.3865404177096) (796,1.8614039378048) (797,1.9062804360466) (798,2.2814222155354) (799,1.8406923109408) (800,1.7339425785175) (801,1.8212103891441) (802,1.9710438633593) (803,2.0020810173042) (804,2.1505680278526) (805,2.3712181242924) (806,2.6760630857727) (807,1.9967328639257) (808,1.947561604334) (809,2.1689127479834) (810,2.3186629288036) (811,1.722024007925) (812,2.132877765506) (813,2.3375885042173) (814,1.8969373203637) (815,2.233919621365) (816,1.8345487039547) (817,1.4981696013053) (818,2.2123310796667) (819,2.0371917142041) (820,2.2040219167489) (821,2.3009318023664) (822,2.1585643705729) (823,2.1637227155988) (824,2.1101136719816) (825,1.8952418759425) (826,2.1688939541127) (827,1.9942526450649) (828,1.975392060444) (829,1.7765508298404) (830,1.5803042378537) (831,2.2403714053771) (832,1.7316109148399) (833,2.3472372709187) (834,1.9833958299629) (835,2.2787374815998) (836,2.0754476336952) (837,1.6486887413739) (838,1.9510028763164) (839,2.318115908318) (840,2.2620853115476) (841,2.0228258517476) (842,2.1864289289117) (843,2.0750675679257) (844,1.73143943978) (845,1.7813050159216) (846,1.7042185620577) (847,1.8570614723166) (848,1.9581232427958) (849,2.0981596102883) (850,1.8911460434843) (851,1.6240973182709) (852,1.9573608852588) (853,1.980872102864) (854,1.8765394069855) (855,1.6343183163114) (856,1.9519363528768) (857,2.0339709934363) (858,1.7231247135146) (859,1.6873633474097) (860,2.2245473281251) (861,1.7490575315448) (862,1.89393025103) (863,1.9792438568647) (864,2.6467741099645) (865,1.8942572617808) (866,1.6858639060305) (867,1.9044160027439) (868,2.0627472957861) (869,1.7708023412371) (870,2.1258644704401) (871,1.7108926760438) (872,1.7409631590517) (873,2.0546368616892) (874,1.9302373419044) (875,2.1568293012908) (876,1.77101393784) (877,1.8754730223044) (878,2.3826059663899) (879,2.0611932515374) (880,1.8312558056657) (881,1.7100035196294) (882,1.8686762270325) (883,1.9283769347005) (884,1.8514881134887) (885,1.4724221638957) (886,1.8614486045878) (887,2.5087767722156) (888,1.9031208129957) (889,1.9328206750395) (890,1.8816486474975) (891,1.5311676403138) (892,1.8072974913309) (893,1.5943534697927) (894,2.0194003064793) (895,2.0757636093721) (896,2.0652631457017) (897,2.3814128845037) (898,2.1569882771656) (899,1.9057668769281) (900,1.6166210238199) (901,2.1108625242082) (902,1.9139248843638) (903,1.7640882180479) (904,2.0195971772111) (905,1.6837703639975) (906,2.086806868693) (907,2.0160204857984) (908,1.6823955779477) (909,2.0518037576461) (910,2.2218628477792) (911,2.0012289607369) (912,2.1181463429816) (913,1.9801151307283) (914,1.5524716438453) (915,1.7067483143803) (916,1.9638672388749) (917,1.8840052798638) (918,2.0744145214881) (919,1.9004820073787) (920,1.873184055008) (921,2.4406586365955) (922,1.6778424814526) (923,1.8968252816521) (924,2.311110404669) (925,1.7288525732348) (926,2.2318897827615) (927,2.1717861576812) (928,2.1387825540079) (929,2.2333350961881) (930,2.0761293898203) (931,1.9449209408851) (932,1.7077072434718) (933,1.8139169953985) (934,1.7491272097209) (935,2.0323637005162) (936,1.9072148360826) (937,2.0954110375911) (938,1.9303039138952) (939,1.955040005527) (940,1.8430258704003) (941,1.9343590019329) (942,1.9800365188584) (943,1.7671396723783) (944,2.3088256906422) (945,1.783324359491) (946,1.9511542172007) (947,2.2139506984124) (948,2.2499561672602) (949,1.8152646369547) (950,2.1515545497447) (951,2.4898895071016) (952,1.8899880262713) (953,2.699934572228) (954,2.2577675570987) (955,1.7931283162138) (956,1.8531991397521) (957,1.5881092421704) (958,1.8745244084801) (959,2.5047073152632) (960,2.0739387529682) (961,2.1102096320033) (962,1.5844977109872) (963,1.5765830979841) (964,1.8828195136209) (965,1.9360667267645) (966,2.4222097192846) (967,1.6976514980769) (968,1.7368545078278) (969,1.8948518956645) (970,1.7432937908088) (971,1.9562860575477) (972,1.9992015094353) (973,1.5610089720959) (974,1.9369899679864) (975,1.7590472831537) (976,2.0683797372061) (977,1.8455290986563) (978,2.0738084476378) (979,1.8730097569879) (980,1.6247698103559) (981,2.1811591689211) (982,1.5682901415839) (983,2.0035748935216) (984,1.8806452298386) (985,1.6541866399376) (986,1.9957339149799) (987,1.767417652981) (988,2.0731477338992) (989,1.6530326279024) (990,1.812009791977) (991,1.9814255950332) (992,2.1807478667108) (993,1.6938150480404) (994,2.0306148148592) (995,2.1504716859166) (996,2.0017774698077) (997,1.6358475088568) (998,2.0048865023721) (999,2.4407346421465) (1000,1.7975517728455) (1001,2.0656133268276) (1002,2.0044985523418) (1003,2.4340451698981) (1004,1.7254031880818) (1005,2.4583905193633) (1006,2.2110078354812) (1007,1.6280946131789) (1008,1.8859435214144) (1009,2.2638006143275) (1010,1.7405066580706) (1011,2.2271339676254) (1012,2.0006206887456) (1013,1.9323280547752) (1014,2.3102258461523) (1015,1.8893761795484) (1016,1.6128965691615) (1017,1.9042611539677) (1018,1.5149496010088) (1019,1.918812050799) (1020,1.8903706415682) (1021,1.587651380105) (1022,1.779714509193) (1023,1.8471326105175) (1024,1.7113965054378) (1025,2.3209816057233) (1026,1.8785166667052) (1027,2.1114851917682) (1028,2.0519775825363) (1029,2.0491501176336) (1030,1.7559225400868) (1031,2.2391320388367) (1032,1.8376478619665) (1033,1.9269653997356) (1034,2.2738220490386) (1035,1.9649876979975) (1036,1.8310786861644) (1037,1.7855377936851) (1038,1.9329180076041) (1039,1.395985603238) (1040,1.6758426879067) (1041,1.9310146001528) (1042,1.9647425907598) (1043,1.5922607692088) (1044,1.7530478558778) (1045,1.8097556586848) (1046,2.053220104453) (1047,1.7792789694543) (1048,1.6598744772525) (1049,2.066567495544) (1050,2.0259234385515) (1051,1.9997108575851) (1052,1.8700383903391) (1053,1.7974888879806) (1054,2.0109398782657) (1055,1.8787894293687) (1056,1.9856521464449) (1057,2.0521036496164) (1058,1.75364260188) (1059,1.5777833905752) (1060,1.8069532006732) (1061,2.0509149102799) (1062,2.241842891868) (1063,1.9086183523554) (1064,2.0796345699099) (1065,1.5829727504781) (1066,2.0673333445487) (1067,1.8379950583232) (1068,2.0021774899451) (1069,1.7103685091114) (1070,1.6545302645626) (1071,1.8409484273507) (1072,2.0228524057214) (1073,1.8193637018025) (1074,1.659562510179) (1075,2.1635535862967) (1076,1.780907848091) (1077,2.1614357276357) (1078,1.4158282484989) (1079,1.9018115913498) (1080,1.7663099969445) (1081,1.6876981284001) (1082,1.7559855879689) (1083,1.8015527271209) (1084,1.7343334562001) (1085,1.6517829497176) (1086,1.8047275831684) (1087,2.1857002626478) (1088,1.8611883259379) (1089,2.0131620509286) (1090,2.0306047720153) (1091,2.0463935005751) (1092,1.3761121009031) (1093,1.7964796265203) (1094,1.8219291938537) (1095,1.7825645084864) (1096,1.7593668186501) (1097,1.8020074647521) (1098,1.6072151987363) (1099,1.9505425363285) (1100,1.6426344317854) (1101,1.7343385305943) (1102,1.8235408027456) (1103,2.559659429776) (1104,2.2411546261816) (1105,2.2444578785667) (1106,2.0159258879374) (1107,1.8029964992876) (1108,1.9239984590389) (1109,1.7245717870312) (1110,1.9975020805944) (1111,1.8086811232422) (1112,1.7324723743453) (1113,1.9214967377091) (1114,1.8526934122324) (1115,1.947167895696) (1116,1.8113383049905) (1117,1.9859628141853) (1118,2.0435289146456) (1119,1.8171067546932) (1120,2.1234578872341) (1121,2.0767768990948) (1122,1.8892255156412) (1123,1.7290040453318) (1124,1.9074919762382) (1125,1.9155280616133) (1126,2.0170044479452) (1127,1.9514941393721) (1128,1.889150177965) (1129,2.3213875587616) (1130,1.8110567558779) (1131,2.0190460829524) (1132,2.0831516291593) (1133,2.1308797110065) (1134,1.6348024014908) (1135,1.748651384403) (1136,1.8917595900106) (1137,2.010415035187) (1138,2.2307316013888) (1139,1.9721395804536) (1140,1.707513989959) (1141,1.342313837887) (1142,2.1198306580816) (1143,1.8114269329458) (1144,2.1103528019472) (1145,1.8837751551018) (1146,1.8213829948999) (1147,1.496941534003) (1148,1.661634786601) (1149,2.0169003482337) (1150,2.0878092353704) (1151,2.0856090709709) (1152,1.8930040617821) (1153,1.7650627488798) (1154,1.9720415237451) (1155,1.8432215457313) (1156,2.3345762738383) (1157,1.7995716841655) (1158,1.9093377831419) (1159,2.0028320274099) (1160,1.6012067920614) (1161,1.860838475923) (1162,1.9053466113359) (1163,2.3869390809232) (1164,1.801557187079) (1165,2.0597410773874) (1166,1.9012740543391) (1167,1.9344903889351) (1168,1.6698887069809) (1169,1.5430890921222) (1170,1.8457195717428) (1171,1.8588126035538) (1172,1.9422306470611) (1173,2.1127781219877) (1174,1.9765941670014) (1175,1.6249767237954) (1176,1.7576348902664) (1177,2.0267626060487) (1178,1.7454716369768) (1179,2.0092866031521) (1180,1.7276450851479) (1181,1.8283771399512) (1182,1.5495779536529) (1183,2.4007211053616) (1184,1.7190439216604) (1185,1.8467534126601) (1186,1.764466917974) (1187,1.9110502540506) (1188,1.7564623978025) (1189,2.5017769940257) (1190,1.8868935692063) (1191,2.0133065614727) (1192,1.747244892788) (1193,2.007110485988) (1194,2.2399591010299) (1195,1.6417956624408) (1196,1.8896946118293) (1197,1.751622446123) (1198,1.7896657830101) (1199,1.812471849915) (1200,2.228217852844) (1201,2.4078854475446) (1202,1.9319855816647) (1203,2.0090870598738) (1204,2.0553101757524) (1205,1.7210437749278) (1206,2.0621756320729) (1207,1.8864940733779) (1208,2.1075252066788) (1209,1.8784730040338) (1210,1.6789263823161) (1211,1.9782754428371) (1212,1.8740056176512) (1213,1.9318536138536) (1214,1.841103567761) (1215,1.6456296257744) (1216,2.0073380198766) (1217,2.2012562398752) (1218,1.6396030531931) (1219,1.7967975622355) (1220,1.6296033974269) (1221,2.2461285264286) (1222,2.5017788029404) (1223,1.8011746215507) (1224,1.9009193842318) (1225,1.8592471633167) (1226,2.4402677436317) (1227,2.0834486871053) (1228,1.8216946891772) (1229,1.8785410128062) (1230,1.8175739007968) (1231,1.5040214235725) (1232,1.8753433144358) (1233,2.0080698958428) (1234,1.5831446278322) (1235,1.8481306189573) (1236,2.0893566230732) (1237,1.5921189695179) (1238,1.5259047733116) (1239,2.0764095076269) (1240,1.6501325430521) (1241,1.5355796813069) (1242,1.5848528800013) (1243,1.6566265557305) (1244,1.5818046546225) (1245,2.0256633381941) (1246,1.7949596886057) (1247,1.7872724464349) (1248,2.0299741035454) (1249,1.7843112858332) (1250,1.7895833943184) (1251,1.9750813767087) (1252,1.829435775771) (1253,1.3729465677827) (1254,1.5823723507293) (1255,1.6666770020618) (1256,1.7599202586664) (1257,1.7999198513254) (1258,1.7865388723916) (1259,2.0884052205199) (1260,1.8595996164347) (1261,1.8913095810607) (1262,1.8160150825253) (1263,1.7855156768047) (1264,1.7333645543853) (1265,1.7493707549881) (1266,1.8263953065088) (1267,2.2767731615701) (1268,1.977015106583) (1269,2.2896979766959) (1270,2.2817711715053) (1271,1.6993197851827) (1272,1.905100166754) (1273,1.6977253231566) (1274,2.0681975816133) (1275,2.0200349796981) (1276,1.911344464311) (1277,2.4074451277264) (1278,1.7948231267972) (1279,1.9522211519743) (1280,2.2343158687331) (1281,1.9562145914016) (1282,1.9956652808031) (1283,2.2215857640697) (1284,1.9338314303509) (1285,2.0830671761722) (1286,2.2319142705183) (1287,2.2157195820285) (1288,2.1148540463341) (1289,1.8406036474108) (1290,2.0837634789514) (1291,1.8890770461125) (1292,1.9905856851928) (1293,2.2968820875674) (1294,1.8947200707963) (1295,1.7808368778135) (1296,2.1597347758146) (1297,1.7456974907037) (1298,1.379370413265) (1299,1.7787909946853) (1300,1.7961366849062) (1301,1.5970124288284) (1302,2.1163394807821) (1303,1.6338276940199) (1304,1.9190386131864) (1305,2.1063097256959) (1306,1.7013015871666) (1307,1.7572415138171) (1308,2.3015716490993) (1309,1.9205890894342) (1310,1.8338688539609) (1311,1.7753811557092) (1312,1.5571485201257) (1313,1.8114145032678) (1314,1.7298327062918) (1315,2.1753250353793) (1316,2.308818315956) (1317,1.9786339806484) (1318,2.2023622527213) (1319,1.8086446299985) (1320,1.8618188655537) (1321,2.0686895648782) (1322,1.7185564364585) (1323,1.4375066284634) (1324,1.7866452975798) (1325,1.4740759327762) (1326,1.7017895114764) (1327,2.0757768362543) (1328,2.5357762376478) (1329,2.117548612998) (1330,1.7508254972169) (1331,1.7868899002789) (1332,2.0392921501013) (1333,2.0504989134124) (1334,1.6865469630152) (1335,1.8238625425403) (1336,1.7655727200259) (1337,2.0049769712347) (1338,1.731949827187) (1339,1.936292083757) (1340,1.8236495374473) (1341,1.9578773190134) (1342,2.0244744857077) (1343,2.149742776715) (1344,1.8624374505468) (1345,1.8156804625945) (1346,1.8647926136903) (1347,1.9978662833896) (1348,1.5883921842949) (1349,1.9328846896434) (1350,2.0268593599663) (1351,2.0748062518978) (1352,2.1353306056266) (1353,1.8334375072384) (1354,1.9601045401556) (1355,1.9591888884028) (1356,1.9465084725311) (1357,1.8556210148598) (1358,2.0002996724953) (1359,1.6447867908894) (1360,1.9942279141236) (1361,1.5500679660499) (1362,1.7188377900249) (1363,2.170023450591) (1364,2.4714183033988) (1365,2.8354790738625) (1366,1.6212413342751) (1367,1.5767829047873) (1368,1.8039016018522) (1369,2.4346460612377) (1370,2.1189299886634) (1371,1.9984195483872) (1372,2.3040598845428) (1373,1.7217924782302) (1374,2.0971569093398) (1375,2.1335786881978) (1376,2.0377065111229) (1377,1.978354785538) (1378,2.0669001962655) (1379,2.0015126219652) (1380,2.0385460090633) (1381,2.0316354032247) (1382,1.9819185258424) (1383,1.8915058254078) (1384,1.870914309649) (1385,2.2778021334608) (1386,1.9882459778406) (1387,1.5123510435387) (1388,1.6794304487241) (1389,1.7168563463413) (1390,1.7357772322369) (1391,2.2148761164379) (1392,1.9542056247351) (1393,1.9016378606825) (1394,1.7675502754828) (1395,2.0111679439035) (1396,1.8991891561479) (1397,1.8752763020166) (1398,2.029433480001) (1399,1.5802584238727) (1400,2.1137316692948) (1401,1.871786009272) (1402,1.9700528707509) (1403,1.9661206629017) (1404,1.9989570537883) (1405,2.0742517291178) (1406,2.1072581919603) (1407,1.6267340547272) (1408,2.1071814457276) (1409,2.0549438763467) (1410,1.9824983383737) (1411,1.8272710831082) (1412,1.8939662290561) (1413,1.8583468453027) (1414,1.496306323603) (1415,1.7605873895894) (1416,2.0432147059652) (1417,1.8054524268666) (1418,1.9080161287744) (1419,2.1733400674696) (1420,1.7859577464035) (1421,1.8219604628595) (1422,1.7727262541421) (1423,2.4692374995413) (1424,1.6157477863229) (1425,2.2570934834467) (1426,1.8950939511558) (1427,1.9751097643342) (1428,2.0041370609235) (1429,1.8577531951551) (1430,1.7104144716652) (1431,2.3286101798383) (1432,1.9945054232313) (1433,2.2065038239239) (1434,1.6619516517347) (1435,1.85180338083) (1436,1.9184163187628) (1437,1.8641404190089) (1438,1.8634608038015) (1439,2.009384035108) (1440,1.8844796931383) (1441,1.5926649738453) (1442,1.9151556864192) (1443,1.8219990770473) (1444,1.7052892081714) (1445,1.872760370829) (1446,1.6845325472797) (1447,1.7717881736194) (1448,1.9627545785687) (1449,1.6760018962999) (1450,1.9715602166337) (1451,1.4789283348859) (1452,1.8941135271721) (1453,2.042261584536) (1454,2.1272914850419) (1455,1.9397010748563) (1456,2.1841553238685) (1457,1.8606934905319) (1458,1.8642001697257) (1459,1.8767972674532) (1460,1.6847420244126) (1461,2.0510855769214) (1462,1.7126955099034) (1463,1.8813150156374) (1464,1.7663678591117) (1465,1.5871379495972) (1466,2.2841093270669) (1467,1.8891818598364) (1468,1.8242132696207) (1469,1.8770244490581) (1470,2.1842541625985) (1471,1.6482794100977) (1472,2.0671013803061) (1473,2.2640278863547) (1474,1.9799479293019) (1475,1.9804523429053) (1476,1.8973469967493) (1477,1.6544343739006) (1478,1.815284429663) (1479,1.8838558787342) (1480,2.0590535053078) (1481,1.6483349360626) (1482,2.1126571518319) (1483,1.8768769625193) (1484,1.867018225014) (1485,1.7501292066521) (1486,1.7260251306849) (1487,2.057348512262) (1488,1.5323154980881) (1489,2.0586746802031) (1490,1.7694365179943) (1491,1.7573582143385) (1492,1.9147831316979) (1493,1.7761383434126) (1494,2.1735712126035) (1495,1.6790060466319) (1496,2.3331163746492) (1497,2.2001052573342) (1498,1.951336668177) (1499,1.5593183264419) (1500,1.8353842872133) (1501,1.7043825210978) (1502,1.6375923521901) (1503,2.0633473101339) (1504,1.8832058438957) (1505,1.9476851748997) (1506,1.5280570528498) (1507,1.9121254560209) (1508,1.9167424070356) (1509,1.9132484990447) (1510,1.9777670158164) (1511,2.0024208286644) (1512,2.1121992536666) (1513,1.5938328105372) (1514,1.7602157271521) (1515,1.6721305931876) (1516,2.2654327999931) (1517,1.9443565092908) (1518,2.3704590020066) (1519,2.152832081778) (1520,2.1880667370418) (1521,1.743065417098) (1522,2.0067300510633) (1523,2.0075835304377) (1524,2.214554842165) (1525,2.0030046620463) (1526,1.4285671156125) (1527,2.2569942495067) (1528,1.9934102385005) (1529,1.9312746120316) (1530,1.851971565748) (1531,1.9275040955415) (1532,2.1429214988122) (1533,2.3347542645605) (1534,2.6121898465684) (1535,1.9867765201037) (1536,2.4348284767114) (1537,1.9672023789832) (1538,1.677505509929) (1539,1.6576161477172) (1540,1.8718376176476) (1541,2.1361919568515) (1542,1.8832326504646) (1543,1.9280521924645) (1544,1.8611236238744) (1545,1.7805346049329) (1546,2.056649167983) (1547,1.9515732470728) (1548,2.0231413730201) (1549,1.7735136059014) (1550,1.686792143357) (1551,2.4159385933932) (1552,1.9828327757039) (1553,2.1883061225766) (1554,2.02811526836) (1555,1.9443602883575) (1556,1.852573448404) (1557,2.1141358464404) (1558,1.6988937204701) (1559,1.7091059163139) (1560,2.0390665684746) (1561,1.9892424955331) (1562,2.0674830814945) (1563,2.007591712492) (1564,1.9268090952791) (1565,1.8629520855299) (1566,2.2538715365115) (1567,1.9817655803947) (1568,1.9198712084895) (1569,1.8648946943616) (1570,1.7467842735299) (1571,2.058234880058) (1572,2.2392835936661) (1573,1.5537664074622) (1574,1.7898779966506) (1575,1.9705422461107) (1576,1.7351405214459) (1577,1.9098370700771) (1578,2.0274313280207) (1579,1.9970625759491) (1580,1.6346798163192) (1581,1.8249224995884) (1582,1.7713760703693) (1583,1.8360911317825) (1584,1.659903132587) (1585,2.2167929792019) (1586,1.5405512498294) (1587,1.7565389974108) (1588,2.2998859615632) (1589,2.0904622396296) (1590,2.4853224836259) (1591,1.7142141587736) (1592,1.8039263973535) (1593,1.7899346708856) (1594,1.6729422585227) (1595,1.5719097181741) (1596,1.7293025681142) (1597,1.9896832191552) (1598,1.510751661385) (1599,2.0411115790677) (1600,1.5035400037271) (1601,1.9949757728193) (1602,1.8364593748876) (1603,1.9077610359312) (1604,1.742174130352) (1605,1.5885143969071) (1606,1.9312113186106) (1607,1.4918800904155) (1608,1.7307943720325) (1609,1.8358227955096) (1610,2.1442598926369) (1611,1.9809287268357) (1612,1.7935489030505) (1613,1.7006097718209) (1614,2.4271347767662) (1615,1.8251902934154) (1616,2.2149920985971) (1617,1.7836902371396) (1618,1.8707313048812) (1619,1.9746951807508) (1620,1.9019414425302) (1621,1.591255311616) (1622,1.8687949077129) (1623,1.9528442997063) (1624,2.0835906480845) (1625,1.9228743563392) (1626,2.3801827075684) (1627,2.1001121136362) (1628,2.3214339193524) (1629,2.0138470692914) (1630,1.7743710178326) (1631,1.8160521236774) (1632,1.9229242373368) (1633,1.6649570293797) (1634,1.6864063220126) (1635,1.7193145384546) (1636,1.9132313394759) (1637,1.6295974001872) (1638,2.1065905976789) (1639,1.8573122324681) (1640,1.6939664089499) (1641,1.7205416394437) (1642,1.6786026609975) (1643,1.5616877543089) (1644,1.8342222745594) (1645,2.059461563068) (1646,1.8749705807555) (1647,2.0569521144581) (1648,1.5981109944653) (1649,2.3545513430926) (1650,1.7232947814662) (1651,2.0263048771612) (1652,1.9799065013424) (1653,1.8590595278817) (1654,1.9711892213849) (1655,1.9600987463453) (1656,1.9296724965137) (1657,2.0508835574855) (1658,1.7821644998672) (1659,2.0651313024133) (1660,2.0910381315655) (1661,2.0172515969783) (1662,2.0324951288176) (1663,2.057210959818) (1664,2.0082755220566) (1665,1.98491833032) (1666,2.0062210791482) (1667,1.674567473857) (1668,1.7617893317354) (1669,1.731632717309) (1670,1.8881112809577) (1671,1.90116380051) (1672,1.7608981065528) (1673,1.4792030589608) (1674,1.9109120853308) (1675,1.7702418366654) (1676,2.1396211421002) (1677,1.6055992898902) (1678,1.9188308134639) (1679,1.8355899277872) (1680,1.7163217234336) (1681,1.8485316273142) (1682,1.6497856924199) (1683,1.7380211274092) (1684,2.0347594949814) (1685,1.7992028328759) (1686,2.0519244121204) (1687,1.8551754217004) (1688,2.1904243294768) (1689,1.8322662870272) (1690,1.4082097203511) (1691,1.6706554868403) (1692,1.8243249682992) (1693,2.0830034889068) (1694,2.1400936710621) (1695,2.1150509466968) (1696,2.0019798208433) (1697,1.5088557754594) (1698,1.9533757637203) (1699,1.9357542007999) (1700,2.0230940404162) (1701,1.9116032538383) (1702,2.3051673937285) (1703,2.0535139172114) (1704,1.494793859603) (1705,1.7162131930106) (1706,1.7905556885274) (1707,1.8968189061354) (1708,1.9012237165593) (1709,1.846799888899) (1710,2.2102342942654) (1711,1.6808379688286) (1712,1.7081711702663) (1713,1.5570264647158) (1714,2.2926555884624) (1715,1.8154782094403) (1716,1.6014968580923) (1717,1.685335572869) (1718,1.9303677245354) (1719,1.9285617425803) (1720,1.5227812888275) (1721,2.0208487153433) (1722,1.6950458992667) (1723,2.0889141702516) (1724,1.7263247528666) (1725,1.845253224576) (1726,1.6794067940592) (1727,2.1956230000397) (1728,2.0836113071515) (1729,1.8073298573949) (1730,1.7573640241855) (1731,2.0343310913631) (1732,1.5714316047861) (1733,1.830818940313) (1734,2.0983229398822) (1735,1.8006141636783) (1736,1.6153546364959) (1737,1.6344431101955) (1738,1.938644798379) (1739,1.7314153792377) (1740,1.8074939066248) (1741,1.7560162930409) (1742,1.7713123070145) (1743,1.9993997639945) (1744,1.7308413176612) (1745,1.7446244290615) (1746,2.0419286790738) (1747,1.6268500020363) (1748,1.8495948360533) (1749,1.8091916764908) (1750,1.9318602723569) (1751,1.4951591357499) (1752,1.767195135159) (1753,1.724516093935) (1754,1.8505242717227) (1755,2.0211082747949) (1756,2.2473024066405) (1757,1.6362023383366) (1758,1.7633101143341) (1759,1.8538252331787) (1760,1.5948749544446) (1761,2.122771280163) (1762,1.7293203913717) (1763,1.9754555367358) (1764,1.2920487585712) (1765,2.0150162213091) (1766,1.4948074085696) (1767,1.8140418183698) (1768,1.8292385881731) (1769,1.7936174404658) (1770,2.147588949138) (1771,1.9301028598439) (1772,1.9443101612287) (1773,1.7817680101999) (1774,1.830025336616) (1775,1.6670910949494) (1776,1.8571565498041) (1777,2.0238177426179) (1778,1.7628565436562) (1779,2.0262973724631) (1780,1.7857412756755) (1781,1.8438009277255) (1782,1.7912139672005) (1783,1.5524004853258) (1784,1.5142222845253) (1785,2.1360115231027) (1786,1.8745253548887) (1787,1.9230858460275) (1788,1.9604597826258) (1789,1.8863655167004) (1790,1.7449543849532) (1791,2.3819951832944) (1792,1.5676606547714) (1793,1.7150582272219) (1794,1.9052395356026) (1795,1.8470781225468) (1796,1.94276409673) (1797,1.8978128127421) (1798,2.0861363852798) (1799,2.3807238633961) (1800,1.6849072614516) (1801,2.3357405869913) (1802,1.7182352493331) (1803,2.1987338990622) (1804,1.674686945575) (1805,1.6215752654902) (1806,1.7384989359006) (1807,1.9303616553741) (1808,1.986330055904) (1809,1.6984053114563) (1810,2.0874156512905) (1811,1.978145384291) (1812,2.1831720508077) (1813,1.9413363379983) (1814,1.6067455968624) (1815,2.146702145575) (1816,1.6457499103777) (1817,1.8454658243483) (1818,1.7678037680701) (1819,2.2291850011582) (1820,1.7014379294425) (1821,2.10349186983) (1822,2.0664965341285) (1823,1.6494719307747) (1824,2.0196973315033) (1825,2.013891329563) (1826,1.6998151339452) (1827,1.7297636282328) (1828,1.6989393797348) (1829,2.0088157851246) (1830,2.03777934113) (1831,1.9669021404872) (1832,1.8626453188744) (1833,2.0721502699233) (1834,1.9548393513167) (1835,1.9164644493429) (1836,1.7379490367088) (1837,2.0903292019247) (1838,1.7244516027301) (1839,1.7667009106425) (1840,1.6705143738304) (1841,1.5672846775508) (1842,2.1029555900747) (1843,1.8418860033824) (1844,2.3812463516581) (1845,2.3538982326107) (1846,1.6050213058569) (1847,1.7992030152148) (1848,1.9501047031854) (1849,1.6380289754045) (1850,1.6983212442528) (1851,1.6966429852324) (1852,1.4288330353564) (1853,1.7106604405562) (1854,1.9867211267332) (1855,1.8476890383807) (1856,1.5366961220704) (1857,1.9980442618948) (1858,1.7582388315511) (1859,1.8068755155401) (1860,1.8343704953398) (1861,1.8006949434279) (1862,1.6678856503229) (1863,1.7151775670006) (1864,1.9413667209213) (1865,1.7146675370703) (1866,1.8130937541604) (1867,2.0140956065461) (1868,1.7653415286068) (1869,1.7947003233944) (1870,1.9630848430085) (1871,2.0869186457998) (1872,1.9766703546234) (1873,1.6452306055701) (1874,1.7750088126982) (1875,2.0967251332176) (1876,2.0185127455224) (1877,1.5613023417497) (1878,1.7336391405273) (1879,2.0721726919935) (1880,1.768418531135) (1881,1.8203600855914) (1882,1.8329883951262) (1883,2.2707715620878) (1884,1.9788639177933) (1885,2.1605560421315) (1886,1.67857681203) (1887,2.0428577941554) (1888,1.7600123401592) (1889,1.7878534614293) (1890,1.8549791615376) (1891,1.7879889117482) (1892,2.0036158596815) (1893,1.5432370897037) (1894,1.8126019493025) (1895,1.5506001646654) (1896,1.957378382679) (1897,1.6517495784127) (1898,1.8744322324658) (1899,1.8014321644466) (1900,2.1078704378555) (1901,1.7973202783359) (1902,1.8184298441096) (1903,1.7572385086403) (1904,1.8136954735995) (1905,2.1812674946067) (1906,1.7595807171477) (1907,1.6459341692053) (1908,1.6528514874517) (1909,1.4977493226438) (1910,1.5122382340853) (1911,1.7020602427435) (1912,1.9428801624291) (1913,1.7830509937981) (1914,1.7459532730305) (1915,1.6396927943579) (1916,1.6795673054985) (1917,1.7080046384402) (1918,2.0557173388746) (1919,1.4419829916508) (1920,1.6728357197926) (1921,1.6206465219224) (1922,1.6758999516233) (1923,2.1050350982109) (1924,2.4148049713499) (1925,1.8601061681745) (1926,1.8252482723464) (1927,2.0693892349725) (1928,1.8411396369711) (1929,2.2278148181504) (1930,1.7049706614534) (1931,2.0746277926213) (1932,1.8051510169115) (1933,2.4676988611098) (1934,1.9805616363399) (1935,1.9333027507574) (1936,2.0660871280668) (1937,1.6289073631979) (1938,1.9931623861399) (1939,1.4325765075123) (1940,1.9314484667222) (1941,1.8190198419919) (1942,2.0811311706992) (1943,2.0961633949734) (1944,1.9465920143493) (1945,1.9120632501648) (1946,1.7583283379038) (1947,1.6534540222504) (1948,1.7946184404627) (1949,1.7340516397372) (1950,1.8580692247263) (1951,1.6104679469501) (1952,1.7014391778986) (1953,1.9311775310461) (1954,1.9179765579465) (1955,1.9546872028555) (1956,1.4790737905397) (1957,1.5167289990552) (1958,1.6678393352899) (1959,1.769104601079) (1960,2.1565032175369) (1961,1.5857160671055) (1962,2.3023038430369) (1963,2.0548891864018) (1964,1.8052365755141) (1965,1.7865387992471) (1966,1.68701209792) (1967,1.7469111779872) (1968,1.9197766038859) (1969,1.8011087019439) (1970,1.8020111049715) (1971,2.007150821232) (1972,2.0765005945339) (1973,1.8134033607036) (1974,1.6953808595613) (1975,1.696535567773) (1976,1.5283762332193) (1977,1.9452146862986) (1978,1.726646561207) (1979,1.730702077548) (1980,1.909953817077) (1981,1.654673946008) (1982,1.7556972733675) (1983,1.6420049857289) (1984,2.0305785580618) (1985,2.2034712574371) (1986,1.9735065002059) (1987,1.9482532279662) (1988,2.224789356624) (1989,1.6499628685119) (1990,2.0139803131655) (1991,1.775894175447) (1992,1.7204083188683) (1993,1.5814510944478) (1994,1.6879928992729) (1995,1.7588211358394) (1996,2.0660563143486) (1997,1.4155336527612) (1998,1.7018828318995) (1999,2.0347485611082) (2000,1.8645771822352) };
\addplot+[line width=2pt, mark=none] coordinates { (1,6.2648273679558) (2,2.5682710957059) (3,2.4685547965721) (4,2.0274054739041) (5,2.0178263009696) (6,1.6814934239656) (7,1.8826809132633) (8,2.0277144057157) (9,2.0560064189501) (10,1.6329308377177) (11,2.1567272600015) (12,1.8730323005667) (13,1.572626916649) (14,3.2961748350176) (15,2.1195288688568) (16,2.1590878505144) (17,1.8683745579893) (18,2.7113424829703) (19,2.0975498250611) (20,1.8048342365351) (21,2.838200289055) (22,2.0067257194117) (23,1.8668574285945) (24,1.6755424870003) (25,2.0311433334799) (26,2.606146177106) (27,1.8187083632462) (28,1.8374981727406) (29,1.9250235166133) (30,2.0850798228551) (31,1.8282680468081) (32,2.1883183382247) (33,1.8485176378122) (34,1.8903088636587) (35,2.2362841904501) (36,2.730456841925) (37,1.8132586187627) (38,1.895559991466) (39,2.3736340619022) (40,1.8571327793951) (41,1.7419957466375) (42,2.3313548370158) (43,1.9817389373821) (44,2.1784283204646) (45,1.8650471001477) (46,2.431491812274) (47,1.7191507272043) (48,1.8154810455349) (49,1.7475632318256) (50,1.9695492489424) (51,1.939238322645) (52,1.7210344895874) (53,1.7827806941844) (54,2.8938168023388) (55,1.6391778050186) (56,1.9547074509783) (57,2.5898059803203) (58,2.0336205656386) (59,2.2564568815518) (60,1.9975253792902) (61,1.9409470736902) (62,1.7669852805254) (63,1.5896421384607) (64,1.7290318858667) (65,2.2410082353984) (66,1.7065553126129) (67,1.8431238120485) (68,2.0820748109061) (69,1.9689292033372) (70,2.2253679019172) (71,2.050130345673) (72,2.4596845771892) (73,1.740702518582) (74,1.9337305037915) (75,1.7332746641334) (76,2.1494199427107) (77,2.7306151843225) (78,1.9482012404401) (79,2.0393464864559) (80,1.8293310911213) (81,1.7376495659502) (82,1.9645429709486) (83,1.6327805805174) (84,1.905617322826) (85,1.9686037489899) (86,1.8167191711246) (87,2.0217475882549) (88,1.8890811888133) (89,2.2426642599065) (90,1.8030383320419) (91,2.1684485063738) (92,1.8491382829716) (93,2.0037988294215) (94,1.975879038198) (95,1.8415488043183) (96,2.2213481250363) (97,1.8753500466615) (98,1.8566796095601) (99,2.0731438916544) (100,1.9599512883483) (101,1.9456186531784) (102,1.804171769965) (103,2.0787747542091) (104,1.6493291870194) (105,2.4389351072233) (106,1.9083752198067) (107,1.8718455554857) (108,2.0113061173237) (109,2.2925090820651) (110,1.8281776387399) (111,2.2781164131299) (112,1.7889037633052) (113,1.8337149644577) (114,1.7612109325103) (115,1.9818712954807) (116,1.7565455651692) (117,1.8113701133493) (118,1.9363237114047) (119,2.7627162426182) (120,1.8147712010465) (121,1.8215961169088) (122,1.8329734168118) (123,1.9672647465325) (124,1.874327645658) (125,1.8099144226701) (126,1.9571643616721) (127,1.7756167761256) (128,2.0278587366757) (129,2.0083362354983) (130,1.9859529282598) (131,2.3054923790201) (132,2.3130449048565) (133,2.0060401750111) (134,2.0088599137228) (135,2.028917630435) (136,1.9343913122375) (137,2.1743759355767) (138,1.7324804769086) (139,2.0672921055187) (140,2.1465828667402) (141,1.972925805405) (142,1.9224459810336) (143,1.8112970433879) (144,1.9930415016198) (145,1.8781996088906) (146,2.3166440857018) (147,2.0425741166198) (148,1.8583185563585) (149,1.6794882706256) (150,1.5632406037768) (151,1.8891568233486) (152,1.8563812386276) (153,1.8849998043225) (154,1.9638074163967) (155,1.9663444217031) (156,1.9464390366156) (157,1.6508417246297) (158,1.7856773416017) (159,1.7773653944537) (160,1.7879569190347) (161,1.8465980311622) (162,2.0965802170841) (163,1.7282599168102) (164,1.8656717463057) (165,1.8599650684797) (166,1.7867242350032) (167,1.9323938098211) (168,1.8728748175337) (169,1.6467417973303) (170,1.8462817002077) (171,2.1239598143489) (172,2.214194930039) (173,1.9451536183367) (174,1.7367905966398) (175,1.6839474115394) (176,1.6273173819677) (177,2.0598695104575) (178,1.8924001392766) (179,2.0557069240124) (180,1.8416216601915) (181,1.8534009088622) (182,1.8455726000043) (183,1.7975028937319) (184,1.619927200479) (185,2.1716898996649) (186,1.9100097165613) (187,1.9233711248575) (188,1.9616344423955) (189,1.7676286184145) (190,1.9013655260338) (191,1.8125152444396) (192,2.1262515088451) (193,1.8059948711887) (194,1.8435113515166) (195,1.7943234315507) (196,1.8741278209696) (197,2.1377546066306) (198,1.91389973822) (199,2.2279720329942) (200,2.0011524731657) (201,1.7385912338299) (202,1.7755807264684) (203,1.7516832359322) (204,1.841487690688) (205,1.6293047617982) (206,1.83616177403) (207,2.3409374850584) (208,1.9263386350024) (209,1.5636213538614) (210,2.0456242798165) (211,1.7284936812652) (212,1.8871818927635) (213,1.7773064916117) (214,2.0343123757008) (215,1.5970976227922) (216,1.8009774350275) (217,1.6304054708621) (218,1.8461592626821) (219,1.6886383607554) (220,2.0233962401765) (221,1.9525020804194) (222,1.9717666632372) (223,1.804820613051) (224,1.8877475355652) (225,1.7500671526245) (226,1.9280631218495) (227,1.7685406766957) (228,1.6147143941776) (229,1.6061394458478) (230,2.00903981523) (231,1.8663476294815) (232,2.0229628410518) (233,1.6574755212574) (234,1.7448687070398) (235,2.0402636721769) (236,1.7217731924733) (237,1.9197298183513) (238,2.1498108315641) (239,1.6802112002307) (240,1.8039374471029) (241,1.6087148391331) (242,1.5697969462786) (243,1.5641855033929) (244,1.8141810234375) (245,1.5815558476158) (246,1.6196128551829) (247,1.5526560378882) (248,1.5687018885553) (249,1.7284029276764) (250,1.804636010628) (251,1.8896799747876) (252,1.7387451385454) (253,1.731415790968) (254,1.9430115729512) (255,1.6775646038146) (256,1.7243549548515) (257,1.8606568992413) (258,1.8689416058072) (259,1.8654739303193) (260,1.802546474906) (261,1.6987526956849) (262,1.9644685387778) (263,1.4523633070578) (264,1.9348528883596) (265,1.7449298227501) (266,1.6360459645158) (267,1.8685845817134) (268,1.6141507246998) (269,1.8293672352267) (270,1.6657846907743) (271,1.9161582254267) (272,1.5876431775093) (273,1.6701863762438) (274,1.7064578853932) (275,1.5810059473198) (276,1.7182581637622) (277,1.6378559510655) (278,1.7014479386329) (279,1.6411464146002) (280,1.7770617130477) (281,1.8419561685688) (282,1.8870184374698) (283,1.7683364184644) (284,2.021150171915) (285,1.7400597105744) (286,1.8838541186011) (287,1.7806322552884) (288,1.8501874958787) (289,1.7093870528459) (290,1.6956459554496) (291,1.9250874312354) (292,1.4493507845353) (293,1.5714731222036) (294,1.8443212509879) (295,1.9114545434743) (296,1.8235067105445) (297,1.736199333699) (298,1.7767029543995) (299,1.8114127701717) (300,1.7508050071573) (301,1.7023044307627) (302,1.4793489760705) (303,1.7195613014484) (304,2.0782689353929) (305,1.6883688761105) (306,1.6887959506922) (307,1.9981483066468) (308,1.5179716048524) (309,1.908810481338) (310,1.7398070458698) (311,1.4167958654506) (312,1.5440022057118) (313,1.5962274824986) (314,1.5719784052905) (315,1.7195263990284) (316,1.7947275491544) (317,1.687987915824) (318,1.4324411584308) (319,1.7595367322488) (320,1.5527234414317) (321,1.6738858298655) (322,1.5256602113207) (323,1.7939871449099) (324,1.8566843981835) (325,1.8034316749933) (326,1.6799411047198) (327,1.7019401763348) (328,1.7380466924705) (329,1.3682124646196) (330,1.7288222468028) (331,1.6677732887156) (332,1.8133876766351) (333,1.6854805181794) (334,1.5211137705027) (335,1.75804144269) (336,1.5128250098698) (337,1.537471339211) (338,1.665833090381) (339,1.6023015873097) (340,1.4132412820387) (341,1.5844123853825) (342,1.598554019046) (343,1.5666244436628) (344,1.501350180783) (345,1.61594301703) (346,1.5467051081552) (347,1.6786328355957) (348,1.6884558965942) (349,1.61441776424) (350,1.4898255428728) (351,1.6545909293881) (352,1.6717738336281) (353,1.575390329837) (354,1.4621877422839) (355,1.6752783811438) (356,1.5065588808224) (357,1.5612621818006) (358,1.5113647914536) (359,1.6737094596248) (360,1.5910808597585) (361,1.5369261156408) (362,1.6206627210198) (363,1.6436041983783) (364,1.4656781099845) (365,1.5070513465843) (366,1.4599881501657) (367,1.586892114251) (368,1.5567116103964) (369,1.688935397782) (370,1.4629114995614) (371,1.3744125769271) (372,1.4300537379861) (373,1.2271127486394) (374,1.5886945537985) (375,1.3422758656597) (376,1.4346083121048) (377,1.3965510623732) (378,1.5342564279226) (379,1.5901001751707) (380,1.5912518400215) (381,1.4670895410053) (382,1.7878637810894) (383,1.5840619909547) (384,1.4397719564235) (385,1.775515928648) (386,1.5479012663249) (387,1.4179045174657) (388,1.6259508660137) (389,1.4205074494141) (390,1.3760666146436) (391,1.5498616294795) (392,1.7276372470434) (393,1.6242708694343) (394,1.7061048459765) (395,1.5013367635726) (396,1.5178311851897) (397,1.5947309393338) (398,1.6573705362229) (399,1.5109869738476) (400,1.4958136707017) (401,1.4430482427124) (402,1.3038653759049) (403,1.391483652747) (404,1.6605409742701) (405,1.6335263141321) (406,1.482547936627) (407,1.7839444832113) (408,1.4334727163692) (409,1.5428228759073) (410,1.3620232233066) (411,1.3372583692519) (412,1.6178561620651) (413,1.3566735556349) (414,1.5210507362187) (415,1.4080432958895) (416,1.4490083988641) (417,1.4378752093519) (418,1.6458973103017) (419,1.3211925764873) (420,1.4059103505481) (421,1.4524907283923) (422,1.4909807967565) (423,1.7353257219949) (424,1.3634904119972) (425,1.5012122667794) (426,1.7461579680907) (427,1.4234746501272) (428,1.3443713413721) (429,1.5990648587429) (430,1.7641309459852) (431,1.7539120615679) (432,1.5421420371475) (433,1.4791342406908) (434,1.7608663248079) (435,1.3754956290616) (436,1.4100996964811) (437,1.446516469814) (438,1.5338361284418) (439,1.429443562123) (440,1.8463196102536) (441,1.4846883284881) (442,1.3828248762206) (443,1.4511341264681) (444,1.3356046382219) (445,1.3349844668238) (446,1.3760496375403) (447,1.6571691188698) (448,1.5835250388237) (449,1.4179197544252) (450,1.4412057934267) (451,1.4423166333719) (452,1.3127407505929) (453,1.2669316735353) (454,1.6796942178291) (455,1.5018742673998) (456,1.4604913976238) (457,1.2691562601038) (458,1.5589468164847) (459,1.335872586136) (460,1.6143879722259) (461,1.6519341093312) (462,1.5287551720705) (463,1.2997393920899) (464,1.4095817811132) (465,1.444343767782) (466,1.5834797570481) (467,1.3572889791308) (468,1.5162359334328) (469,1.4812641295959) (470,1.5241622008117) (471,1.4392530131491) (472,1.4329862173153) (473,1.2028282261065) (474,1.2617330353247) (475,1.4377683721585) (476,1.5117826717521) (477,1.7079291987395) (478,1.4240779895695) (479,1.3247086179618) (480,1.5657050020901) (481,1.4917690090136) (482,1.4963872950563) (483,1.5768786638426) (484,1.4899291922809) (485,1.2215719624225) (486,1.4432394564275) (487,1.4610879211603) (488,1.3729656363361) (489,1.4784718071242) (490,1.3194308310067) (491,1.3608960621766) (492,1.3904427990105) (493,1.5232600536732) (494,1.5697363366629) (495,1.3553002590938) (496,1.4765782743238) (497,1.5147463011669) (498,1.5717444451152) (499,1.4135726545653) (500,1.3159797299555) (501,1.3747053665756) (502,1.5348697477584) (503,1.3062665376195) (504,1.3689910164375) (505,1.4574559934045) (506,1.6443548678812) (507,1.4295233044206) (508,1.3716549271737) (509,1.3542257287986) (510,1.7286612792469) (511,1.4451315612403) (512,1.4002505515133) (513,1.2322113565628) (514,1.2872706177022) (515,1.433658810064) (516,1.4312156949831) (517,1.7177274836979) (518,1.5901654024852) (519,1.4630558321672) (520,1.4081552690432) (521,1.5272717851512) (522,1.2275709485545) (523,1.3501409823263) (524,1.4163594530336) (525,1.6120226591569) (526,1.3653195870822) (527,1.8025631221656) (528,1.483278971907) (529,1.4370393624395) (530,1.6774446389818) (531,1.6546916730876) (532,1.275433829142) (533,1.3003543674695) (534,1.5131624506881) (535,1.5367136609695) (536,1.5488308224592) (537,1.3294579190683) (538,1.5240577726374) (539,1.3605476537308) (540,1.389878956129) (541,1.6100840976395) (542,1.545733465859) (543,1.4993875045272) (544,1.5169808729221) (545,1.3472002406366) (546,1.4374072688828) (547,1.4347064235724) (548,1.394320921818) (549,1.5374755970272) (550,1.1494935796295) (551,1.6134944745265) (552,1.2808698569554) (553,1.2120207654654) (554,1.3799447369807) (555,1.4916848769742) (556,1.2249968892668) (557,1.7626561764789) (558,1.3682107106638) (559,1.4085820004141) (560,1.4939135019033) (561,1.5986269475827) (562,1.3852151241531) (563,1.4360477806465) (564,1.4795793963139) (565,1.3707299803452) (566,1.2189984270231) (567,1.3729649531706) (568,1.4109771490122) (569,1.2818134361914) (570,1.4127499156501) (571,1.5010059422554) (572,1.507888080106) (573,1.4480859002048) (574,1.4385233833351) (575,1.6640326125745) (576,1.5757990704087) (577,1.4246486606259) (578,1.1763566253009) (579,1.5603356163072) (580,1.4422067372771) (581,1.4406041097564) (582,1.4330155905854) (583,1.4383477839558) (584,1.2419125936344) (585,1.3817457400266) (586,1.521696842878) (587,1.6028989059175) (588,1.4752094205548) (589,1.2776391278873) (590,1.5251295461799) (591,1.4494070708417) (592,1.4455975933008) (593,1.3058518449239) (594,1.4216792043681) (595,1.2831554275417) (596,1.471657230047) (597,1.4467597500924) (598,1.3774391112864) (599,1.7091795925786) (600,1.2236650792832) (601,1.4916472109248) (602,1.6087303287227) (603,1.5869859638432) (604,1.4475972308722) (605,1.5031315693203) (606,1.4957434276911) (607,1.5810669210048) (608,1.5612458179014) (609,1.7998734056142) (610,1.4085955314281) (611,1.5043212779885) (612,1.6063039543943) (613,1.3757316439131) (614,1.3733308239927) (615,1.5384569370894) (616,1.4406497837387) (617,1.3213312696779) (618,1.359358570433) (619,1.3517590079657) (620,1.3271453793886) (621,1.3888996865901) (622,1.6001686106122) (623,1.5665428699254) (624,1.2024742588898) (625,1.5551519035857) (626,1.4693204064101) (627,1.5525909737116) (628,1.5819858374324) (629,1.3103986999872) (630,1.4320722706372) (631,1.4964384250278) (632,1.4839452268204) (633,1.4231183790896) (634,1.6017464651047) (635,1.3344561997162) (636,1.4534504405076) (637,1.6023889942695) (638,1.5316586042437) (639,1.3543583212937) (640,1.4839305632013) (641,1.5516172447506) (642,1.7683653801334) (643,1.434362489695) (644,1.4302426140824) (645,1.2559984795633) (646,1.7163572026228) (647,1.5986758249297) (648,1.7277305722057) (649,1.4130099882345) (650,1.5533073123069) (651,1.3307305820355) (652,1.9576065672842) (653,1.3421784606691) (654,1.3560701799526) (655,1.6027636207257) (656,1.5017047842491) (657,1.5177247214203) (658,1.3567649908518) (659,1.3441245462295) (660,1.5181734866982) (661,1.3113127006978) (662,1.4241161546472) (663,1.6476830865603) (664,1.4830094865023) (665,1.7802927619156) (666,1.2398465993982) (667,1.5283547914416) (668,1.3918616087338) (669,1.5739961336279) (670,1.7730877843708) (671,1.487410483301) (672,1.4909358813585) (673,1.6574610928517) (674,1.4657118891395) (675,1.4263818427494) (676,1.4404296949407) (677,1.6173726990039) (678,1.4847389361497) (679,1.439630475341) (680,1.3977553933142) (681,1.5412623883335) (682,1.2756490010768) (683,1.2014311037002) (684,1.6050455151536) (685,1.4819530808924) (686,1.5924599162855) (687,1.6801869522169) (688,1.4395724519833) (689,1.7020133651361) (690,1.3337079046168) (691,1.5041173025567) (692,1.3712669657202) (693,1.4605984051408) (694,1.4301069266177) (695,1.3469334041034) (696,1.4022887496455) (697,1.2267009460119) (698,1.5580356763475) (699,1.3461222696091) (700,1.4873863178668) (701,1.5168984398003) (702,1.4471390314453) (703,1.4951738947713) (704,1.3071132468372) (705,1.4314799626568) (706,1.2132771846784) (707,1.4791593995347) (708,1.4865129883937) (709,1.4308921328723) (710,1.440812598442) (711,1.4190513174788) (712,1.9081982961808) (713,1.564154557058) (714,1.639863157146) (715,1.407444111201) (716,1.3244605445989) (717,1.2307386072488) (718,1.4717775861186) (719,1.446366575198) (720,1.3790375131534) (721,1.3973955556044) (722,1.3915781774977) (723,1.5179878279694) (724,1.3826715141242) (725,1.688664312669) (726,1.5043477554768) (727,1.6699784726741) (728,1.2170950159823) (729,1.5518520505708) (730,1.4962448143178) (731,1.7399576553896) (732,1.4211590818801) (733,1.4201333007999) (734,1.5271029477013) (735,1.5803824744548) (736,1.3550141339221) (737,1.4013716851266) (738,1.9118842437519) (739,1.522370536625) (740,1.3617210683441) (741,1.5040065448426) (742,1.416265339546) (743,1.319617642453) (744,1.4453216170293) (745,1.2277153780064) (746,1.4659244015135) (747,1.6013149652069) (748,1.4993558497155) (749,1.4107143554348) (750,1.6173633751298) (751,1.4715681545213) (752,1.4764905680758) (753,1.403771161005) (754,1.3783395552134) (755,1.5874072719704) (756,1.4531658787411) (757,1.8029789564494) (758,1.1950233495688) (759,1.3642231233388) (760,1.4464901881143) (761,1.5447985118739) (762,1.3987144561395) (763,1.4134892718253) (764,1.5654324156795) (765,1.4238012497027) (766,1.41211525632) (767,1.3542102039659) (768,1.7113467057496) (769,1.4510488347181) (770,1.5739695581727) (771,1.2255004403904) (772,1.7209917610753) (773,1.3519631996297) (774,1.7410449425898) (775,1.5556981733918) (776,1.5126077318911) (777,1.4623740166431) (778,1.1517642856821) (779,1.3066420527576) (780,1.6465235193461) (781,1.2901475003089) (782,1.6436799614467) (783,1.5666938242774) (784,1.3310424196959) (785,1.2891562937335) (786,1.3863523038755) (787,1.7659261819344) (788,1.5329484487712) (789,1.3187020248631) (790,1.4713981624078) (791,1.3090963136664) (792,1.0783386478582) (793,1.5086354606438) (794,1.6387544175492) (795,1.581572018234) (796,1.7749938240614) (797,1.376033208975) (798,1.3767741017175) (799,1.5885053468892) (800,1.5161410235552) (801,1.1750296985851) (802,1.5156630039106) (803,1.6815309346424) (804,1.681766742766) (805,1.6549316291544) (806,1.5140684005689) (807,1.4999453827418) (808,1.7147831678965) (809,1.5255369884654) (810,1.6141977057615) (811,1.4947986584568) (812,1.5370873896562) (813,1.5399060904011) (814,1.4650514721571) (815,1.5005414626285) (816,1.4039726461655) (817,1.426372543743) (818,1.3859130769071) (819,1.5288759865766) (820,1.608915280604) (821,1.619883056678) (822,1.4237665473189) (823,1.5265851533913) (824,1.2807496280341) (825,1.3674265906604) (826,1.4179051394525) (827,1.3911307023966) (828,1.5542848013718) (829,1.5084949384744) (830,1.4823468340277) (831,1.561608553899) (832,1.3741055783019) (833,1.4135942356955) (834,1.4935957639918) (835,1.4467582319245) (836,1.3369577725254) (837,1.3669728434089) (838,1.8045920920795) (839,1.4881157794814) (840,1.3880720361864) (841,1.8699383997809) (842,1.4918709340599) (843,1.5566914051867) (844,1.4312964406123) (845,1.4179993680372) (846,1.2387179970915) (847,1.2906885924804) (848,1.4589089260264) (849,1.5050932318176) (850,1.3673595941818) (851,1.4431109535812) (852,1.5566085776353) (853,1.2432956931463) (854,1.3052134429492) (855,1.2576550768053) (856,1.3826452220161) (857,1.4068284959236) (858,1.2831875536738) (859,1.3928213312789) (860,1.2448992313334) (861,1.5382663549819) (862,1.2875206454119) (863,1.3023000212486) (864,1.5330744445933) (865,1.6846173074369) (866,1.5452951236404) (867,1.8440036860277) (868,1.44844082443) (869,1.3204634818525) (870,1.3074194319669) (871,1.8767316483133) (872,1.3597982710979) (873,1.7588990515219) (874,1.5279483568441) (875,1.3984667034579) (876,1.4583860941076) (877,1.4086536625378) (878,1.3630205186069) (879,1.4269941355892) (880,1.4214690043117) (881,1.3563602324728) (882,1.7599056369521) (883,1.6804996046316) (884,1.6078342052271) (885,1.3307238051408) (886,1.3015175932616) (887,1.5892907135115) (888,1.5597654426369) (889,1.2378308121953) (890,1.2613412477178) (891,1.434338050928) (892,1.3314645756731) (893,1.5912176699171) (894,1.414247352166) (895,1.5072793080077) (896,1.4463185328495) (897,1.7258722975201) (898,1.5428219269967) (899,1.432997694263) (900,1.5241424325142) (901,1.5133955065119) (902,1.5660067806889) (903,1.4824012535629) (904,1.307290923151) (905,1.3858583994049) (906,1.510947616049) (907,1.472271834355) (908,1.4734188833009) (909,1.5773563284254) (910,1.3529187768673) (911,1.2361943815393) (912,1.4320718055371) (913,1.2052458494173) (914,1.8039378737259) (915,1.3296174089975) (916,1.302406506366) (917,1.4598566984903) (918,1.3336311583617) (919,1.685990728575) (920,1.2414460609863) (921,1.4602388385635) (922,1.6803008377164) (923,1.6341513174973) (924,1.7474590317107) (925,1.6797429160964) (926,1.6657452932369) (927,1.3559421421918) (928,1.4840202547709) (929,1.8063379865283) (930,1.3686362879559) (931,1.3282888351193) (932,1.6560385742055) (933,1.6047185682667) (934,1.3424182893544) (935,1.3983741495637) (936,1.4319340453948) (937,1.3145461199669) (938,1.3485815590512) (939,1.0896716158394) (940,1.2871634912742) (941,1.5493369902122) (942,1.504025250678) (943,1.609704529499) (944,1.6912913380592) (945,1.4442593000413) (946,1.6120995824235) (947,1.5832594249559) (948,1.4720523485954) (949,1.5994177607072) (950,1.6818205739631) (951,1.2312081518018) (952,1.538705269158) (953,1.4144061041218) (954,1.3185509625804) (955,1.6754035507404) (956,1.5617629210545) (957,1.3498624517164) (958,1.5055415068593) (959,1.346156648944) (960,1.3188842389019) (961,1.4831481017922) (962,1.4342165120865) (963,1.7369154723296) (964,1.4397894548855) (965,1.571739314008) (966,1.5335116219359) (967,1.6733785315735) (968,1.4030077398002) (969,1.5881690218596) (970,1.135423673925) (971,1.2478273902263) (972,1.708362309507) (973,1.4097219150607) (974,1.4615925244707) (975,1.4012847012263) (976,1.4430734506025) (977,1.3298533870955) (978,1.5112357222133) (979,1.5583242050976) (980,1.3687860574555) (981,1.6543524270434) (982,1.468133534922) (983,1.4378851199179) (984,1.5488926427503) (985,1.3137474410094) (986,1.3211697084387) (987,1.3578690395551) (988,1.3375524986549) (989,1.3345333178397) (990,1.5666365231328) (991,1.199354497168) (992,1.4184016833677) (993,1.5881809017289) (994,1.6079973918545) (995,1.5085535719427) (996,1.3277889782824) (997,1.2568681087317) (998,1.3823537673391) (999,1.5142079741266) (1000,1.7042478912037) (1001,1.5161716693) (1002,1.1730289683164) (1003,1.7818434156332) (1004,1.4100729297976) (1005,1.301580130423) (1006,1.2618282696431) (1007,1.537489230462) (1008,1.4535389645899) (1009,1.3649559784526) (1010,1.4127526607514) (1011,1.514732278973) (1012,1.6193381841882) (1013,1.5125636472907) (1014,1.3927631255032) (1015,1.2695004640981) (1016,1.3147199028433) (1017,1.5388024183104) (1018,1.4159579502089) (1019,1.539890676144) (1020,1.4029725958692) (1021,1.557028298529) (1022,1.4177599544788) (1023,1.2789147108973) (1024,1.6345079441764) (1025,1.4150324062759) (1026,1.4873543248831) (1027,1.5964452022625) (1028,1.3861751509445) (1029,1.52557265248) (1030,1.5552729142183) (1031,1.4518993716139) (1032,1.5642252161949) (1033,1.4556179399234) (1034,1.6890701238021) (1035,1.4193011318654) (1036,1.3822592454466) (1037,1.2432432378269) (1038,1.3940143104604) (1039,1.5220656301719) (1040,1.5627847940638) (1041,1.2681531194666) (1042,1.2489196384703) (1043,1.0917951216415) (1044,1.4065705625634) (1045,1.6268949669036) (1046,1.6007902125703) (1047,1.5613028049996) (1048,1.4583953467119) (1049,1.2591207257724) (1050,1.3901383536804) (1051,1.4151183156238) (1052,1.3972567331997) (1053,1.6049293016624) (1054,1.632324534625) (1055,1.3961521373847) (1056,1.390488762596) (1057,1.2966059574799) (1058,1.4542810883413) (1059,1.2432291068895) (1060,1.3868793735476) (1061,1.3445180302936) (1062,1.3849219355186) (1063,1.3387079540676) (1064,1.5383891039142) (1065,1.7032777981362) (1066,1.232553126509) (1067,1.4510220638435) (1068,1.6452480749555) (1069,1.5503508418208) (1070,1.6130901975719) (1071,1.41435904451) (1072,1.4553644113145) (1073,1.3782823380993) (1074,1.2610182789947) (1075,1.2591253391364) (1076,1.4269610620566) (1077,1.3681895266552) (1078,1.6471217127696) (1079,1.5577433250046) (1080,1.2848321270715) (1081,1.4354310509476) (1082,1.2863955475738) (1083,1.5031193281872) (1084,1.7218305848335) (1085,1.4207811449059) (1086,1.2914416844577) (1087,1.5043729408211) (1088,1.7074438521976) (1089,1.4698686880703) (1090,1.2645090840317) (1091,1.2618403038552) (1092,1.5571148939047) (1093,1.6334264623088) (1094,1.1830014889427) (1095,1.4024658727657) (1096,1.4003808770308) (1097,1.4614659377631) (1098,1.1695008429514) (1099,1.7736998689574) (1100,1.3800331930766) (1101,1.3345572234072) (1102,1.5767844469317) (1103,1.9344399268735) (1104,1.1603481809158) (1105,1.3820261097332) (1106,1.4340060795903) (1107,1.4876281209453) (1108,1.2985105644785) (1109,1.3020308343033) (1110,1.2947509623656) (1111,1.5927210611814) (1112,1.5712735501632) (1113,1.5082829757914) (1114,1.490023868604) (1115,1.2948250791786) (1116,1.3047996969642) (1117,1.3558805127975) (1118,1.4185113759375) (1119,1.6179426478581) (1120,1.5311391923219) (1121,1.323363586519) (1122,1.4903385357304) (1123,1.4984471599478) (1124,1.6204998851542) (1125,1.4641511803263) (1126,1.330321099123) (1127,1.3940493733463) (1128,1.3354791054489) (1129,1.304567239542) (1130,1.5607215399005) (1131,1.5141713362432) (1132,1.2905756634046) (1133,1.376497366604) (1134,1.3197313809052) (1135,1.4202029606938) (1136,1.2172149864152) (1137,1.411822763986) (1138,1.2596491462056) (1139,1.4190535229791) (1140,1.36492197788) (1141,1.417938101092) (1142,1.6056753999533) (1143,1.6927630486228) (1144,1.6347114102094) (1145,1.454491117367) (1146,1.3076096461948) (1147,1.3981657323732) (1148,1.3253137354915) (1149,1.4629924321152) (1150,1.2778440803255) (1151,1.631797617441) (1152,1.0994681933574) (1153,1.4183226490477) (1154,1.3870996278221) (1155,1.3426274684528) (1156,1.6187977843259) (1157,1.6238909674086) (1158,1.2926425955028) (1159,1.5321353500562) (1160,1.5132078930649) (1161,1.5735377705805) (1162,1.3479222590656) (1163,1.5106522948882) (1164,1.2851157538577) (1165,1.3968665659598) (1166,1.3260646476158) (1167,1.4374872499177) (1168,1.346609719826) (1169,1.432616628672) (1170,1.5022175033443) (1171,1.5314680923106) (1172,1.4800010521638) (1173,1.5445477237258) (1174,1.3946936716987) (1175,1.3705346253888) (1176,1.5885868339975) (1177,1.6550527225444) (1178,1.1692122989996) (1179,1.3599317467112) (1180,1.6038811999291) (1181,1.8348433182506) (1182,1.6439413895485) (1183,1.393403901472) (1184,1.6777828858062) (1185,1.4976214318511) (1186,1.550223154821) (1187,1.663469604115) (1188,1.4432175805476) (1189,1.4021615236351) (1190,1.6203153878747) (1191,1.3268122184335) (1192,1.344552518053) (1193,1.7351647163755) (1194,1.4638159076005) (1195,1.3930815686163) (1196,1.3881720411438) (1197,1.6252156446578) (1198,1.2400712328216) (1199,1.5123600269422) (1200,1.4761055445817) (1201,1.5015428950991) (1202,1.3619113432807) (1203,1.4290212158009) (1204,1.4002953483594) (1205,1.4891237738483) (1206,1.339577933116) (1207,1.4154456905121) (1208,1.2992301068475) (1209,1.3649754338104) (1210,1.5396910686538) (1211,1.1706751546063) (1212,1.0570394767855) (1213,1.3711966230928) (1214,1.2134085102767) (1215,1.5199121192705) (1216,1.2726430683279) (1217,1.4155974394257) (1218,1.3498489784112) (1219,1.3746084680589) (1220,1.2869974215838) (1221,1.8222646456521) (1222,1.3854085413336) (1223,1.6677110548539) (1224,1.1925330716782) (1225,1.5256400618655) (1226,1.2682714131922) (1227,1.4351321853144) (1228,1.4037277241627) (1229,1.5016679997092) (1230,1.441641644641) (1231,1.2688132380909) (1232,1.41782539728) (1233,1.4520288047593) (1234,1.6163568340464) (1235,1.5046098935201) (1236,1.4105055209755) (1237,1.4120269010681) (1238,1.4299645927778) (1239,1.460123116232) (1240,1.4213375307765) (1241,1.4096931185367) (1242,1.3977877430536) (1243,1.4343568979996) (1244,1.8563547017562) (1245,1.4914576613799) (1246,1.4259986015195) (1247,1.4578321963423) (1248,1.5766210737437) (1249,1.3973528933144) (1250,1.1490730909785) (1251,1.5220236134589) (1252,1.3442505192694) (1253,1.6601870656865) (1254,1.6217993421611) (1255,1.498722188453) (1256,1.4037493207935) (1257,1.4979568111111) (1258,1.3613337900184) (1259,1.3700432656527) (1260,1.3106382770044) (1261,1.6601475582485) (1262,1.3267208377405) (1263,1.3448725523078) (1264,1.4547696332422) (1265,1.6125426767665) (1266,1.5311730750455) (1267,1.6388868385211) (1268,1.4121778504459) (1269,1.3698892350209) (1270,1.5459498104524) (1271,1.5382288319366) (1272,1.6411623894524) (1273,1.5853099193297) (1274,1.4988890982214) (1275,1.3904559602216) (1276,1.3915207021479) (1277,1.5401718652463) (1278,1.2788503244928) (1279,1.4029995819951) (1280,1.2951643946203) (1281,1.1702909631745) (1282,1.390800188599) (1283,1.5387601510101) (1284,1.531358479833) (1285,1.3850149968805) (1286,1.5893217932935) (1287,1.1215136907569) (1288,1.235733567818) (1289,1.2424626896687) (1290,1.1613394124987) (1291,1.504398914217) (1292,1.5199259489066) (1293,1.4659647029714) (1294,1.4247914147918) (1295,1.4476349519096) (1296,1.3177683031011) (1297,1.6760637990403) (1298,1.3723290104762) (1299,1.3185580181966) (1300,1.181495437339) (1301,1.5157728143252) (1302,1.3834285155186) (1303,1.4760345691198) (1304,1.3001618381523) (1305,1.718599188064) (1306,1.264158738293) (1307,1.4918731582618) (1308,1.1894072603979) (1309,1.3987748209051) (1310,1.4072318884728) (1311,1.0643559256227) (1312,1.3593112465498) (1313,1.4023065532271) (1314,1.4790690765498) (1315,1.5634221142376) (1316,1.2768492244827) (1317,1.5983830344122) (1318,1.3627681826746) (1319,1.8205950533741) (1320,1.2961210551527) (1321,1.4714163739633) (1322,1.4480682944912) (1323,1.4182866070081) (1324,1.634511780515) (1325,1.8094572233059) (1326,1.6977702912966) (1327,1.4674738755731) (1328,1.4944075892585) (1329,1.4919953106485) (1330,1.3843274608754) (1331,1.6311452891352) (1332,1.4545429048718) (1333,1.2588539428989) (1334,1.4545915815852) (1335,1.3686518233994) (1336,1.5069121453051) (1337,1.4352035492108) (1338,1.2564788539016) (1339,1.3561964110939) (1340,1.2276768186892) (1341,1.528514279842) (1342,1.4810323347503) (1343,1.5432791679489) (1344,1.6476050500331) (1345,1.4944487602015) (1346,1.7163696012356) (1347,1.5039441013004) (1348,1.4623088483039) (1349,1.6539081436904) (1350,1.3359169568179) (1351,1.5978026490994) (1352,1.5705022498093) (1353,1.3759541057593) (1354,1.3818941625978) (1355,1.6003088231436) (1356,1.3567601841278) (1357,1.6705518369652) (1358,1.548016141816) (1359,1.6893152311459) (1360,1.2885442013836) (1361,1.6197664118616) (1362,1.4530083693596) (1363,1.2887367980703) (1364,1.3433101355816) (1365,1.3466994906781) (1366,1.4145413972643) (1367,1.7176351872367) (1368,1.4318183494899) (1369,1.5840615182978) (1370,1.3620143273994) (1371,1.6134535653548) (1372,1.5097678261355) (1373,1.2506378226226) (1374,1.6491847175034) (1375,1.5170690361617) (1376,1.3726549926748) (1377,1.706185557172) (1378,1.2776763582487) (1379,1.261741252241) (1380,1.4299185736681) (1381,1.4619319610802) (1382,1.3868156884174) (1383,1.536659670547) (1384,1.5021083841716) (1385,1.3135074832402) (1386,1.6933311032971) (1387,1.3602913498542) (1388,1.335554917019) (1389,1.571876745458) (1390,1.3854354661351) (1391,1.1418146628062) (1392,1.3350841296206) (1393,1.6894058443296) (1394,1.2695168456493) (1395,1.4861390283937) (1396,1.3857230762536) (1397,1.3050962745081) (1398,1.3376678106959) (1399,1.4636798164186) (1400,1.4252511518369) (1401,1.6850151698437) (1402,1.4168134995455) (1403,1.8308876606765) (1404,1.4367575989951) (1405,1.6620900483874) (1406,1.2876915439233) (1407,1.1235964528727) (1408,1.3822845856204) (1409,1.3151072338336) (1410,1.5372079225201) (1411,1.1315614749355) (1412,1.6343768397378) (1413,1.5742021607756) (1414,1.4003659262121) (1415,1.4633572469523) (1416,1.6873307740491) (1417,1.5949615494038) (1418,1.5357050939525) (1419,1.6378614646606) (1420,1.3765993939098) (1421,1.6868478983763) (1422,1.7292136500199) (1423,1.6408159289125) (1424,1.4376307912157) (1425,1.2474614010911) (1426,1.3977186273803) (1427,1.4391800140076) (1428,1.5926636051207) (1429,1.592630892241) (1430,1.5096320108434) (1431,1.3567736178587) (1432,1.3402325996224) (1433,1.4548317961791) (1434,1.4593825536265) (1435,1.4288917931992) (1436,1.5240626303228) (1437,1.3040875014857) (1438,1.271908897299) (1439,1.254647342183) (1440,1.4946042523355) (1441,1.439637589451) (1442,1.4248203876589) (1443,1.3357793293602) (1444,1.3543814914369) (1445,1.1312579091052) (1446,1.4941365278915) (1447,1.5821553448161) (1448,1.5128594258692) (1449,1.431300675661) (1450,1.5082354347992) (1451,1.2522625919993) (1452,1.4662408532394) (1453,1.5210175427952) (1454,1.2893538979024) (1455,1.311252655682) (1456,1.5105384545652) (1457,1.4319951147649) (1458,1.7059484666154) (1459,1.626524627644) (1460,1.280152519414) (1461,1.5196419215576) (1462,1.2930188124885) (1463,1.6194920286583) (1464,1.4088399423127) (1465,1.4041274699311) (1466,1.3909737491904) (1467,1.5659668711794) (1468,1.7311661909134) (1469,1.4445359549747) (1470,1.4363770458945) (1471,1.7112669079095) (1472,1.2822278678581) (1473,1.4350974934513) (1474,1.1930968122421) (1475,1.680381091697) (1476,1.594311699445) (1477,1.6255061495235) (1478,1.8107408780514) (1479,1.576258710277) (1480,1.7367725491727) (1481,1.3568857467375) (1482,1.3565619994085) (1483,1.5463710436552) (1484,1.5186089500955) (1485,1.4344558369638) (1486,1.1977889318916) (1487,1.3718488565142) (1488,1.4838508053041) (1489,1.5100161913) (1490,1.6349498499872) (1491,1.4184772227136) (1492,1.844525378383) (1493,1.5269025997755) (1494,1.3749762472047) (1495,1.5039658051229) (1496,1.4280218284299) (1497,1.6181779994151) (1498,1.6027554791154) (1499,1.3676948978556) (1500,1.3443786955499) (1501,1.7583987929951) (1502,1.6408070689637) (1503,1.4358344508759) (1504,1.2463383292825) (1505,1.4958742200959) (1506,1.5841440042513) (1507,1.4413827036613) (1508,1.7004360707031) (1509,1.635870112407) (1510,1.8967785486711) (1511,1.4690615729109) (1512,1.6770182746309) (1513,1.423990275537) (1514,1.1079526794215) (1515,1.286364010475) (1516,1.3879827440822) (1517,1.6215064015924) (1518,1.3868995774082) (1519,1.6714498915835) (1520,1.3513282451981) (1521,1.4975767016487) (1522,1.4539725665303) (1523,1.6349314078817) (1524,1.4321708877746) (1525,1.5427565582082) (1526,1.7083041313336) (1527,1.4702088031808) (1528,1.4374384688165) (1529,1.5318398379521) (1530,1.4856310439149) (1531,1.6224914764103) (1532,1.5927743358091) (1533,1.5903269447788) (1534,1.4166257061824) (1535,1.5120283372056) (1536,1.3301935774474) (1537,1.4157074097164) (1538,1.3997329796111) (1539,1.4216191202111) (1540,1.5861659810523) (1541,1.4433305213711) (1542,1.1850898233085) (1543,1.3791289880143) (1544,1.340122179154) (1545,1.2241234900244) (1546,1.3209985585723) (1547,1.2909669478752) (1548,1.2984373437651) (1549,1.2054478427764) (1550,1.4015543081231) (1551,1.289836172919) (1552,1.6246132310308) (1553,1.7923761667744) (1554,1.7504432039354) (1555,1.4480610511763) (1556,1.1856440539213) (1557,1.3963353003317) (1558,1.8977441545955) (1559,1.6272579083641) (1560,1.4447846559857) (1561,1.6315650109971) (1562,1.4044318968472) (1563,1.7088323422355) (1564,1.3319653736663) (1565,1.3779827340887) (1566,1.560946925509) (1567,1.4195784689867) (1568,1.6422930568085) (1569,1.5135083964237) (1570,1.2175566760632) (1571,1.2566719689846) (1572,1.663289482923) (1573,1.5587315523261) (1574,1.4812581558615) (1575,1.3664619957505) (1576,1.6208468536675) (1577,1.4951742545544) (1578,1.5549483993804) (1579,1.4384459705604) (1580,1.2315860283779) (1581,1.5239187371262) (1582,1.405121588266) (1583,1.6783720517899) (1584,1.2958113621499) (1585,1.3184447927518) (1586,1.5547563355625) (1587,1.5139969112409) (1588,1.502070626827) (1589,1.4531456059703) (1590,1.3745854140932) (1591,1.3038858033348) (1592,1.4307964500595) (1593,1.649049417734) (1594,1.4580830521481) (1595,1.388127046188) (1596,1.5162483605762) (1597,1.3684815916196) (1598,1.5852854784545) (1599,1.4165303760523) (1600,1.3648017368318) (1601,1.2882674959968) (1602,1.4695416578659) (1603,1.5768748452541) (1604,1.4367121174851) (1605,1.2680310292581) (1606,1.4570472053695) (1607,1.2555825573341) (1608,1.6053174725136) (1609,1.4591996725059) (1610,1.374372905955) (1611,1.6170128312907) (1612,1.6401104283944) (1613,1.6918860647353) (1614,1.3601004986156) (1615,1.422568735872) (1616,1.5571642101121) (1617,2.0327443077091) (1618,1.3245087746086) (1619,1.7477701455529) (1620,1.3635390811565) (1621,1.3219194869191) (1622,1.3291645036536) (1623,1.2939100906684) (1624,1.2096362563981) (1625,1.3747255800437) (1626,1.3315421715493) (1627,1.3928914663511) (1628,1.2362099183497) (1629,1.4538401566073) (1630,1.4084056582691) (1631,1.4646009757144) (1632,1.6427832348331) (1633,1.3041437812872) (1634,1.2793827822927) (1635,1.2494025060158) (1636,1.2956745688616) (1637,1.2962649068662) (1638,1.7963764407302) (1639,1.2037083138904) (1640,1.4207165782277) (1641,1.2154462945738) (1642,1.5809388171097) (1643,1.3428960380194) (1644,1.4013681712056) (1645,1.4978783923692) (1646,1.5161314158527) (1647,1.5061797749255) (1648,1.286117314943) (1649,1.3489121651334) (1650,1.3878730528821) (1651,1.4772278905059) (1652,1.475626705889) (1653,1.5489391295942) (1654,1.3582247278469) (1655,1.4022276758621) (1656,1.4021772441823) (1657,1.3593696417849) (1658,1.4452039126045) (1659,1.4293104687078) (1660,1.5353394960888) (1661,1.3199126666823) (1662,1.5172987559207) (1663,1.2783510271019) (1664,1.4505523136378) (1665,1.3764942645428) (1666,1.1377675654208) (1667,1.4506202554254) (1668,1.2781348130917) (1669,1.471140589945) (1670,1.3658733651687) (1671,1.4262080146476) (1672,1.4283197964981) (1673,1.3879710211678) (1674,1.3846184310057) (1675,1.3507105012574) (1676,1.4707490781731) (1677,0.96232872445216) (1678,1.3303075184029) (1679,1.4591103670156) (1680,1.2753095784261) (1681,1.3066305861224) (1682,1.256318619167) (1683,1.5017641100663) (1684,1.4170488946383) (1685,1.5016497145188) (1686,1.5690730004966) (1687,1.4951183660851) (1688,1.1857494903017) (1689,1.3008000722653) (1690,1.2595664534124) (1691,1.3714500316946) (1692,1.5563794165687) (1693,1.6729931327184) (1694,1.575130905044) (1695,1.460216284634) (1696,1.5954061026717) (1697,1.397107013484) (1698,1.3563414969471) (1699,1.2015215067594) (1700,1.4015390986426) (1701,1.5435809953285) (1702,1.4344583766494) (1703,1.431334992384) (1704,1.5101497198302) (1705,1.4503269191624) (1706,1.5624531195551) (1707,1.3469016030917) (1708,1.2908189680268) (1709,1.2160863567489) (1710,1.4352058227597) (1711,1.2851584717207) (1712,1.3702269380114) (1713,1.361782850267) (1714,1.3079642260048) (1715,1.4179096390156) (1716,1.4169961953701) (1717,1.7152192867451) (1718,1.1870484560899) (1719,1.5380442891643) (1720,1.4629372769016) (1721,1.2667129615243) (1722,1.414181995869) (1723,1.2711203588223) (1724,1.4951719161247) (1725,1.6423713113776) (1726,1.5068588230728) (1727,1.3978865873642) (1728,1.393858355997) (1729,1.3981311222209) (1730,1.4381170810801) (1731,1.4239182528171) (1732,1.3568382070572) (1733,1.4123100550265) (1734,1.511693023067) (1735,1.5796452745627) (1736,1.1868099099181) (1737,1.3827637430666) (1738,1.8682573431473) (1739,1.3855455747191) (1740,1.2010270829589) (1741,1.2573669641119) (1742,1.283575895252) (1743,1.5236432304769) (1744,1.6300740180694) (1745,1.4036983821653) (1746,1.2529020428846) (1747,1.3443566908326) (1748,1.5726800983725) (1749,1.3287449278496) (1750,1.353967618994) (1751,1.5262084125683) (1752,1.3701187647842) (1753,1.6210357496507) (1754,1.5014200818899) (1755,1.3059826654509) (1756,1.3633088825963) (1757,1.5169997188055) (1758,1.4331664148266) (1759,1.4367550520929) (1760,1.2408497901834) (1761,1.3847190605712) (1762,1.2088860296696) (1763,1.3149471491363) (1764,1.6386723723033) (1765,1.3223922982184) (1766,1.2225847358239) (1767,1.5006632265207) (1768,1.3462607445923) (1769,1.1465597967723) (1770,1.3712885340318) (1771,1.5043138508479) (1772,1.7032274849613) (1773,1.461250681665) (1774,1.4266380481893) (1775,1.4312825768173) (1776,1.5338545914061) (1777,1.4887262118648) (1778,1.4874127675963) (1779,1.415946419338) (1780,1.5566847676451) (1781,1.402790649019) (1782,1.6409693656623) (1783,1.2745548212458) (1784,1.4273771168309) (1785,1.2793698008891) (1786,1.5335514311947) (1787,1.4939081262789) (1788,1.508360345392) (1789,1.7937443396451) (1790,1.3508656733275) (1791,1.4122465384577) (1792,1.6994861802396) (1793,1.5948810055808) (1794,1.330906719212) (1795,1.5572346133884) (1796,1.481382571842) (1797,1.416578257183) (1798,1.343412018505) (1799,1.5012839087063) (1800,1.4106169415784) (1801,1.2996040404411) (1802,1.366516323652) (1803,1.3230694447172) (1804,1.4031075070172) (1805,1.2637669210667) (1806,1.295320621787) (1807,1.3475192622951) (1808,1.3000528661101) (1809,1.0581112535744) (1810,1.2538116049197) (1811,1.3253644143798) (1812,1.4831767790113) (1813,1.1866126812828) (1814,1.6129567532404) (1815,1.5780717120722) (1816,1.7106602270832) (1817,1.2844303888081) (1818,1.4731257326322) (1819,1.5437683420464) (1820,1.5295053050664) (1821,1.4715835524514) (1822,1.5039594305702) (1823,1.523072473317) (1824,1.529677287837) (1825,1.5522218388678) (1826,1.6970398406199) (1827,1.3752940279255) (1828,1.5961150309266) (1829,1.4235799661308) (1830,1.3929732092655) (1831,1.366716547732) (1832,1.5303135616394) (1833,1.2101899107874) (1834,1.3634716024679) (1835,1.458784799047) (1836,1.4126175121094) (1837,1.7501311279454) (1838,1.4759260086021) (1839,1.4895226701842) (1840,1.6127176693825) (1841,1.3885168853354) (1842,1.502293651468) (1843,1.7594231564327) (1844,1.7309563559497) (1845,1.4024468737339) (1846,1.3803780353713) (1847,1.5140348845923) (1848,1.6790116252154) (1849,1.2661588250596) (1850,1.6338848314349) (1851,1.3884779356182) (1852,1.3832505690398) (1853,1.3283847119584) (1854,1.419519047649) (1855,1.4199276421008) (1856,1.3745464830629) (1857,1.4010244330283) (1858,1.5809795312182) (1859,1.6334611496731) (1860,1.2851836613835) (1861,1.5976299875807) (1862,1.6634256817992) (1863,1.3805169683418) (1864,1.2147211580648) (1865,1.3030318556861) (1866,1.4163812626229) (1867,1.5397400147132) (1868,1.4612645157134) (1869,1.4708755193014) (1870,1.5509622637052) (1871,1.2826221302285) (1872,1.5865582493909) (1873,1.301081662326) (1874,1.2698057452303) (1875,1.2379739481768) (1876,1.6337473619323) (1877,1.2142147530464) (1878,1.534582220001) (1879,1.6122568903516) (1880,1.6851191843935) (1881,1.276599887068) (1882,1.3801165163579) (1883,1.6018675847626) (1884,1.3866504081143) (1885,1.6150661098262) (1886,1.7472070857152) (1887,1.4295743313726) (1888,1.4671609671021) (1889,1.4092740887901) (1890,1.6010258664315) (1891,1.4154865443103) (1892,1.2802253889027) (1893,1.4842223819633) (1894,1.4881814990779) (1895,1.5315102026064) (1896,1.2895590289632) (1897,1.3309317611921) (1898,1.3531496204846) (1899,1.6324847765892) (1900,1.4592015031212) (1901,1.2599034556845) (1902,1.7501116517222) (1903,1.4239627092433) (1904,1.3147840008079) (1905,1.4735131182247) (1906,1.4313473049098) (1907,1.3447520219082) (1908,1.5450535378384) (1909,1.2918436265835) (1910,1.2060261068738) (1911,1.3123857121309) (1912,1.2021637006228) (1913,1.5329998611066) (1914,1.2658101523485) (1915,1.3934440610689) (1916,1.3415516856172) (1917,1.3119677654667) (1918,1.2048752466197) (1919,1.7480749336359) (1920,1.4593124286112) (1921,1.3228662818081) (1922,1.2890126044997) (1923,1.5473301740234) (1924,1.3441962728064) (1925,1.3692236718474) (1926,1.4835942855397) (1927,1.4328691753031) (1928,1.4627821674515) (1929,1.5134625597764) (1930,1.3451192343865) (1931,1.6324813392124) (1932,1.5401839194316) (1933,1.3467144643771) (1934,1.4405462668245) (1935,1.5793947536754) (1936,1.4774392327008) (1937,1.3091496042244) (1938,1.463425681374) (1939,1.3080845201459) (1940,1.5428852689994) (1941,1.3501759000923) (1942,1.3132268133194) (1943,1.2929155009421) (1944,1.404918601469) (1945,1.411630111774) (1946,1.333720125716) (1947,1.1636246529551) (1948,1.2277578098375) (1949,1.160276414736) (1950,1.7279925455762) (1951,1.3555675270536) (1952,1.3526499194385) (1953,1.3774380187184) (1954,1.4779343526023) (1955,1.3355868985385) (1956,1.4421929535913) (1957,1.4639680742251) (1958,1.7004533527796) (1959,1.3265599227706) (1960,1.4206899951392) (1961,1.3230483293641) (1962,1.3163435753414) (1963,1.6822489529071) (1964,1.5725223040833) (1965,1.3846737612738) (1966,1.3771152463457) (1967,1.5039813750108) (1968,1.4741157943187) (1969,1.4315609992396) (1970,1.3589410418051) (1971,1.5154414457152) (1972,1.6100755364483) (1973,1.1242974021433) (1974,1.4776729725699) (1975,1.5373703808082) (1976,1.3319547478558) (1977,1.5000334097696) (1978,1.6421682396491) (1979,1.3925414919947) (1980,1.6592664391999) (1981,1.4309175813451) (1982,1.5672295063386) (1983,1.054161008163) (1984,1.3466561977572) (1985,1.5190821473431) (1986,1.4351861923687) (1987,1.3727823244393) (1988,1.3458682777021) (1989,1.368144187065) (1990,1.359140274165) (1991,1.6537589636277) (1992,1.1137231433148) (1993,1.5029182814618) (1994,1.6850091383541) (1995,1.6800856446983) (1996,1.321907130358) (1997,1.5040489021968) (1998,1.5550506757337) (1999,1.4796155746607) (2000,1.6427307386248) };
\addplot+[line width=2pt, mark=none] coordinates { (1,7.2269870138007) (2,2.1007493751212) (3,3.8191321407036) (4,1.8914959098733) (5,3.9229613598553) (6,1.989575047743) (7,2.4644291931702) (8,1.526253081831) (9,2.1389350712549) (10,1.6969021088443) (11,2.4132348022948) (12,1.5488989938505) (13,2.5226578168045) (14,1.9900668829672) (15,2.5551659546292) (16,1.8215521714943) (17,2.262620272592) (18,1.7250012201549) (19,2.080120125974) (20,1.696535432898) (21,1.7070046611547) (22,1.6417130382542) (23,2.2214093819611) (24,1.7300377035304) (25,2.3555384897611) (26,1.5500619000007) (27,2.2576834102408) (28,1.7046090824068) (29,2.5178045261498) (30,1.7320555245629) (31,2.1587016806349) (32,1.6099752060862) (33,1.7216228909728) (34,1.7924428562096) (35,1.6670334176216) (36,2.0659081238291) (37,1.9250520031296) (38,1.7028684610614) (39,1.8121818559266) (40,2.1758237884368) (41,1.8565136413465) (42,2.2847554476504) (43,1.79449623305) (44,1.8334307597013) (45,1.5848751401172) (46,2.4248913507336) (47,1.869200016928) (48,1.9245808453841) (49,1.701014487639) (50,2.1644088698722) (51,1.7392314260182) (52,2.094898802065) (53,1.8639570540511) (54,1.7748857131158) (55,1.5942749813346) (56,1.9204524546344) (57,1.6138860909649) (58,1.6621038438364) (59,1.8590935441913) (60,2.0463894323349) (61,1.8065755486649) (62,1.800511899631) (63,1.8812108717851) (64,1.9273898379792) (65,1.8651106105454) (66,1.7243821770998) (67,2.1732140697065) (68,1.3896420459725) (69,2.3143482825215) (70,1.7871830482351) (71,1.6929815913754) (72,1.5146462982339) (73,2.2313750790721) (74,1.6127137389739) (75,2.0491239248751) (76,1.4470869825494) (77,1.9983114079638) (78,1.4982322108462) (79,1.7791712358361) (80,1.8077864478405) (81,1.6783198375799) (82,1.8341124288858) (83,1.5872310973617) (84,2.2354018448252) (85,1.7816243168141) (86,1.8931753581304) (87,1.8425945068476) (88,2.0635745127204) (89,1.5956149487085) (90,2.2788424793105) (91,1.6581112652094) (92,1.6780905666666) (93,1.61131745782) (94,1.7798323335348) (95,2.0326592339788) (96,1.537928477584) (97,1.9954681945203) (98,1.8098640624506) (99,1.7137985397396) (100,2.4056915420825) (101,1.5643179175728) (102,2.0790664585876) (103,1.4458466014765) (104,1.9618035032545) (105,1.6831318565323) (106,1.8452160935367) (107,1.4104073599943) (108,2.0479928198313) (109,1.6842407636135) (110,1.494678212736) (111,1.8673226947889) (112,1.5970111703902) (113,1.6646884037528) (114,1.5133138456691) (115,1.8226159701998) (116,1.7125102638468) (117,1.895742581695) (118,1.4096997628875) (119,1.9202269068264) (120,1.5449556154927) (121,2.3566994086875) (122,1.4397496415095) (123,1.7762266623646) (124,1.2567746007689) (125,1.726056468535) (126,1.6359214166319) (127,2.0195788828175) (128,1.7420444763136) (129,1.7486470832478) (130,1.5950797588502) (131,1.8283856481115) (132,1.571785853364) (133,1.8051430381364) (134,1.5797980871015) (135,1.348659823691) (136,1.9439271413721) (137,1.7727761741634) (138,1.8015053419001) (139,1.5979643615925) (140,1.5692236477699) (141,1.9834048358279) (142,1.5711728249226) (143,1.5968318480913) (144,1.5682039123466) (145,1.947165667619) (146,1.580632332091) (147,1.7341809369574) (148,1.8208572362589) (149,1.5998811914976) (150,1.6315725237339) (151,1.9797718621281) (152,1.5436805892357) (153,1.6991918144786) (154,1.5948924375489) (155,1.7859764603226) (156,1.5884210923152) (157,1.5844916148558) (158,1.6910003204334) (159,1.4255610479195) (160,1.9433103362795) (161,1.3704109960806) (162,1.4086033926455) (163,1.7271060574668) (164,1.3811677610263) (165,1.9841598736809) (166,1.538293388113) (167,1.7473447186355) (168,1.3762470920978) (169,1.2923326211959) (170,2.3186511720158) (171,1.5446575256203) (172,1.7722587853704) (173,1.5278172461074) (174,1.6094377714787) (175,1.6020564543773) (176,2.196573163787) (177,1.4926813696674) (178,1.8684921785546) (179,1.4056475049282) (180,1.757684988735) (181,1.3959242275579) (182,1.8746486802654) (183,1.1948722760636) (184,1.6975090310191) (185,1.5607614076907) (186,1.3413964843484) (187,1.5310992190208) (188,1.4304067988434) (189,1.6898814492772) (190,1.7013779584438) (191,1.6099399076706) (192,1.8160380714114) (193,1.3226318782173) (194,1.4646650565472) (195,1.4086660659252) (196,1.7475474563742) (197,1.8181636871027) (198,1.9795764997101) (199,1.5001465546724) (200,2.0838085457272) (201,1.6101873258232) (202,2.0543762010558) (203,1.4124890293867) (204,1.5958420801964) (205,1.6306707531399) (206,1.6883519592306) (207,1.4223313640548) (208,1.5925159296787) (209,1.511374609288) (210,1.6576825420233) (211,1.2799813435749) (212,1.8647066766213) (213,1.7701695619899) (214,1.5243196228628) (215,1.5413457493271) (216,1.3915472447852) (217,1.3381665681311) (218,2.0239026871297) (219,1.3973885343829) (220,1.9568681588873) (221,1.7513513810419) (222,1.9703821499518) (223,1.509559820875) (224,1.9661177966095) (225,1.4884545931972) (226,1.7849969831204) (227,1.5820229429698) (228,1.6543320393667) (229,1.3382660238086) (230,2.1035672803661) (231,1.3517776417884) (232,1.9972740081142) (233,1.7851151628321) (234,1.5743576795964) (235,1.5044330841025) (236,1.5933593028438) (237,1.6634622824238) (238,1.684986644316) (239,1.5893118095717) (240,1.4603424535279) (241,1.6447812572065) (242,1.8320410851389) (243,1.4235128607713) (244,1.4156926158286) (245,1.9438245341631) (246,1.3162229740922) (247,1.8402542338859) (248,1.7892656343063) (249,1.5776836452936) (250,1.2568905107346) (251,1.5846794036807) (252,1.6780180611976) (253,1.4151695667834) (254,1.8922101709838) (255,1.4127207569624) (256,1.6169897255968) (257,1.6174979292602) (258,1.5007306053923) (259,1.6614989886644) (260,1.6085927431053) (261,1.9901222006128) (262,1.2987659856941) (263,2.2556148341656) (264,1.598920218049) (265,1.5644902015156) (266,1.4713861445554) (267,1.7976998354764) (268,1.5012665044156) (269,1.611246274578) (270,1.6525883222122) (271,1.724556084186) (272,1.4121833896335) (273,2.1364285614286) (274,1.4545058347502) (275,1.686630536899) (276,1.4817868057874) (277,1.5708271190963) (278,1.5524794740607) (279,1.5120859814449) (280,2.1198174273886) (281,1.5677209412473) (282,1.4275625828237) (283,2.2339638203148) (284,1.6306993213157) (285,2.5285074579475) (286,1.5002624176777) (287,1.7406404611869) (288,2.0171741277861) (289,1.5722218435567) (290,1.6257624529589) (291,1.7120278707398) (292,1.696607730761) (293,1.500540538661) (294,1.6756708525202) (295,1.4516050817271) (296,1.8395438086423) (297,1.3958352735306) (298,1.966753973942) (299,1.5086481308276) (300,1.8473251560679) (301,1.239271757639) (302,1.8028781232031) (303,1.4148304557358) (304,1.8234296705377) (305,1.6053966916209) (306,1.804303434263) (307,1.6271180710468) (308,1.7021815026484) (309,1.4030473103889) (310,1.909461998249) (311,1.6542864740809) (312,1.6744935216899) (313,1.6641699022652) (314,2.2941898415063) (315,1.5987686168724) (316,1.894264398506) (317,1.4985552973439) (318,1.5798339973503) (319,1.5581091508399) (320,1.6437316115103) (321,1.739313831049) (322,1.3831308833279) (323,1.8442986616799) (324,1.4632935486473) (325,1.802827325792) (326,1.5027932135709) (327,1.5357753155416) (328,1.8108718599062) (329,1.304021296409) (330,2.0956136588696) (331,1.4917329257596) (332,1.7136788283311) (333,1.8193498018168) (334,1.4614205788515) (335,1.9647190173863) (336,1.6874258296605) (337,1.5273231398055) (338,2.1795625008236) (339,1.4521294919828) (340,1.365245027753) (341,1.4862826738406) (342,1.4683028715972) (343,1.6972957319887) (344,2.4150531634138) (345,1.5104092386861) (346,1.8457447385272) (347,1.5047479875005) (348,1.632947767804) (349,2.191973276199) (350,1.3538059770044) (351,1.6179548069428) (352,1.581820077105) (353,1.6953328181146) (354,1.774361474769) (355,1.2750925991364) (356,2.0591322477061) (357,1.3855507252338) (358,1.8166256531653) (359,1.5371598646105) (360,2.1486672027871) (361,1.6450824894565) (362,1.8344098237701) (363,1.8246364675147) (364,1.3030364600611) (365,1.5633639497202) (366,1.4165734589828) (367,1.8142723421505) (368,1.58145641921) (369,1.7243325279029) (370,1.9179670565815) (371,1.3415827563336) (372,1.688755762949) (373,1.4649060375821) (374,1.8383263334265) (375,1.5086098914249) (376,1.7684311267197) (377,1.3556560697149) (378,1.5165391217286) (379,1.4584573560811) (380,1.8320478755812) (381,1.5242567797281) (382,1.6400501398744) (383,1.8946372517968) (384,1.4714254707953) (385,1.5566023781585) (386,1.6958813769196) (387,1.5419485147966) (388,1.4744770885775) (389,2.321689506957) (390,1.3956870813351) (391,2.00713603783) (392,1.4707023234512) (393,1.9612225903095) (394,1.4203866455007) (395,2.0778948313329) (396,1.2996403469432) (397,1.9176725341106) (398,1.7361215293705) (399,1.9100616837857) (400,1.3410324258444) (401,1.6605940341501) (402,1.828148228231) (403,1.7460873745853) (404,1.4970296148412) (405,1.788258565282) (406,1.5850881868811) (407,1.77278790638) (408,1.3601774172441) (409,1.6340553462643) (410,1.3732591919225) (411,1.5230715467684) (412,1.6018897289502) (413,1.8075969819696) (414,1.350066197184) (415,1.5741905041992) (416,1.6045101388297) (417,1.5379464334146) (418,1.9912837923829) (419,1.1999234114778) (420,1.8484305575086) (421,1.3301026344463) (422,1.7796123979678) (423,1.396294397418) (424,1.7915437377904) (425,1.8482499943546) (426,1.6215032381394) (427,1.5939781134941) (428,2.1804424610805) (429,1.32451469278) (430,1.7922253980857) (431,1.7246088160478) (432,1.7888046496104) (433,1.6351533613205) (434,1.6347735527207) (435,1.4917653349318) (436,1.4647802923981) (437,1.5793519252511) (438,2.0257909804533) (439,1.5748815323917) (440,1.4665423940415) (441,2.2752563335557) (442,1.3264418199964) (443,1.6222789161984) (444,1.964024448529) (445,1.5279982454146) (446,1.983690107503) (447,1.6087215711692) (448,1.9089995088806) (449,1.4337070247443) (450,2.4400335142968) (451,1.584344650729) (452,1.896876505858) (453,1.869911706898) (454,1.4436010276134) (455,2.1515916358597) (456,1.5670977441048) (457,1.5262450403791) (458,1.7260780372252) (459,1.573843513723) (460,1.9224137549204) (461,1.6825916829201) (462,2.4718353426806) (463,1.629247643536) (464,2.0588302871527) (465,1.5938190406196) (466,1.4439110230991) (467,1.5706480622783) (468,1.5040471926311) (469,1.5564672095829) (470,1.9481342246969) (471,1.4426703644876) (472,1.7029302756694) (473,1.6038699081533) (474,1.7180686113603) (475,1.8692313385742) (476,1.8126702447861) (477,1.2404883454947) (478,1.6556492268008) (479,1.4964877671742) (480,2.3069845756336) (481,1.3955572497703) (482,1.9529527927379) (483,1.3411049189101) (484,1.7088910292234) (485,1.2889385126764) (486,1.7603672213695) (487,2.0514318627656) (488,1.7480667218045) (489,2.2695892334418) (490,1.4666657034663) (491,1.4970878629228) (492,1.6292093648859) (493,1.6526550490569) (494,1.7515725720905) (495,1.2707771258912) (496,1.5434829987551) (497,2.5431606866399) (498,1.6600121516583) (499,1.6864301325125) (500,1.5557428883134) (501,1.6595323074581) (502,1.5988582426591) (503,1.6693082314473) (504,1.6594113592206) (505,1.7002912573853) (506,2.2976619153852) (507,1.5363478344627) (508,1.7196232671798) (509,1.5454843271821) (510,2.2328107528926) (511,1.9219204522767) (512,1.5611116678112) (513,1.5754449462505) (514,1.9080222899139) (515,1.9300286251523) (516,1.8716692881116) (517,1.8119418977828) (518,1.8178957020002) (519,1.552147499492) (520,2.2059711922411) (521,1.6937445411561) (522,2.0129469042825) (523,1.4476190708123) (524,1.6673862434917) (525,1.8295879939061) (526,1.4624743847967) (527,2.0060850875149) (528,1.5204650935293) (529,1.7694304450313) (530,1.4731275644787) (531,1.9494419356448) (532,1.4966305136137) (533,1.5252840602787) (534,1.4181979461921) (535,1.5077054056031) (536,2.3245138188122) (537,1.8124564821357) (538,1.5297615130456) (539,1.74980831989) (540,1.7037440234623) (541,1.6294420743967) (542,2.0746478677325) (543,1.551350675583) (544,1.7439213198494) (545,1.8705370743265) (546,1.5441044113623) (547,1.3404904883543) (548,2.3337436671544) (549,1.4291961694019) (550,2.1525710054792) (551,1.596467349448) (552,1.5302660748207) (553,1.6163786772566) (554,1.4999700979147) (555,1.6268605235406) (556,1.9547081692336) (557,1.5025065894123) (558,1.3024133136872) (559,1.586345430734) (560,1.7246381548821) (561,1.5865977868286) (562,1.6291653439995) (563,2.0219494005021) (564,1.6129859327974) (565,1.8236645504607) (566,1.5182711727079) (567,1.7119139634428) (568,1.6355063274449) (569,2.3009362910921) (570,1.6060088860376) (571,1.4769049615802) (572,1.673775173642) (573,2.1104118001163) (574,1.5911503106548) (575,1.8783278405073) (576,1.4328545224853) (577,1.6469042581762) (578,1.5982716346897) (579,1.9288887849892) (580,1.4588718739596) (581,1.8418595933098) (582,1.7979667927826) (583,1.7547330592697) (584,1.3826588982406) (585,2.0666451891631) (586,1.4292836160898) (587,1.678854029584) (588,1.5075383410385) (589,2.1144045148811) (590,1.7417497417217) (591,1.618372672055) (592,1.5525522679272) (593,1.630662599587) (594,1.8457678023692) (595,1.5661188173777) (596,2.0753227488644) (597,1.568581256909) (598,1.9049323167185) (599,1.9201098502591) (600,1.4509115653391) (601,1.3521698895264) (602,2.0502508397099) (603,1.574969292132) (604,1.6232524131431) (605,2.0041823589508) (606,1.6654361747834) (607,1.5830454265835) (608,1.707371271092) (609,1.5208470773657) (610,1.7424290529188) (611,1.4480690271947) (612,1.5838684024104) (613,1.7006414549225) (614,1.4459869115517) (615,1.591496653834) (616,1.4776353850597) (617,2.2724282498455) (618,1.5603557234832) (619,1.854610789959) (620,1.5940623791867) (621,2.3178586727644) (622,1.3709011012971) (623,1.6433621528311) (624,2.2503298087569) (625,1.8374387108922) (626,1.8272375121339) (627,1.7782819619098) (628,1.9353138786546) (629,1.6206953556121) (630,2.2060583115436) (631,1.6891090174787) (632,1.1940441952767) (633,1.7058241073455) (634,1.6122670445664) (635,1.5757590070281) (636,1.3266365997488) (637,1.4913489039347) (638,2.1635379790163) (639,1.4934990948218) (640,1.5294166939513) (641,1.7018325712202) (642,1.614327912582) (643,1.9113787087922) (644,1.5755049273447) (645,1.5580420359733) (646,1.5402083129461) (647,1.4808607194966) (648,1.7686501677522) (649,1.867126983207) (650,1.5797664725094) (651,1.6300447138121) (652,1.6153427837553) (653,1.4115291247107) (654,2.2914419212669) (655,1.5674287968628) (656,1.7433376540482) (657,1.6381490109782) (658,1.4254224674) (659,1.6157478505303) (660,2.1064162051657) (661,1.4825089684995) (662,1.5901971800938) (663,1.7671979484543) (664,1.7314448277739) (665,1.9285610815858) (666,1.5502862500445) (667,2.2422315742668) (668,1.4739170760254) (669,1.4024423920578) (670,1.4053959705285) (671,1.5725307683403) (672,1.5599269910653) (673,1.4524389894885) (674,1.3457097917896) (675,1.3628577048647) (676,1.4967160855642) (677,2.197372138683) (678,1.4305197440165) (679,1.9258292469418) (680,1.5201979017881) (681,1.8500981948828) (682,1.5321137086403) (683,1.7288749257171) (684,1.6624150554926) (685,1.4901507260907) (686,1.715731951607) (687,1.4881265461386) (688,1.9959893399805) (689,1.4676264515102) (690,1.6328162289088) (691,1.3939555469778) (692,1.3159436557572) (693,1.5808974305667) (694,1.7979813380151) (695,1.4962418553702) (696,1.8273636706176) (697,1.3660754835138) (698,1.8574577793344) (699,1.6632567657658) (700,1.673254397295) (701,1.6544426335582) (702,1.9804895490718) (703,1.7283463470722) (704,1.6603430339288) (705,1.5855382733793) (706,1.8312671777046) (707,1.654273507189) (708,2.3295956169666) (709,1.3928714931224) (710,1.8604460522355) (711,1.4629033217369) (712,2.5857256047423) (713,1.5434413765042) (714,1.7882154975424) (715,1.6310175663984) (716,1.5345620886541) (717,1.7096675566698) (718,1.7681680409748) (719,1.4212751465793) (720,1.6378345062375) (721,1.9906424113332) (722,1.603253339954) (723,1.3427957845077) (724,1.913764754134) (725,1.7613214958705) (726,1.4295897636723) (727,1.5416918402565) (728,1.6298795275698) (729,2.1208868698992) (730,1.519277751138) (731,1.4797587730456) (732,1.5399454922935) (733,1.5777724996123) (734,1.8777180624568) (735,1.7047609416914) (736,1.5489775116629) (737,1.4908247260064) (738,1.7431127909423) (739,1.6057644293427) (740,2.197853620912) (741,1.7481210519253) (742,1.528900772439) (743,1.4067156130947) (744,1.7392671778111) (745,1.4894854693159) (746,1.5560261106794) (747,1.8879780729525) (748,1.8301079212062) (749,1.6422425379331) (750,1.8706290746955) (751,1.7039265772421) (752,1.3427756925377) (753,1.8734943144416) (754,1.4099005118628) (755,1.5364095589111) (756,1.6959434653701) (757,2.0113905149797) (758,1.5517352770238) (759,1.8605346005077) (760,1.4422042950914) (761,1.7988720443103) (762,1.6595682428958) (763,1.695598309142) (764,1.7778426056939) (765,2.0180645050393) (766,1.4392300362108) (767,1.795040765575) (768,1.5531517969378) (769,1.6855793483584) (770,1.5705884296096) (771,1.7163593823351) (772,1.4396474820709) (773,1.4781217437509) (774,2.459603621986) (775,1.8695835510584) (776,1.6002007504988) (777,1.4791214998229) (778,2.1084288600563) (779,1.6654419651503) (780,1.7275097113535) (781,1.5415055378019) (782,1.4618563602884) (783,1.5722078721722) (784,1.7928786644319) (785,1.5602955696185) (786,1.4284858172161) (787,1.5164017283795) (788,1.4207599333602) (789,1.9447151665978) (790,1.3251495097142) (791,2.5208957160977) (792,1.4937578669812) (793,1.6940522533784) (794,1.6120339904043) (795,2.1781067450563) (796,1.6504956845339) (797,1.4919171247573) (798,1.8461910838902) (799,1.2746170724238) (800,1.4623631025487) (801,1.5854923961165) (802,1.8688390283921) (803,1.5525646478256) (804,1.7835804054835) (805,3.1092383382921) (806,1.8080912596963) (807,1.6010022036663) (808,1.770320970998) (809,1.8249888678947) (810,1.8165818514083) (811,1.3500194712819) (812,1.6399857167728) (813,1.4451945723757) (814,1.9529546665781) (815,1.5301141457496) (816,1.372201379787) (817,1.4701890864777) (818,1.9682018214799) (819,1.279758854741) (820,1.9037245883782) (821,1.7065834057542) (822,1.7340870654654) (823,1.7206847870115) (824,1.7073403441384) (825,1.7119471343431) (826,2.2918040687065) (827,1.6383793350218) (828,1.4143480500321) (829,1.4563938642327) (830,1.6283213533373) (831,1.5298070334309) (832,1.5737344966001) (833,1.6097421054432) (834,1.6741047898206) (835,1.514651422579) (836,1.6246753578341) (837,1.674296218609) (838,1.668421483928) (839,1.8986000670506) (840,2.1555856472779) (841,1.7937158529505) (842,1.4992771837737) (843,1.7083753448442) (844,1.427293706768) (845,1.4584968540873) (846,2.6137667594231) (847,1.764442354649) (848,1.5008438660883) (849,1.5390657804278) (850,1.6636851130546) (851,1.5309472126655) (852,1.4614842618578) (853,2.0670850859504) (854,1.5674822193406) (855,1.4026174934502) (856,1.6226573548059) (857,1.6527962960933) (858,1.6947608415655) (859,1.5139240837318) (860,1.6907434383803) (861,1.8016639252828) (862,1.3178922949398) (863,1.5599870257198) (864,1.7455130148728) (865,1.6316614199072) (866,1.8487917638199) (867,1.1147185420427) (868,1.542398616094) (869,1.7357920662145) (870,1.6241098923691) (871,1.7223256082725) (872,1.7406507434004) (873,1.5236611232897) (874,1.645418740303) (875,1.4433098587675) (876,1.3930450327598) (877,1.4796313672137) (878,1.641261667047) (879,1.6199713758317) (880,1.8636887989833) (881,1.7416480404419) (882,1.6395355696601) (883,1.8414477522889) (884,1.8260821994782) (885,2.0312214432746) (886,1.6095278210919) (887,1.4629030891865) (888,1.5733253373342) (889,1.6035228449165) (890,1.4769556962627) (891,1.5344385361068) (892,1.7671020351368) (893,1.8387277868123) (894,1.9970017143842) (895,1.4246042721513) (896,1.8012530977848) (897,1.6904788356592) (898,1.7530449620772) (899,2.0176822713678) (900,1.4765384990346) (901,1.6369746174014) (902,1.4481443942489) (903,1.6319248800598) (904,1.9095537626524) (905,1.5965188390096) (906,1.8438818290803) (907,1.8833028405641) (908,1.657956498529) (909,1.8585918946017) (910,1.7220096657973) (911,1.7151791687262) (912,1.5603199331324) (913,1.6011694543542) (914,1.4812455456736) (915,1.569874125124) (916,2.1463769285945) (917,1.7775317658644) (918,1.7921503910699) (919,1.3804883367666) (920,2.0542150101991) (921,1.676972001633) (922,1.4169789552413) (923,1.4589058202178) (924,1.3597064766871) (925,1.5881440201224) (926,1.6996896410915) (927,1.4350782137688) (928,1.5698495297749) (929,1.6089450407601) (930,1.8857981730456) (931,1.5154778802136) (932,1.6810603922201) (933,1.6323442729488) (934,1.8564680674302) (935,1.7857223171672) (936,1.7579516511377) (937,1.9188206260909) (938,1.5927782648807) (939,1.8757673191719) (940,1.5085845835953) (941,1.5741904023833) (942,1.7617172677967) (943,1.4227141401896) (944,1.6878169377971) (945,1.6767887775149) (946,1.68009070501) (947,1.5186944127843) (948,1.7228742306628) (949,1.7425434741779) (950,1.7542942848742) (951,1.9409708581422) (952,1.578147840843) (953,1.7974048432289) (954,1.3482559803752) (955,1.6385724533451) (956,1.7974558204977) (957,1.7001284369704) (958,1.9654853519296) (959,1.83695972602) (960,1.8999966030473) (961,1.8647581938254) (962,1.742519874488) (963,1.8975422062986) (964,1.6923446866575) (965,1.8809583418252) (966,1.6659707436286) (967,1.427826938855) (968,1.8736825281552) (969,1.6551707586635) (970,2.1489171371504) (971,1.6533723516774) (972,1.387772209442) (973,1.3633386662592) (974,1.7978042166206) (975,1.5576875591086) (976,1.7444364320022) (977,1.5899559940382) (978,1.764753973215) (979,1.63749798135) (980,1.4039626219739) (981,1.7425538514217) (982,1.701290387659) (983,1.6639576503037) (984,1.4577702377685) (985,1.6662004676939) (986,1.4247138027008) (987,1.7933494443454) (988,1.5741928369234) (989,1.6765806903449) (990,1.7779097522335) (991,1.3704016785717) (992,1.6890874731417) (993,1.4868142854727) (994,1.669051074512) (995,1.5042356316781) (996,1.3787744134228) (997,1.6454336433277) (998,1.593642935653) (999,1.4360328156483) (1000,1.4244593264694) (1001,1.679151262544) (1002,1.6299362502612) (1003,1.8067550179536) (1004,2.0229544050357) (1005,1.5101878365675) (1006,1.6076782288771) (1007,1.137579940439) (1008,1.3147683533847) (1009,1.5206694169068) (1010,1.4361709547708) (1011,1.6303807665833) (1012,1.7135812717809) (1013,1.3467197658266) (1014,1.3475661539833) (1015,1.9300718956518) (1016,1.3980207692496) (1017,1.5276085300917) (1018,1.4071093761853) (1019,1.5803242431637) (1020,1.9738877999173) (1021,1.5836962359053) (1022,2.115975053915) (1023,1.3970983963724) (1024,1.669114806762) (1025,1.5671559027013) (1026,1.5584319641066) (1027,1.7759034461987) (1028,1.7995150961213) (1029,1.4733040961373) (1030,1.6674504562791) (1031,1.7540993748327) (1032,1.6517735269988) (1033,1.3345384353166) (1034,1.5123145912695) (1035,1.4206693279353) (1036,1.4934719161481) (1037,1.6355808060177) (1038,1.9661385895344) (1039,1.5850962491994) (1040,1.8743405181956) (1041,1.5674108708546) (1042,1.3114717682679) (1043,1.6293013377252) (1044,1.4747062002368) (1045,2.155518439097) (1046,1.6544801423995) (1047,1.3624434512621) (1048,1.4978584400753) (1049,1.3608508285293) (1050,1.5110014487376) (1051,1.427480407025) (1052,1.4801401141469) (1053,1.5832009001108) (1054,1.5346261417037) (1055,1.4403252007231) (1056,1.4090725300118) (1057,1.4125662339481) (1058,1.653493006314) (1059,1.4463807799793) (1060,1.3852430193143) (1061,1.5846402989578) (1062,1.7595103599646) (1063,1.4973298470937) (1064,1.82032940313) (1065,1.7091422001709) (1066,1.5362214518328) (1067,1.800811035901) (1068,1.7831332465961) (1069,1.7190444482304) (1070,1.5334151496883) (1071,1.7317837160433) (1072,1.7337578420668) (1073,1.7603316738632) (1074,1.8496543983776) (1075,1.6058726133975) (1076,1.6190147674996) (1077,1.6358190597881) (1078,1.7506933035473) (1079,1.5323071022722) (1080,1.5932161464583) (1081,1.7998424639139) (1082,1.6080116695816) (1083,1.7274389684986) (1084,1.4629011231919) (1085,1.6160466966923) (1086,1.6406128961312) (1087,1.3798823759576) (1088,1.6760004551798) (1089,1.5069960776782) (1090,1.7106302763689) (1091,1.7651911524929) (1092,1.3704723727767) (1093,1.7000121552223) (1094,1.4692404262519) (1095,1.4752936352191) (1096,1.4429273274134) (1097,1.4527350083678) (1098,1.6421501694791) (1099,1.4844728436671) (1100,1.6246235669666) (1101,1.541955788653) (1102,1.656359653935) (1103,1.5814143490528) (1104,1.4357036803566) (1105,1.6804200548835) (1106,1.2196490364055) (1107,1.4144828959452) (1108,1.7004401783968) (1109,2.0677782081209) (1110,1.8607338762807) (1111,1.3641185587291) (1112,1.5723072609885) (1113,1.8230323222768) (1114,1.8528142697994) (1115,1.4652363182024) (1116,1.5628428167033) (1117,1.6924683082092) (1118,1.7598786558061) (1119,1.9753017485375) (1120,1.3344559639837) (1121,2.0829750869147) (1122,1.4455413038355) (1123,1.334258609853) (1124,1.418150992335) (1125,1.4456563397933) (1126,1.6462949213077) (1127,1.5799315577877) (1128,1.5948949549024) (1129,1.649425070783) (1130,2.2278087363124) (1131,1.7302388264461) (1132,1.6924399452471) (1133,1.3863540392222) (1134,1.5787041280332) (1135,1.6055861684437) (1136,1.795483227325) (1137,1.8505077154451) (1138,2.1140905825215) (1139,1.625589814663) (1140,1.9528846412263) (1141,1.8374480811228) (1142,1.7526097013843) (1143,1.7035928812779) (1144,1.8479360402556) (1145,1.509791310649) (1146,1.7512085077486) (1147,1.6561459790235) (1148,1.6607092523419) (1149,1.2257563575068) (1150,1.2723457299266) (1151,1.6085707699312) (1152,1.6754300716754) (1153,1.4882718714405) (1154,1.5831726359843) (1155,1.5530222502403) (1156,1.1847138372083) (1157,1.7567431003531) (1158,1.4452028580912) (1159,1.7302644256624) (1160,1.624535714604) (1161,1.6109794943866) (1162,1.6586244045268) (1163,1.6346397099438) (1164,1.6990441748118) (1165,1.5558568837175) (1166,1.8704556281011) (1167,1.8692613418741) (1168,1.3100925090956) (1169,1.1828847846782) (1170,1.6887924587222) (1171,1.232082237841) (1172,1.5399867666124) (1173,1.5300385892088) (1174,1.5648929992553) (1175,1.5760239692986) (1176,1.4967660591382) (1177,1.6881181712485) (1178,1.6013210010587) (1179,1.6377202449153) (1180,1.4996803554986) (1181,1.8608477944128) (1182,1.5861695627807) (1183,1.5395705830656) (1184,1.5409199257449) (1185,1.5766905833379) (1186,1.5324736732166) (1187,1.7985567547593) (1188,1.6158155047586) (1189,1.6269899732811) (1190,1.6243112112085) (1191,1.3297625851336) (1192,1.6749581245913) (1193,1.7179257290221) (1194,1.5402516609933) (1195,1.5137971110977) (1196,1.6684987169566) (1197,1.4520230901903) (1198,1.4061097574149) (1199,1.4629247612529) (1200,1.7264871195668) (1201,1.7863799673545) (1202,1.6894755160682) (1203,1.7000044811492) (1204,1.5280541899011) (1205,1.5865493459235) (1206,2.1020644570927) (1207,1.6416674452242) (1208,1.597229795934) (1209,1.6121541298655) (1210,1.4908015853673) (1211,1.4141874151741) (1212,1.5354359010788) (1213,1.6036386779507) (1214,1.5559770410787) (1215,1.7872620099233) (1216,1.5877283633852) (1217,1.5403386959289) (1218,2.287976832723) (1219,1.5873732548487) (1220,1.927970043735) (1221,1.585487323041) (1222,1.7158139624566) (1223,1.5691254359738) (1224,1.4416312707572) (1225,1.7732178640903) (1226,1.9394662149539) (1227,1.7496224098623) (1228,1.5788710370007) (1229,1.6334085427599) (1230,1.8915170372586) (1231,1.8186703826231) (1232,1.743054289313) (1233,1.7979908658146) (1234,1.8133963774302) (1235,1.8631719621927) (1236,2.0528540373341) (1237,1.560331870516) (1238,1.3770211534385) (1239,1.5860233922789) (1240,1.9562220227497) (1241,1.9478781998459) (1242,2.0888159727943) (1243,1.7861859057518) (1244,1.8572199268981) (1245,2.2478026794523) (1246,1.4811524315548) (1247,1.9493290321312) (1248,1.7385332539413) (1249,1.6638138779024) (1250,1.6616067356331) (1251,1.9913720877506) (1252,1.7688359629401) (1253,1.6010520709557) (1254,1.6479684046589) (1255,1.8828475920332) (1256,1.3608548340408) (1257,1.6475851264764) (1258,1.7728481533329) (1259,1.6892181214682) (1260,1.5568402418299) (1261,1.7147078017773) (1262,1.9481660247979) (1263,2.0590522346853) (1264,1.4889669494772) (1265,1.7551529520566) (1266,1.6809254819549) (1267,1.8255139280686) (1268,1.5098676527881) (1269,1.6201573789781) (1270,1.4195912769018) (1271,1.535419568299) (1272,1.852134307476) (1273,1.7810931127906) (1274,1.6874291893875) (1275,1.5518844414136) (1276,1.7233163296118) (1277,1.4273212775409) (1278,1.8305160225753) (1279,1.4180317932533) (1280,2.1019311649154) (1281,1.3820013157133) (1282,1.3692080194581) (1283,1.4239442616537) (1284,1.8564444693841) (1285,1.3951444765628) (1286,1.6210404316035) (1287,1.547715085697) (1288,1.242599199116) (1289,1.6771335355846) (1290,1.802904866103) (1291,1.7227896438522) (1292,1.4689293005273) (1293,1.564732011062) (1294,1.8859448915749) (1295,1.8201638019372) (1296,1.4793115501255) (1297,1.5723783154621) (1298,1.5004498813421) (1299,1.7445692799723) (1300,1.2727027072256) (1301,1.3334313286801) (1302,1.5595328101406) (1303,1.7132417902463) (1304,1.5165523440893) (1305,1.3362214144734) (1306,1.7457246677423) (1307,1.5781607221046) (1308,1.8245186127677) (1309,1.5843088801072) (1310,1.4984963791857) (1311,1.7627075444599) (1312,2.0723877825832) (1313,1.8673239363083) (1314,1.6724138824631) (1315,1.4185393358712) (1316,1.370965861061) (1317,1.617821031561) (1318,1.6736505500573) (1319,1.8462589584073) (1320,1.2485111990919) (1321,1.428557000299) (1322,1.4510715701211) (1323,1.6385023847581) (1324,1.5215042512509) (1325,1.4722067370218) (1326,1.8976986116773) (1327,1.4822291254242) (1328,2.1380701138299) (1329,1.4931796689861) (1330,1.9537360298971) (1331,1.6230774207878) (1332,1.8181699713781) (1333,1.8777454016623) (1334,1.7641518369053) (1335,1.4065396615599) (1336,1.8877009995468) (1337,1.9264445995134) (1338,1.4737960808234) (1339,1.5830591198436) (1340,1.8063416176885) (1341,1.4763170548714) (1342,1.6417119980456) (1343,1.6906635167198) (1344,1.875752267777) (1345,1.8904082350054) (1346,1.5573006458901) (1347,1.5917329565756) (1348,1.6706991882286) (1349,1.7166056432158) (1350,1.4103672312308) (1351,1.3281604074269) (1352,1.5021723464748) (1353,1.6718776551923) (1354,1.5876700472934) (1355,1.6421761438664) (1356,1.5563481407164) (1357,1.6842499160991) (1358,1.3767981581128) (1359,1.48581652034) (1360,1.5446016326237) (1361,1.5207021270764) (1362,1.8090654195251) (1363,1.5877614265662) (1364,1.4936422903298) (1365,1.4479377727811) (1366,1.6127586237793) (1367,1.5399244239392) (1368,1.4114265537572) (1369,1.6130155313338) (1370,1.4329962154284) (1371,1.9082248541593) (1372,1.3617667874748) (1373,1.8143904987736) (1374,1.7500141183421) (1375,1.6507616932294) (1376,1.4395852562123) (1377,1.5321570114613) (1378,1.5276414631063) (1379,1.7141968184393) (1380,1.859181542729) (1381,1.8824295256324) (1382,1.4071534458979) (1383,1.6605696014183) (1384,1.38439195386) (1385,1.7905600177492) (1386,1.6166769969024) (1387,1.7429150680815) (1388,1.6006907125989) (1389,1.9881412840864) (1390,2.1507182384913) (1391,1.6092348913843) (1392,1.8847096034762) (1393,1.6702667905963) (1394,1.4566925342115) (1395,1.4700120741333) (1396,1.4649585639677) (1397,1.7124181303245) (1398,1.765901742692) (1399,1.4662165228931) (1400,1.9749574597261) (1401,1.5841206005872) (1402,1.8412203962964) (1403,1.6470871330638) (1404,1.7537938855336) (1405,1.6610377339461) (1406,1.8118186161978) (1407,1.9644845413315) (1408,2.1315533417259) (1409,1.4034130307102) (1410,1.709670789848) (1411,1.6170199854436) (1412,1.5047411458541) (1413,1.378917672379) (1414,1.7009699745902) (1415,1.6245501684457) (1416,1.92131383387) (1417,1.6489584354852) (1418,1.5025699160331) (1419,1.6970919387897) (1420,1.4542089712007) (1421,1.6289546675252) (1422,1.374323888853) (1423,1.52773100305) (1424,1.8963540689589) (1425,1.8383234300914) (1426,1.7433922613363) (1427,1.6152605087581) (1428,1.3543673317922) (1429,1.8453438967405) (1430,1.370341838793) (1431,1.6113288610407) (1432,1.6146894135022) (1433,1.62700832149) (1434,1.6360565743468) (1435,1.6399564666944) (1436,1.7891610982598) (1437,1.433139624983) (1438,1.5875173614356) (1439,1.8110742459614) (1440,1.5147267005932) (1441,1.8110113836841) (1442,1.5612487006006) (1443,1.820229556932) (1444,1.5379678968073) (1445,1.6924524090861) (1446,1.7685804015009) (1447,1.9715081486015) (1448,1.4487686675831) (1449,1.4999172150965) (1450,1.7792750372372) (1451,1.5862824865679) (1452,1.881112220979) (1453,1.5415332294597) (1454,1.4550907015556) (1455,1.6845150752542) (1456,1.6693595531203) (1457,1.8163452626212) (1458,1.525309486006) (1459,1.6902594496464) (1460,1.6658470978363) (1461,1.4267849303302) (1462,1.5343277913853) (1463,1.7738628223459) (1464,1.9005445824044) (1465,1.8502283345538) (1466,1.72587200695) (1467,1.936643710344) (1468,1.5708909145302) (1469,1.9466424873988) (1470,1.6300138422387) (1471,1.7008768574312) (1472,1.681003198101) (1473,1.7010077721839) (1474,2.2202576256754) (1475,1.9987222782394) (1476,1.681427031511) (1477,1.9978596753826) (1478,1.4463558124129) (1479,1.4029472522898) (1480,1.550684008947) (1481,1.7414958208957) (1482,2.1330668276205) (1483,1.8503389453362) (1484,1.3802982735534) (1485,1.6717004916685) (1486,1.6501574217723) (1487,1.3317277753381) (1488,1.7351604354812) (1489,1.8618471788573) (1490,1.8996538093124) (1491,1.8926214998066) (1492,1.9746320586444) (1493,1.8388568917884) (1494,1.5338945594169) (1495,1.6471292365258) (1496,1.8096025414962) (1497,1.4547078667742) (1498,1.1947897944935) (1499,1.5624007992907) (1500,1.4329317397743) (1501,1.6199237817693) (1502,1.4545897639384) (1503,1.7915497185487) (1504,1.7574691130637) (1505,1.4120214316578) (1506,1.5910806555973) (1507,1.794481730526) (1508,1.9468243557644) (1509,1.9130980097919) (1510,1.4989687048401) (1511,1.5406995597655) (1512,1.8971621367302) (1513,2.0529314639346) (1514,1.69745322139) (1515,1.7533907831366) (1516,1.6121491273803) (1517,1.7814628318241) (1518,1.6700265451505) (1519,1.6262631689771) (1520,1.9086799664703) (1521,1.7633997549345) (1522,1.47480256922) (1523,1.8154259576021) (1524,1.6290878098084) (1525,2.0289579388719) (1526,1.6492225089015) (1527,1.4996731944906) (1528,1.3900041565555) (1529,1.4030610699832) (1530,1.821485866185) (1531,2.0643038603425) (1532,1.795484581554) (1533,1.7290183032958) (1534,1.76313258653) (1535,1.4990924470694) (1536,1.5568876719067) (1537,1.456506655284) (1538,1.4067615632015) (1539,1.6110725372746) (1540,1.7091811916034) (1541,1.340860896489) (1542,1.3048754967821) (1543,2.0209804371328) (1544,1.5942640256872) (1545,1.5569771929288) (1546,2.0084375211503) (1547,1.7954240812678) (1548,1.6895591692073) (1549,1.7005753672229) (1550,1.7290844641013) (1551,1.7882721378793) (1552,1.5104456485486) (1553,1.9207492860803) (1554,1.526284190109) (1555,1.4914011697182) (1556,1.8309822484586) (1557,1.4235764854172) (1558,1.6468688793613) (1559,1.4838359532115) (1560,1.4505838106314) (1561,1.4445099294223) (1562,1.7425300660955) (1563,1.4398065164279) (1564,1.6829000218542) (1565,1.5342639367379) (1566,1.8509513393665) (1567,1.6004501500845) (1568,1.7376880288106) (1569,1.5093828279261) (1570,1.657279516467) (1571,1.801054556883) (1572,1.3717818380543) (1573,1.7421470274887) (1574,1.8660660896912) (1575,1.6503280849315) (1576,1.3749581192989) (1577,2.2047975417322) (1578,1.9330519587549) (1579,1.6075612024967) (1580,1.7160489882821) (1581,1.8854154602096) (1582,2.1186294562061) (1583,1.8239797980296) (1584,1.9980120528298) (1585,1.8334582616205) (1586,1.6000789854493) (1587,1.8048246573896) (1588,1.4414400081654) (1589,1.4988205032085) (1590,1.607969040027) (1591,1.5389039319154) (1592,1.4782895686314) (1593,1.754134957622) (1594,1.7532690202487) (1595,1.7146100765927) (1596,1.7049954178363) (1597,1.811302173383) (1598,1.6429297444889) (1599,1.5583750581783) (1600,1.6720734283773) (1601,1.597979080472) (1602,1.6099079409706) (1603,1.423215501358) (1604,1.5997832360081) (1605,1.6256424975753) (1606,1.5019172315636) (1607,1.5780689330285) (1608,1.9705416758192) (1609,1.9633016957756) (1610,1.8810500757332) (1611,1.9133343302063) (1612,1.7168295858329) (1613,1.7165496508802) (1614,1.6372143755858) (1615,1.9149875335738) (1616,1.6540026871277) (1617,1.7139024395764) (1618,2.0538146085846) (1619,1.4767348492977) (1620,1.7891144578468) (1621,1.4314264005261) (1622,1.4324861246417) (1623,1.5825710726388) (1624,1.9664623088156) (1625,1.7352577445173) (1626,1.7343595660073) (1627,1.5420935294841) (1628,1.4762728327382) (1629,1.66404126672) (1630,1.5646914731716) (1631,1.6289193384331) (1632,1.8081113757234) (1633,1.6775814374302) (1634,1.6070664387606) (1635,1.4377053379533) (1636,1.6252562182519) (1637,1.7696623624281) (1638,2.0260954984677) (1639,1.8728454174039) (1640,1.322652624384) (1641,1.3737064854973) (1642,1.5766862202094) (1643,1.4356760201054) (1644,1.7687031075338) (1645,1.6019990498406) (1646,1.6101346373168) (1647,1.6717515122236) (1648,1.6208897093552) (1649,1.8538004562184) (1650,1.6937860559117) (1651,1.9479494239777) (1652,1.4422037610224) (1653,1.6532848414055) (1654,1.6367482209504) (1655,1.6511673773504) (1656,1.5501884843545) (1657,1.7711671806174) (1658,1.7565214580894) (1659,1.5752763728922) (1660,1.7928990166053) (1661,1.9763979241937) (1662,1.7267941205301) (1663,1.433763888873) (1664,1.6939218414521) (1665,1.6280649886598) (1666,1.5534588265084) (1667,1.7869555943993) (1668,1.5380782428915) (1669,1.4626966884905) (1670,1.5872735905372) (1671,1.5226887821136) (1672,1.7691965482405) (1673,1.5678205341691) (1674,1.5177445638935) (1675,1.4670722583019) (1676,1.8941495022754) (1677,2.0550810572803) (1678,1.6356150409229) (1679,1.6891588579415) (1680,1.7766348474118) (1681,1.6611032952029) (1682,1.8355241536045) (1683,1.6318388517481) (1684,1.6366402601532) (1685,1.4450547599011) (1686,1.352639914324) (1687,1.6715032177008) (1688,1.7325464901625) (1689,1.4267394944569) (1690,1.6506258980565) (1691,1.6822363568684) (1692,2.1166037932524) (1693,1.9920364045886) (1694,1.8430357860304) (1695,1.8777259339374) (1696,2.1085033686395) (1697,2.1747386773127) (1698,1.7010009498025) (1699,2.0577572074026) (1700,2.1375493813467) (1701,1.7806477483559) (1702,1.9995446796937) (1703,1.9742223107991) (1704,1.6781232038724) (1705,1.373800812386) (1706,1.8168939977746) (1707,1.5974861925498) (1708,1.7086582290674) (1709,2.4348434195962) (1710,1.7895953453732) (1711,1.7299142784568) (1712,1.653748570791) (1713,1.6760580791593) (1714,1.3920101713598) (1715,1.3129158286477) (1716,1.4060885711591) (1717,1.6419991953968) (1718,1.8428463751573) (1719,1.7585111531786) (1720,1.9131237766247) (1721,1.8223370508662) (1722,1.9210130142733) (1723,1.7824154949848) (1724,1.6073436398678) (1725,1.6875762214125) (1726,1.749156601842) (1727,1.493051107679) (1728,1.4911534065595) (1729,1.5652036896385) (1730,1.7995340650846) (1731,1.7257068919043) (1732,2.1329022828128) (1733,1.6787855323599) (1734,1.4769679946122) (1735,1.6098523711819) (1736,1.7602242478676) (1737,1.6326923588456) (1738,1.7959488367798) (1739,1.5727956204664) (1740,1.8429557112261) (1741,1.7184713338942) (1742,1.7558118441025) (1743,1.6445715409544) (1744,1.7497220488246) (1745,1.6382792444558) (1746,1.83725544131) (1747,1.6208460541449) (1748,1.8649350361663) (1749,1.7409409333139) (1750,1.6562748471902) (1751,1.6323440321438) (1752,1.4932265787183) (1753,1.6675171773121) (1754,1.5424073225198) (1755,1.9059776856194) (1756,1.5758878167897) (1757,1.7882870964129) (1758,1.76368343723) (1759,1.4225420781601) (1760,1.7631680364348) (1761,1.8676197449423) (1762,1.644433256448) (1763,1.5978438608792) (1764,1.4240597332767) (1765,1.545272166325) (1766,1.5943053514092) (1767,1.4557204011561) (1768,1.8658650419577) (1769,2.1278574104803) (1770,1.4680100144406) (1771,1.4954606661471) (1772,1.9942411262257) (1773,1.8590232762948) (1774,1.8817960901928) (1775,1.8510890258207) (1776,1.7782399633214) (1777,1.5055790042488) (1778,1.7268517916388) (1779,2.1006887848033) (1780,1.6632465855512) (1781,1.91999613817) (1782,1.5799429935507) (1783,1.6085737922737) (1784,1.6278021799098) (1785,1.8586783432254) (1786,1.436691794024) (1787,1.5634849215333) (1788,1.4902655191788) (1789,1.4701095491828) (1790,1.6123274977796) (1791,1.6250852880605) (1792,1.65535263694) (1793,1.9091164072663) (1794,2.0821038662223) (1795,1.8602409888736) (1796,1.6562571938244) (1797,2.0091594844123) (1798,2.0780822431043) (1799,2.0269591133627) (1800,1.6231591492615) (1801,1.7575562569123) (1802,1.6224234463105) (1803,1.460521731326) (1804,1.5813579419536) (1805,1.8361516121277) (1806,1.807866554378) (1807,1.6593699357644) (1808,1.5989538679036) (1809,1.510636230119) (1810,1.7180550966863) (1811,1.6845023583538) (1812,1.7379774607264) (1813,1.6586343258291) (1814,1.6857979744545) (1815,1.7541406226881) (1816,1.9887085135368) (1817,1.6229472463746) (1818,1.5335377947803) (1819,1.6976512300574) (1820,1.8963697619321) (1821,1.9347935730883) (1822,1.7073743804854) (1823,1.9933217915531) (1824,1.7656893210066) (1825,1.7193941214292) (1826,1.5471251892162) (1827,1.5763952526179) (1828,1.8225869489544) (1829,1.8055315281639) (1830,1.6895342479623) (1831,1.6753375690986) (1832,1.6962328424495) (1833,1.7581903354734) (1834,1.4629366750819) (1835,1.5299352851189) (1836,1.725863224482) (1837,1.6116336240227) (1838,1.5892431770237) (1839,1.698163717611) (1840,1.7861353960779) (1841,1.2947889224857) (1842,1.7129689755009) (1843,1.3548150232542) (1844,1.5126711197044) (1845,1.8970731331678) (1846,1.5533030081267) (1847,1.9476670695929) (1848,1.8993376088411) (1849,1.9208986409456) (1850,1.854841061455) (1851,1.6238056479911) (1852,1.7503095814878) (1853,1.802605924549) (1854,1.7281266427646) (1855,1.9587823782009) (1856,1.4882206741147) (1857,1.8004751885893) (1858,1.8661539882721) (1859,1.5635200588861) (1860,1.5520691323804) (1861,1.7453483948853) (1862,1.8933634631274) (1863,1.5107015817735) (1864,1.8004290257545) (1865,1.5738052754366) (1866,1.7337462909825) (1867,1.639526541308) (1868,1.962237664947) (1869,1.7309019568244) (1870,1.4314210660229) (1871,1.6148266003918) (1872,1.9575448392425) (1873,1.370635970472) (1874,2.0220465679548) (1875,1.6947648430131) (1876,1.5636195608711) (1877,1.8103747001245) (1878,1.7889445849075) (1879,1.8852131054521) (1880,1.960133633867) (1881,2.0009640753468) (1882,1.8623794308908) (1883,1.6463404067103) (1884,1.3002768431326) (1885,1.5437341320401) (1886,1.4880786364606) (1887,1.4779266128648) (1888,1.5886337924969) (1889,1.7843651157561) (1890,1.7537562738874) (1891,1.7500532497585) (1892,1.5076588359669) (1893,1.5541497037168) (1894,1.2770286242388) (1895,1.7730419315184) (1896,1.6145519319352) (1897,1.6066142099391) (1898,1.7206694880995) (1899,1.7652670984607) (1900,1.4865045724203) (1901,1.6510253445952) (1902,1.8418913558315) (1903,1.631196661441) (1904,1.9565696008608) (1905,1.6872653455917) (1906,1.6179722069033) (1907,1.6121055505267) (1908,1.8384666252782) (1909,1.7973892750972) (1910,1.3892546432252) (1911,1.6602562010827) (1912,1.8231629592329) (1913,1.6530775549135) (1914,1.7583755484117) (1915,1.7131124448602) (1916,1.9723543063281) (1917,1.6988253841156) (1918,1.3495674778383) (1919,1.666093674855) (1920,1.6157881411625) (1921,1.8148515218926) (1922,1.4830894575854) (1923,1.4758514479207) (1924,1.7560476446687) (1925,1.6491706896558) (1926,1.5117059478191) (1927,1.6908892403279) (1928,1.1993096603834) (1929,1.4012695411647) (1930,1.8426578405131) (1931,1.734366642324) (1932,1.7353585759344) (1933,1.9918467305833) (1934,1.7369263517795) (1935,1.8588923711595) (1936,2.2810992174147) (1937,1.2856167089911) (1938,1.6776393773814) (1939,1.503881032838) (1940,1.7787595074851) (1941,1.3172345905518) (1942,1.6172733909958) (1943,1.4125700517956) (1944,1.9822132401819) (1945,2.0367516401826) (1946,1.8177362745347) (1947,1.6643214214365) (1948,1.7755432061062) (1949,1.6134210595959) (1950,1.5260244464645) (1951,2.0042742934893) (1952,1.4724519981443) (1953,1.3117548231776) (1954,1.510853977344) (1955,1.7406085337037) (1956,1.6203612128765) (1957,1.7904806652286) (1958,1.437045472197) (1959,1.8918818591449) (1960,1.5844270681869) (1961,1.3588348749447) (1962,1.70200293905) (1963,1.6299133079874) (1964,1.8215635112627) (1965,1.7194161981122) (1966,1.7385569110036) (1967,1.5165685264577) (1968,1.615006725756) (1969,1.8242506522553) (1970,1.8444239532161) (1971,1.4459771899469) (1972,1.587512079021) (1973,1.8339273198586) (1974,2.081415878897) (1975,1.8353775514934) (1976,1.3675403094504) (1977,1.368346080529) (1978,1.8497799038153) (1979,1.4004883152255) (1980,1.3782016674149) (1981,1.54129857425) (1982,1.5842499495894) (1983,1.6735640074999) (1984,2.1122599329963) (1985,1.5164585938034) (1986,1.7413073752557) (1987,1.9920948804698) (1988,1.8068062416933) (1989,1.6523603105735) (1990,1.6999864048219) (1991,1.9518016360251) (1992,1.7343655544892) (1993,2.1039190375302) (1994,2.0201856442722) (1995,1.9715987187431) (1996,1.7118943868266) (1997,1.4833367745702) (1998,1.6596666479769) (1999,1.4830585342919) (2000,1.7679911286168) };


==> supplemental_experiments.tex <==
%!TEX root = cvpr2017A_supplement.tex
\clearpage
\section{$\EMD$ as pre-training on ImageNet}

\begin{figure}[h]
\centering
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[   height=3cm,  width=6cm,
y filter/.code={\pgfmathparse{100*(1-#1)}\pgfmathresult},
scale only axis, ymin=0,ymax=20,xmin=2,xmax=200 ,enlargelimits=false, y label style={at={(axis description cs:-0.075,.5)},anchor=south},  ylabel=Top-1 Accuracy (\%),  x label style={at={(axis description cs:0.5,-0.1)},anchor=north},  xlabel=Epoch, legend cell align=left, legend pos=outer north east, legend style={font=\tiny}]
\addplot+[olive, line width=1pt, mark=none, line join=round] table[x expr=\coordindex+2, y index=1] {results/CE_0_LR005_ErrorRate1.log};
\addplot+[teal,  line width=1pt, mark=none, line join=round] table[x expr=\coordindex+2, y index=1] {results/EMD2_0_ErrorRate1.log};
\addplot+[blue,  line width=1pt, mark=none, line join=round] table[x expr=\coordindex+2, y index=1] {results/SMALL_EMD1.log};
\addplot+[red,   line width=1pt, mark=none, line join=round] table[x expr=\coordindex+2, y index=1] {results/SMALL_EMD_TO_CE1.log};
\legend{$\CE$,$0.5 CE $+$ 0.5 \EMD^2$,$\EMD^2$,$\EMD^2$ until epoch 135 and then $\CE$}
\end{axis}
\end{tikzpicture}
\caption{
Top-1 accuracy on ImageNet using 50K images for training using different loss functions.
The $\CE$ loss strongly favors Top-1 accuracy, therefore it trains fast with regards to this metric.
Conversely, $\EMD^2$ tries to optimize the entire output space resulting in a slower convergence rate.
The combined $0.5 \CE + 0.5 \EMD^2$ shows mixed performance, achieving fast convergence and better accuracy.
However, if we give enough time to let $\EMD^2$ embed the output hierarchy in the network, and then further train the network using the $\CE$ loss we achieve the best results on this metric.
}
\label{fig:pretraining}
\end{figure}

%{\color{red}needs a caption. also, maybe legend to EastOutside?}


In the main paper (Sec. 5.3), we report the results of training on the reduced ImageNet (50K images) dataset using the CrossEntropy~($\CE$) loss alone, the regularized Earth Mover's Distance~($\EMD^2$) loss alone, and an equally weighted combination of the two.
The combined loss $0.5 \CE + 0.5 \EMD^2$ outperforms both individual losses, and also shows fast convergence.

However, as the output space is very large, we think that $\EMD^2$ is not provided the opportunity to learn the output space hierarchy on the model when used in combination with $\CE$.
To test this hypothesis, we perform the following experiment.

We train using the $\EMD^2$ loss until Top-1 accuracy stops improving.
This acts as a pre-training step for the network.
In our experiment this happens at epoch 135.
We then switch the loss function to $\CE$ and employ a very small learning rate (0.001) that only refines the learned parameters of the network.

As $\CE$ strongly favors Top-1 accuracy, it learns on top of the previous network to achieve a Top-1 accuracy of $14.97\%$ (compared to $6.34\%$ for $\CE$, $8.20\%$ for $0.5 \CE + 0.5 \EMD^2$, and $7.66\%$ for $\EMD^2$).
\figref{pretraining} shows the performance for the proposed experiment.
%{\color{red}can you also plot CE + EMD on this?}


